Mechanism Design for Value Maximizers

In many settings, money is a tool of exchange with minimal inherent utility --- agents will spend it in a way that maximizes the value of goods received subject to reasonable constraints, giving only second-order consideration to the trade-off between value and price. While this perspective is commonly captured in consumer choice theory, market equilibrium theory, and other fields, it is markedly absent from the mechanism design literature --- agents strategizing in a mechanism with money are almost always assumed to incorporate money as an objective through quasilinear valuations. We study a simple model of value maximizers that captures online advertisers and other agents who may view money solely as a constraint, and study general questions of mechanism design for such agents. We show that the feasible and optimal points faced by a mechanism designer change dramatically from the quasilinear realm and lay a foundation for a broader study of value maximization in mechanism design. Along the way, we offer new insight into the generalized second price (GSP) auction commonly used in Internet advertising. Through the lens of value maximization, GSP metamorphosizes into a truthful auction, sound in its principles and elegant in its simplicity.

==> alpha-hybrid.tex <==


\section{$\alpha$-Hybrid Utilities}  \label{sec:a-alpha-hybrid}

It is interesting to consider a hybridization of quasilinear and value-maximizing utilities for both theoretical and practical reasons. On the theory side, it illustrates the connection between the welfare-maximizing auctions. On the practical side, it gives a way to implement a mechanism when bidders' true preferences are believed to lie somewhere between the extremes. For this purpose, we introduce the following model:

\begin{definition}%[$\alpha$-Hybrid Utilities]
\label{def:ahp}
A bidder with {\em $\alpha$-hybrid utilities} wishes to maximize the utility $u_i(o, p_i)=v_i(o)^\alpha-p_i^\alpha$.
\end{definition}

Note that for $\alpha=1$ these are quasilinear preferences, and in the limit when $\alpha\rightarrow\infty$ they become value-maximizing, except in the case where $v_i=p_i$ (this event will have measure zero in our auctions).

\subsection{Hybrid Generalized GSP}

While we contend that value maximization is a better model of bidder preferences than quasilinear, it also has its own problems. For example, a value maximizer will prefer 1000 clicks at \$1 each to 999 clicks for free. We hypothesize that bidders' true preferences lie somewhere between quasilinear and value-maximizing, and propose that another way to generalize GSP is to design an auction truthful for $\alpha$-hybrid preferences:

\begin{definition}[Hybrid Generalized GSP]
The hybrid generalized second price auction (GSP) is the auction that maximizes welfare in the standard quasilinear sense, then charges prices that are truthful for a bidder with $\alpha$-hybrid preferences.
\end{definition}


\subsection{Generalizing VCG}

As hinted by our mention of $L^p$-norms, we can use $\alpha$-hybrid preferences to illustrate why the mechanism we proposed in Section~\ref{sec:value-max} generalized the structure of VCG. In particular, we will see that the natural analog of VCG maximizes the $L^\alpha$-norm of welfare:
\begin{definition}\label{def:awm-auction}
The {\em $L^\alpha$-welfare-maximizing auction} proceeds as follows:
\begin{enumerate}
\item Choose the outcome $o^*$ that maximizes the $L^\alpha$-norm of bidders' values, i.e.
\[o^*=a(b)=\argmax_o \left(\sum_ib_i(o)^\alpha\right)^{\frac{1}{\alpha}}\]
%\[o_{-i}^*=a(b_{-i},0)=\argmax_o \left(\sum_{j\neq i}b_j(o)^\alpha\right)^{\frac{1}{\alpha}}\]
\item Charge ``externality payments''
\[p_i(b)=\left(\sum_{j\neq i}\left(b_j(o_{-i}^*)^\alpha-b_j(o^*)^\alpha\right)\right)^{\frac1\alpha}\]
where $o_{-i}^*$ is the optimal outcome with bidder $i$ removed.
\end{enumerate}
For $\alpha=\infty$, we choose $o$ to maximize the limit of the $L^\alpha$-norm of welfare as $\alpha\rightarrow\infty$, and take the limit of the payment function.
\end{definition}
It is a straightforward exercise to verify that the limiting behavior of this auction matches the informal Definition~\ref{def:wm-auction}.

\begin{theorem}\label{thm:ah-welfare-auction}
For any $\alpha$-hybrid utilities ($\alpha\leq\infty$), the $L^\alpha$-welfare-maximizing auction is truthful (DSIC-AE).
\end{theorem}

\begin{proof} When $\alpha<\infty$, the proof follows the standard reasoning for VCG --- we can write bidder $i$'s uility for bidding $b_i$ when her true value is $v_i$, as follows:
\[u_i(v_i, b_i)=v_i(b)^\alpha-p_i(b)^\alpha=v_i(b)^\alpha+\sum_{j\neq i}b_j(b)^\alpha-\sum_{j\neq i}b_j(b_{-i},0)^\alpha\enspace.\]
The standard observation is that bidder $i$ cannot affect the last term, and the first two terms are precisely the welfare objective maximized by the mechanism, so $i$ cannot gain by lying.

For the case where $\alpha=\infty$, we defer proof until Theorem~\ref{thm:ah-unrestricted}. In that theorem, we show that any $L^\infty$-affine maximizer is truthful, of which this welfare maximizing auction is a special case.\footnote{We could have relied on Theorem~\ref{thm:ah-unrestricted} for the entire proof of this theorem.}
\end{proof}



\subsection{Unrestricted Domains}

For quasilinear utilities, it is known that the only mechanisms implementable in the most general settings are affine maximizers~\cite{roberts79}. While we have discussed how a broader range of ``bias'' schemes are implementable for value maximizers, we show that this is a fragile result that only holds for value maximizers --- for bidders with $\alpha$-hybrid preferences over value and money, we show that affine maximizers are the only kind of truthful mechanism for all finite $\alpha$.

\begin{definition}
A mechanism is a {\em $L^\alpha$-affine-maximizer} if it maximizes $\left(z(o)^\alpha+\sum_i(w_ib_i(o))^\alpha\right)^{\frac1\alpha}$.
\end{definition}

\begin{theorem}\label{thm:ah-unrestricted}
For any $\alpha<\infty$, when $|\mathcal O|\geq3$, bidders are $\alpha$-hybrid, and bidders can have any value function $v_i:\mathcal O\rightarrow\Re^+$ (the standard unrestricted setting), the only truthful mechanisms are $L^\alpha$-affine-maximizers.
\end{theorem}

\begin{proof} We reduce to and from quasilinear mechanisms, then rely on~\cite{roberts79} to do the rest of the work. The main observation is that a mechanism that is truthful for bidders with utilities $u_i=v_i^\alpha-p_i^\alpha$ is equivalent to a truthful mechanism for quasilinear bidders with $u_i=\hat v_i-\hat p_i$, where $\hat v_i=v_i^\alpha$ and $\hat p_i=p_i^\alpha$.

Formally, we first show that any truthful mechanism must be an $L^\alpha$-affine maximizer for $\alpha<\infty$. Suppose we are given a truthful mechanism $\mathcal M^\alpha=(f_\alpha,p_\alpha)$ for some $\alpha$. Observe that by truthfulness of $M_\alpha$, it must be that bidder $i$ prefers reporting her true value $v_i$ to reporting another value $b_i$:
\[v_i(f_\alpha(b_{-i},v_i))^\alpha-p_{\alpha,i}(b_{-i},v_i)^\alpha\geq v_i(f_\alpha(b))^\alpha-p_{\alpha,i}(b)^\alpha\enspace.\]

Now, we construct a mechanism $\mathcal M^q$ that is truthful for quasilinear bidders with value $\hat v_i$ as follows: the outcome is $f_q(\hat v_i)=f_\alpha(\hat v_i^{\frac1\alpha})$ and the payments are $p_{q,i}=p_{\alpha,i}^\alpha$. To see that this is truthful, observe that a quasilinear bidder with value $\hat v_i$ prefers to bid $v_i$ than $\hat b_i$:
\begin{align*}
u_i&=\hat v_i(f_q(\hat b_{-i},\hat v_i))-p_{q,i}(\hat b_{-i},\hat v_i)\\
&=\left(\hat v_i(f_\alpha(\hat b_{-i}^{\frac1\alpha},\hat v_i^{\frac1\alpha}))^{\frac1\alpha}\right)^\alpha-p_{\alpha,i}(\hat b_{-i}^{\frac1\alpha},\hat v_i^{\frac1\alpha})^\alpha\\
&\geq\left(\hat v_i(f_\alpha(\hat b^{\frac1\alpha}))^{\frac1\alpha}\right)^\alpha-p_{\alpha,i}(\hat b^{\frac1\alpha})^\alpha\\
&=\hat v_i(f_q(\hat b))-p_{q,i}(\hat b)\enspace,
\end{align*}
where the inequality comes from truthfulness of $\mathcal M^\alpha$.

By Roberts's Theorem, $f_q$ must be an affine maximizer, so our reduction tells us that $f_\alpha(\hat b^{\frac1\alpha})$ must also be an affine maximizer, i.e.
\[f_\alpha(\hat b^{\frac1\alpha})=\argmax_o \hat z(o)+\sum_i\hat w_i\hat b_i(o)\enspace.\]
%which implies
%\[f_\alpha(b)=\argmax_o \hat z(o)+\sum_i\hat w_ib_i(o)^\alpha\enspace.\]
By defining $\hat z(o) = z(o)^\alpha$ and $\hat w_i=w_i^\alpha$ we get that $f_\alpha$ is precisely an $L^\alpha$-affine-maximizer:
\[f_\alpha(b)=\argmax_o z(o)^\alpha+\sum_iw_i^\alpha b_i(o)^\alpha=\argmax_o \left(z(o)^\alpha+\sum_iw_i^\alpha b_i(o)^\alpha\right)^{\frac1\alpha}\enspace.\]


To complete the case where $\alpha<\infty$, it is necessary to show that any $L^\alpha$-affine maximizer is truthful. In the quasilinear case, this is the easy direction for Roberts's theorem and is straightforward to do from first-principles --- the same is true here in the manner of Theorem~\ref{thm:ah-welfare-auction}. Alternatively, we could use a similar reduction to prove that any $L^\alpha$-affine maximizer is truthful. We leave either as an exercise. \end{proof}


==> general.tex <==


\section{GSP Defined and Generalized}  \label{sec:general}

A significant byproduct of our results in Section~\ref{sec:truthful} is that we now have a theoretically justified axiomatic definition of GSP:
\begin{proposition}%[Generalized GSP]
\label{prop:ggsp}
A generalized second price auction (GSP) maximizes expected bidder value and charges prices that make the auction truthful for simple value maximizers.
\end{proposition}
This definition is important because it allows us to soundly extend GSP to new contexts. A small existing literature has struggled to generalize GSP in the context of quasilinear bidders, generally finding equilibria may not exist and that even when they do, they may not be efficient~\cite{deng10,cavallo14,bachrach14}. Our work suggests that these negative results are because GSP's strength was misunderstood.

Generalizing GSP is an important problem because ads are becoming progressively more complex, and with them the algorithms required to optimize their placement and features. The traditional separable model is a poor fit for these settings, so GSP does not immediately apply and the industry has typically moved to a VCG auction due to its purported truthfulness and elegant implementation. Facebook and Google's Contextual Ads~\cite{varian14} adopted VCG for precisely these reasons. However, those implementations of VCG were straightforward because they were largely from scratch; VCG is a more problematic prescription for established marketplaces like sponsored search that are currently based on GSP. Advertisers are accustomed to GSP prices, so any switch will force advertisers to revise their expectations. Moreover, GSP prices are higher than their VCG counterparts, so to the degree that advertisers do not react, there may be a significant revenue loss for the advertising platform.  A small research thread has explored ways to transition smoothly from GSP to VCG (e.g.~\cite{bachrach16}), again assuming bidders maximize profit. Our approach of understanding GSP through alternative models of advertiser preferences gives a new foundation for tackling this problem, and Cavallo et al.~\cite{cavallo17} use results from this paper and~\cite{cavallo15} as the foundation for an application to Yahoo's sponsored search platform.

\subsection{Single Parameter Generalizations}

To generalize GSP we will characterize the allocations that can be implemented truthfully for value maximizers. In quasilinear settings, it is known that any monotone allocation rule is incentive compatible~\cite{myerson81, archer01}; we find that the same is true for value maximizers. This auction has very simple prices: the price is the minimum values required to maintain the same allocation $x$:

\begin{theorem}\label{thm:vm-sp-char}
For simple value maximizers in a single parameter domain, a mechanism is truthful (DSIC-AE) if and only if it is monotone and the price is the minimum value required to get the same allocation:%a mechanism is truthful and individually rational if and only if it is monotone in the standard sense. Prices are computed for a bid $b_i$ by finding the minimum bid $\underline b_i$ that achieves the same allocation $x_i(b_{-i},b_i)$ and setting $p_i(b_{-i})=\underline b_i x_i(b_{-i},b_i)$.
\begin{itemize}
\item {\em (monotonicity)} for any $v_{-i}$, $x_i(z, v_{-i})> x_i(v)$ if and only if $z>v_i$ almost everywhere over $v_i$
\item {\em (pricing)} $p_i(v)=\inf_{z|x_i(z, v_{-i})=x_i(v)}z$
\end{itemize}
\end{theorem}
Before we prove our characterization we note an important corollary:
\begin{corollary}
For any monotone $x_i$, the mechanism that charges $p_i(v)=\inf_{z|x_i(z, v_{-i})=x_i(v)}z$ is DSIC-AE.
\end{corollary}
This corollary follows because the $\inf$ only differs from the $\min$ where $x$ is discontinuous, and a monotone function is continuous almost everywhere (discontinuities are countable and therefore have measure zero).


\begin{proof}[of Theorem~\ref{thm:vm-sp-char}.] Fix other bidders' values $v_{-i}$ and drop them for clarity.


{\em Necessity.} Fix a type $v_i$ and define
\[\mathcal{Z}^<=\{z|x_i(z)<x_i(v_i)\}\quad\mbox{and}\quad \mathcal{Z}^==\{z|x_i(z)=x_i(v_i)\}\]
to be the types that get a strictly smaller allocation than $v_i$ and an equal allocation respectively. A value maximizer with single parameter type $v_i$ will choose a bid $b_i$ that maximizes $x_i(b_i)$ subject to $p_i(b_i)\leq v_i$. Thus, for any $v_i$, $p_i(v_i)$ must be high enough that bidders who get a smaller allocation do not want to lie, i.e.
\[p_i(v_i)\geq \underline p_i\triangleq\sup \mathcal{Z}^<\enspace.\]
Similarly, all types who exactly get $x_i(v_i)$ must pay the same price, and it must be that any bidder who gets $x_i(v_i)$ must be willing to pay for it, so
\[p_i(v_i)\leq\overline p_i=\inf \mathcal{Z}^=\enspace.\]
Since $\sup\mathcal{Z}^<\geq\inf\mathcal{Z}^=$, it must be that $\underline p_i\geq\overline p_i$, and therefore to satisfy $\underline p_i\leq p_i(v_i)\leq \overline p_i$ a mechanism will be truthful if and only if $\underline p_i=\overline p_i=p_i(v_i)$ --- this happens if and only if $x$ is nondecreasing and is the price defined in the theorem.

{\em Sufficiency.} Note that for DSIC-AE we only need to prove sufficiency almost everywhere. We must consider three deviations: (1) a bidder underbids for a smaller allocation, (2) a bidder deviates for the same allocation at a lower price, and (3) a bidder overbids for a larger allocation. Remark that deviation (1) will not happen because a value maximizer will always want the larger allocation (since $p_i(v_i)\leq v_i$ by definition of $p_i$), and that  (2) cannot happen because all types who get the same allocation pay the same price.

It remains to show that bidders almost never have an incentive to raise a bid (3). Deviation (3) will only be beneficial if there exists a type $z>v_i$ such that $x_i(z)>x_i(v_i)$ but $p_i(z)<v_i$. By definition of $p_i$, there exists a type $\underline b_i(z)\geq v_i$ such that
\[p_i(z)=\underline b_i(z)\enspace.\]
As long as $\underline b_i(z)>v_i$ this deviation cannot be beneficial. Unfortunately, when $b_i(z)=v_i$ then deviation (3) will be beneficial; however, this can only happen at a discontinuity in $x$. Since $x$ is monotone, discontinuities can only happen rarely (the set of discontinuities is countable and therefore has measure 0) and we get truthfulness in our almost-everywhere sense (DSIC-AE).
\end{proof}

\subsection{Substantiating GSP's Folk Definition}

While we have given the first rigorous axiomatic definition of GSP, the following folk description is well-known:
\begin{proposition}[Folklore]
GSP is the auction that maximizes expected bidder value and charges the minimum bid required to keep the same allocation.
\end{proposition}
Until now, this definition was merely a pleasant-sounding heuristic for general auction settings; however, our work gives this definition theoretical teeth:
\begin{obs}
The folklore definition of GSP is equivalent to the truthful auction for value maximizers defined in Theorem~\ref{thm:vm-sp-char}.
\end{obs}
By consequence, this folklore definition is also equivalent to Proposition~\ref{prop:ggsp}, closing the loop on defining GSP.








==> introduction2.tex <==


\section{Introduction}  \label{sec:intro}

%Quasilinear utilities epitomize {\em lex parsimoniae}: they are ubiquitous in economics because they are the simplest objective that trades value for money. However, exceedingly large categories of strategic agents do not even consider money to be a first-order objective; rather, agents want value, and money is simply a constraint. This is true across a wide range of settings, from corporate purchasing (e.g. advertising) to individual consumer behavior (e.g. housing).

%In this paper, we start with the agents we know best---online advertisers---and
%find that a remarkably simple {\em value-maximizing} model captures their
%preferences surprisingly well.\footnote{A similar model was discovered independently in concurrent
%work by Fadaei and Bichler~\cite{fadaei16}. See related work.} \if Moreover, advertisers are not unique; our
%model arises naturally in many common situations where budgets are fixed ex
%ante or profit is difficult to measure. \fi Our model can be seen as the
%natural embodiment of {\em lex parsimoniae} when money is merely a constraint:


It is widely acknowledged that advertisers will have complex preferences and behaviors (e.g.~\cite{aggarwal09}), but it has gone unquestioned that a quasilinear utility model is the natural starting point for designing ad auctions. But from a vantage point within a company that sells advertising, this strains credulity; considering requests from both advertisers and the account managers who advocate on their behalf, the way buyers interact with a marketplace and make local bidding decisions is very far from profit maximization.  Rather, advertiser behavior is more fundamentally driven by a desire to maximize the value of what they buy --- total impressions, clicks, sales, market share, etc. --- subject to budget constraints and return on investment (ROI) demands. For these bidders, a remarkably simple {\em value-maximizing} model captures their
preferences surprisingly well:\footnote{A similar model was discovered independently in concurrent
work by Fadaei and Bichler~\cite{fadaei16}. See related work.}

\begin{definition}%[Simple Value Maximizer, Informal\footnote{A similar model
%matching the informal definition was discovered independently in concurrent
%work by Fadaei and Bichler~\cite{fadaei16}. See the section on related work.}]
%
A {\em simple value maximizer} maximizes value $v_i$ while maintaining budget balance, i.e. while keeping
payment $p_i\leq v_i$; when value is equal, a lower price is preferred.
%
\end{definition}

Of course, bidders are rarely willing to surrender their whole value as payment; however, this objection fades and the model carries surprising
power when bids are reparameterized in terms of what a bidder is
willing to pay. For example, a constraint on return on investment (ROI) simply maps preferences to a reduced value function: a value maximizer who requires ROI at least
$\gamma$ will require $p_i\leq \frac{v_i(o)}{1+\gamma}$,\footnote{ROI is
computed as $\frac{v_i(o)-p_i}{p_i}$, so $ROI\geq\gamma\Rightarrow p_i\leq
\frac{v_i(o)}{1+\gamma}$.} ergo such a bidder is equivalent to a value maximizer with a reduced value
$v_i'(o)=\frac{v_i(o)}{1+\gamma}$ for many purposes. In particular, {\em if we run a mechanism that is truthful for value maximizers, it will be a dominant strategy for bidders to report their true willingness-to-pay $v_i'$}. The ability to reparameterize bids as willingness-to-pay is used in both our work and a
parallel work by Fadaei and Bichler~\cite{fadaei16}, and naturally maps to the meaning ascribed to bids in practice.



We begin with a theoretical study to identify allocations that can be implemented truthfully. When bidders' values fit the standard single-parameter model, we get the same result as in quasilinear settings: an allocation is implementable if and only if it is monotone. Next we consider general domains and present the natural analog of VCG's externality pricing; interestingly we prove that the space of implementable mechanisms expands beyond the obvious affine maximizers suggested by Roberts's Theorem~\cite{roberts79}.

Next, we make an interesting observation bridging theory and practice: the generalized second price (GSP) auction commonly used in practice is the truthful auction for value maximizers (this was first discovered by Aggarwal et al.~\cite{aggarwal09} in the context of a general matching model). This observation not only justifies GSP's use and desirability, but also lays a foundation for generalizing GSP that can address a current industry challenge.

Finally, we show that value maximizers are practically useful because a wide variety of preferences converge to value maximization in the presence of ROI constraints. The conditions under which this happens are surprisingly testable, and we show that the vast majority of auctions on a slice of traffic from Yahoo's Gemini Native platform would be truthful for bidders with a plausible ROI constraint.






\paragraph{Preferences of Online Advertisers}

Online advertisers are quintessential examples of value maximizers. One class of advertisers target growth and reach; they are intuitively modeled as value maximizers. These advertisers want to reach as many people as they can, generate as many clicks as they can, capture as much market share as they can, generate as much revenue as they can, and so on. These objectives are often designed to meet business goals other than profit (e.g. revenue growth), are difficult to map to money (e.g. market share), or are difficult to directly measure (e.g. monetary impact of display advertising). Thus, instead of managing a delicate trade-off between value and money, it is natural that such an advertiser tries to purchase as much advertising as possible without violating coarse spending constraints.

When advertisers do consider cost-benefit trade-offs as a primary concern, return on investment (ROI) is the standard metric across all types of advertising. ROI measures the ratio of the profit obtained (``return'') to the price paid (``investment''), i.e., the density of profit in cost:
\[\texttt{ROI}=\frac{\texttt{Value-Price}}{\texttt{Price}}=\frac{\texttt{Profit}}{\texttt{Price}}\enspace\]
Being a density metric, unconstrained maximization of ROI is not sensible;\footnote{Unconstrained maximization of ROI would likely cause an advertiser to buy only the single cheapest impression or click available.} instead, it is used as a constraint or coupled with other constraints:
\begin{itemize}
\item {\em ROI as a constraint; value as an objective.} An advertiser with a ROI constraint naturally tries to buy as much advertising as possible while maintaining ROI at least $\gamma$, i.e., $\frac{v_i-p_i}{p_i}\geq\gamma$.
\item {\em ROI as an objective; total cost as a constraint.} An advertiser who makes ROI an objective subject to a fixed demand that an exact amount of money be spent (no more, but also no {\em less}).
\end{itemize}
Both of these scenarios point towards the same fundamental model of preferences: advertisers buy as much advertising as possible subject to constraints on ROI and total spend. In this paper we will focus on advertisers with ROI constraints.

An orthogonal justification our model is that bidders often use ROI as a heuristic. For example, ROI targets are a way to maximize the effectiveness of a fixed advertising budget~\cite{borgs07,kitts04,szymanski08,zhou08,auerbach08} among auctions on the same advertising platform (as in a display advertising exchange), between advertising platforms (deciding how to bid between Yahoo and Google), and even structuring spend within a company (incentives for individual marketing staff).

Anecdotal evidence also highlights ROI-centric behavior across all sizes and types of performance-driven advertisers. For example, the following story plays out regularly at Yahoo:
\begin{enumerate}
\item Advertiser X designates a small budget for testing a Yahoo advertising product.
\item Advertiser X measures ROI --- if X is happy with its ROI, it increases its budget hoping to {\em maintain the same ROI}; if it is unhappy, it withdraws.
\end{enumerate}
The standard industry tools paint a similar picture: Google's AdWords campaign management tool buys as much advertising as possible while maintaining a target average CPC and budget --- an average CPC constraint is appropriate for ROI-centric preferences, while a marginal CPC constraint would be appropriate for profit-centric preferences. Yahoo's display ad products also offer options with ``CPC goals'' and ``CPA goals'' that buy impressions while aiming to achieve a target average cost-per-click or cost-per-conversion (e.g., cost per purchase) respectively.


Thus, we reach the conclusion that {\em advertisers are naturally modeled as
bidders who prefer more value as long as ROI, budget, and value constraints are
satisfied}. There are always exceptions; anecdotal evidence suggests that a
savvy minority of small businesses do target profit. In small businesses,
advertising is often managed by the business owner, so it is easier to directly
tie advertising to profit. Likewise, there are special cases with unusual
objectives, such as an advertiser who (rationally or irrationally) always wants
the top slot on Google. Such outlying examples will exist for any model; we
contend that value maximization is simple, empirically well-motivated, and thus
worthy of dedicated study.


\paragraph{Value Maximizers Beyond Advertising}

Parallel models to value maximization are standard in many areas. For example, the default model in demand theory --- which underpins both consumer choice theory and general equilibrium theory --- is that consumers choose their favorite bundle among the choices they can afford~\cite{mas-collel95}. This is related (but not identical) to value maximization with a budget constraint in our model. A value-maximizing consumer with a budget constraint would buy the best item/bundle that (a) is worthwhile at the offered price and (b) satisfies its budget. Buying a house is an example: buyers will commonly fix a budget and what they are willing to pay for particular features, then push to get as much ``value'' out of the house as possible---number of rooms, land, upgrades, etc.---subject to those constraints. Remark that in the interest of simplicity, we do not study budgeted value maximizers in this work.

Even when (e.g.) profit maximization is a better fit for an agent's true preferences, value maximizing behavior can naturally arise when long-term value is unclear or constrained by present circumstances. For example, markets often evaluate companies on both their revenue and profit, where instantaneous revenue is taken a signal of long-term performance instead of the more mathematically-appealing future-discounted-profit. Companies will also commonly need to make an instantaneous profit, limiting their ability to, e.g., buy advertising whose payout is far-out and/or unclear.

Value maximizing behavior also arises naturally any time agents spend money that is not their own.
This is particularly common in large organizations like companies and
governments --- an employee is given a budget for a particular task (say, to
provide food for an event), and the employee is typically rewarded primarily
for doing that task well, not for saving money. %Since the money is not the
%employee's, she won't get any benefit from underspending the budget. Thus, the
%only incentive is to maximize value of what is provided (say, quality or
%quantity of food) with the budget as a constraint.
Again, advertising is a special case.


\paragraph{Truthful Mechanisms for Value Maximizers}

Since value maximizers do not fit the standard models in the current literature, we first revisit foundational results in mechanism design and extend the standard single-parameter and affine-maximizer results to value maximizers. An immediate challenge is that value maximizers have a kind of lexicographic preference that cannot be represented by a utility function --- they prefer value first, and only care about price for a fixed value.

For single-parameter domains, we show that an allocation rule can be implemented if and only if it is monotone, just as in the standard quasilinear setting~\cite{myerson81, archer01}. The price a bidder pays is the minimum bid required to receive the same value. Our proof is a general characterization that applies to a large family of bidder preferences, not just value maximizers.

For general domains, we show that an externality-based mechanism analogous to the celebrated Vickrey-Clarke-Groves mechanism (VCG) always exists. In quasilinear settings, maximizing the $L^1$-norm of agents' values is known as maximizing welfare; it is always incentive compatible with externality payments. For value maximizers, we show that the analogous mechanism loosely maximizes the $L^\infty$ norm of agents values and charges an appropriate externality --- the mechanism maximizes the value of the highest-value bidder, then the value of the second-highest-value bidder, and so on. Moreover, this sequential maximization can be applied to any monotone functions of bidders' values, in contrast to quasilinear settings where only affine transformations (linear transformation of bidders' values) maintain incentive compatibility as per Roberts's theorem~\cite{roberts79}.

Many of these results come with a technical caveat about ties --- if a tie would occur in a continuous bid space, then agents will have an incentive to lie. This is an unavoidable consequence of the particular lexicographic form of bidders' preferences but happens very rarely, so we accept that those mechanisms will only be truthful ``almost everywhere'' over bidders' typespaces.


\paragraph{Value Maximizers, GSP, and Advertising} 

As a case study, we apply our fundamental results to online advertising, and learn key insights about the generalized second price (GSP) auction used in practice.
We first observe an ironic twist of fate: the auction (GSP) used in practice but derided as non-truthful in theory is in fact the incentive compatible externality pricing for value maximizers. This observation was first made by Aggarwal et al.~\cite{aggarwal09} who studied matching mechanisms (as a generalization of sponsored search auctions) under a class of valuations that included value maximizers. In our context, we observe that GSP is the special case of the ``welfare-maximizing'' auction for the standard sponsored search model.

Moreover, we take this observation a step further and suggest that GSP should be defined this way --- {\em GSP is the auction that is truthful for value maximizers with an ROI constraint}. %This definition allows us to generalize GSP while maintaining two key properties that are often cited: the price a bidder pays is the minimum bid required to maintain the same value, and the price can be uniquely attributed to the value a single competitor would have otherwise obtained.
%
Generalizing GSP in this way helps us solve a problem facing search engines today --- what should be done with complex ad types? Search ads today often come with many different features and in many different sizes, something that cannot be handled properly by a standard GSP auction. Our definition tells us what a GSP auction should do in these complex settings and how prices should be computed. %Moreover, if this version of GSP is unsatisfactory, it suggests a natural way to interpolate between GSP and VCG: construct a family of preferences that interpolate between quasilinear and value-maximizing, then run a truthful auction for a set of preferences in that family. We use the family of preferences used in our characterization theorems and discuss how they might be used for this purpose.


Finally, we discover that value-maximizing preferences are robust in a useful sense: {\em ROI constraints make almost any advertiser look like a value maximizer} under plausible constraints. We study the standard GSP auction for advertisers who have ``super-quasilinear'' preferences (roughly, anything between profit-maximizing and value-mazimizing preferences) and show that adding a sufficient ROI constraint makes that advertiser behave like a pure value maximizer as long as the available bundles of goods are sufficiently differentiated. Moreover, this is not merely a theoretical curiosity: based on data from Yahoo's Gemini Native advertising platform, we show that 80\% of auctions would be truthful under GSP pricing given only that advertisers required an $ROI>1$. This suggests that it may be reasonable in practice to assume that bidders are value maximizers.

\paragraph{Related Work}

The idea that agents maximize value is common. For example, the traditional studies of consumer choice and market equilibria begin with agents who pick the most-preferred bundle they can afford based on their endowment~\cite{mas-collel95}.

In the context of mechanism design, a limited literature studies non-quasilinear bidders.
%A preliminary work by Cavallo, Krishnamurthy, and Wilkens~\cite{cavallo15} focused on sponsored search; many results were precursors to this paper.
Concurrent work by Fadaei and Bichler introduce a similar model of ``value bidder''~\cite{fadaei16} and discuss a plethora of similar and interesting motivating examples, then study revenue maximization. Our model differs notably because we say bidders prefer lower prices when value is held constant, while Fadaei and Bichler imply bidders strictly prefer to spend their money.%; Fadaei and Bichler leave some ambiguity about bidders' preferences in such a setting, but their characterization of truthful mechanisms implies bidders strictly prefer to spend their full value rather than to have money left over.
%This distinction leads to substantially different pricing approaches --- whereas we design auctions resembling GSP, Fadaei and Bichler find that first-price auctions are truthful. We contend that bidders generally prefer lower prices, but there are circumstances when underspending may be undesirable, e.g. if it results in a smaller budget in the future.
Aggarwal et al.~\cite{aggarwal09} design sponsored search (slot) auctions for advertisers whose preferences add constraints on top of a quasilinear utility. While their general models are technically incomparable to ours, they do cover our value maximizers in the special case of sponsored search, and they make the observation that the truthful auction is simply GSP. Alaei et al.~\cite{alaei11} show how Walrasian equilibria in non-quasilinear unit-demand settings can be leveraged to build ad auctions where estimation errors break quasilinearity. A few papers study general truthful mechanisms for non-quasilinear preferences~\cite{adachi13,morimoto15}. These papers develop axiomatic characterizations of a VCG-analog for multi-unit and unit-demand settings.

A few threads within the qasilinear advertising literature are also related. One line of work studies the effect of using ROI to set bids across different auctions~\cite{borgs07,kitts04,szymanski08,zhou08,auerbach08}. Another line of work uses ideas from behavioral economics to capture observed behavior~\cite{rong14}. Finally, a small thread studies GSP and the problem of generalizing it to new contexts. The canonical analyses of GSP in a quasilinear world are~\cite{eos07,varian07}. Attempts to generalize GSP and consider its performance outside the standard model include~\cite{cavallo14,hummel14,abrams07,aggarwal06}.


==> native.tex <==


\section{Value Maximizers as ``Sink'' Type}  \label{sec:real}

Any ROI constraint makes a bidder look more like a simple value maximizer. For example, suppose that a bidder has an ROI constraint of 1 and has choices between an outcome $o$ with value $v_i(o)=1$ and an outcome $o'$ with value $v_i(o')=10$. At any price $p'\leq\$9$, a profit-maximizing bidder will prefer $o'$ to $o$; however, since bidder $i$ has an ROI constraint of 1, she will only consider outcome $o'$ when $p'\leq\$5$. As a result, any time $o'$ is cheap enough for her to consider it, she will always prefer it to outcome $o$ --- in this example, {\em bidder $i$ is effectively a simple value maximizer with value $v_i'=\frac12v_i$.}


More generally, when outcomes in an auction have dramatically different values, a bidder must pay a very high price before a lesser outcome (lower value) would become preferable. In such cases, a mild ROI constraint --- which caps the price an advertiser is willing to pay --- will push a bidder towards simple value maximizing behavior.

The ultimate effect of ROI constraints is surprising --- even if bidders are fundamentally profit-maximizers, a sufficient ROI constraint will make them value maximizers for all relevant purposes. To the degree that this is true, this again suggests that we should model advertisers as value maximizers for the purposes of designing auctions. In this section, we establish this phenomenon in theory, then show that it is very real in practice.

\subsection{General Valuations}

\begin{theorem}\label{thm:robust}
When bidders have super-quasi-linear preferences $\prec_i$, an ROI constraint $\gamma$, and
\[v_i(o)\frac{\gamma}{\gamma+1}\geq v_i(o')\mbox{ for all }v_i,o,o'\mbox{ where }v_i(o)>v_i(o')\enspace,\]
no bidder wishes to lie in an auction that is truthful, individually rational for value maximizers, and has no positive transfers.\footnote{No positive transfers means that the auctioneer never pays the bidders; individual rationality says that every bidder is at least as happy as if she had not participated at all.}
\end{theorem}
\begin{proof} Let $o$ and $p_i$ be the outcome and price that the bidder sees if it reports truthfully. Let $o'$ and $p_i'$ be any outcome and price that the bidder can achieve by lying.

First, suppose that $v_i(o')<v_i(o)$, i.e. bidder $i$ is lying to achieve an outcome with a lower value. Then we can use individual rationality
\[p_i(b)\leq\frac{v_i(x(b))}{\gamma+1}\]
and we know from no-positive-transfers that $p_i'\geq0$. Thus, by the conditions of the theorem, we know that
\[v_i(o)-p_i\geq v_i(o)\frac{\gamma}{\gamma+1}>v_i(o')\geq v_i(o')-p_i'\enspace.\]
In words, a profit-maximizing bidder prefers truthful reporting at the maximum individually-rational price to lying, even if $o'$ happened for free. Since bidder $i$ has super-profit-maximizing preferences and $v_i(o)>v_i(o')$, it follows $(v_i(o),p_i)\succ_i(v_i(o'),p_i')$.

Next, suppose that $v_i(o')=v_i(o)$. We know that the mechanism is truthful for value maximizers, so it must be that $p_i\leq p_i'$, otherwise a value maximizer would lie to achieve $o'$, $p_i'$. Since any super-quasi-linear bider will prefer $(v_i,p_i)$ to $(v_i,p_i')$ when $p_i\leq p_i'$, we can conclude that $(v_i(o),p_i)\succeq_i(v_i(o'), p_i')$.

Finally, suppose that $v_i(o')>v_i(o)$. Since the auction is truthful for value maximizers, we know that $p_i'>v_i(o')$, otherwise a value maximizer would lie to achieve $o'$, $p_i'$. By individual rationality we know $(v_i(o),p_i)\succeq_i(0,0)$ and any super-quasi-linear bidder prefers $(0,0)$ an outcome $o'$ at price $p'>v(o')$. Thus, $(v_i(o),p_i)\succeq_i(0,0)\succ_i(v_i(o'),p_i')$, so bidder $i$ will therefore prefer to tell the truth.
\end{proof}

\subsection{Empirical Analysis of Slot Auctions}

In advertising slot auctions, a profit-maximizer's relative value for two slots depends only on the likelihood of a click. Significantly, this gives us an easy way to test Theorem~\ref{thm:robust} in practice, since we can compare the likelihood of a click between slots. Formally, if we directly apply the theorem to an advertising slot auction we get the following corollary:
\begin{corollary}[of Theorem~\ref{thm:robust}]
If $\alpha_i\geq\frac{\gamma}{\gamma+1}\alpha_{i+1}$ for all $i$ in a standard sponsored search auction, then no bidder with super-quasi-linear preferences and a ROI constraint of $\gamma$ wishes to lie under GSP pricing.
\end{corollary}
This claim gives conditions under which no bidder has an incentive to lie, independent of other bidders' bids; however, reality may be even stricter. Given bids, we can ask a simpler question of whether any bidder could possibly prefer to lie under current marketplace conditions:
\begin{lemma}\label{lem:native-robust}
When no two bidders have the same score $\beta t$, and
\[\forall i,\; \frac{\alpha_i}{\alpha_i-\alpha_{i+1}}-\frac{\alpha_{i+1}}{\alpha_i-\alpha_{i+1}}\frac{\beta_{i+2}b_{i+2}}{\beta_{i+1}b_{i+1}}<\gamma\enspace,\]
no bidder with super-quasi-linear preferences and a ROI constraint of $\gamma$ wishes to lie under GSP pricing.
\end{lemma}
The proof (omitted) is similar to Theorem~\ref{thm:robust} and a version can be found in an earlier version of this work~\cite{cavallo15}.

We tested this lemma empirically by looking at bid data for the slot
auctions on Yahoo's homepage stream. We took a dataset consisting of over one
hundred thousand auctions from a brief period of time within a single day. Of
course it's impossible for us to know whether the submitted bids are reflective
of true values, but we can answer the following question: assuming bidders are
ROI constrained profit-maximizers, and assuming our empirically derived
estimates of parameters $\alpha$ and $\beta$ are correct, what is the minimum
value of $\gamma$ for which Lemma~\ref{lem:native-robust} says no bidder should lie, regardless of the precise form of their preferences?

Our results are striking --- if bidders require an ROI of 1, then 80\% of auctions would be such that no bidder can benefit by lying under GSP pricing. This strongly suggests that GSP may in fact be the appropriate auction for this setting. See Figure~\ref{fig:emp}.

\begin{figure}[h!]
\centering  
\hspace{-0mm}
\epsfxsize=3.5in \epsfbox{fig/natgsp.eps}
\caption{\label{fig:emp} Illustration of the proportion of auctions in which truthtelling is a best-response for every advertiser, given the bids of all others, assuming all bidders have a ROI constraint of $\gamma$. At $\gamma=1$, 80\% of auctions are such that nobody should lie; as $\gamma$ approaches 2, virtually all auctions satisfy Lemma~\ref{lem:native-robust}. This is derived from a dataset of auctions from Yahoo's homepage stream, in which slot advertisements are interspersed in a stream of rich content links.}
\vspace{-0mm}
\end{figure}





==> objectives.tex <==


\section{Advertisers and their Objectives}  \label{sec:obj}

We briefly introduced a handful of reasons that revenue maximization is a better model of an advertiser's preferences. We discuss those in detail here.

\subsection{Return on Investment (ROI) Constraints}

In marketing, the cost-benefit trade-off is generally measured by an advertiser's return on investment (ROI). Whereas profit measures the difference between value and cost, the ROI depends on the ratio. This somewhat small change results in manifestly different applications; ROI becomes a constraint instead of an objective, naturally leading advertisers to maximize revenue.

Profit is a standard objective in theory. For an agent with value $v$ who pays cost $p$, the profit is simply
\[Profit=v-p\enspace.\]
Profit maximization is consistent with standard quasi-linear utility functions ($u=v-p$) and is well-studied.

In contrast, advertisers usually measure ROI. Again considering an agent who gets value $v$ and pays price $p$, the ROI is given by
\[ROI=\frac{v-p}{p}=\frac{v}{p}-1\enspace.\]
Because ROI is a density measure (value per unit spend), it does not make sense to optimize for it directly; rather, ROI is manifested as a constraint.

Sponsored search illustrates the senslessness of optimizing for ROI. Note that an advertiser in sponsored search can get clicks at a very low price per click simply by being the lowest ad on the page; however, while this will maximize ROI, the advertiser will get very few clicks this way. This is not what advertisers want.


It remains to build preferences with ROI constraints. Since costs are already included through the ROI constraint, the most basic model says that an advertiser's objective should not depend on costs, i.e. the advertiser should maximize revenue. Thus, we argue that {\em value maximization with a ROI constraint} is the natural fundamental model for an anyone whose costs are primarily accounted for in ROI metrics.

That said, ROI constraints can be added to any model of preferences. As we will see later, these have 



\subsection{Budgets and Fiat Money}

Value maximization is a natural model when agents have no value for money, which is commonly true of marketers.

The standard model of quasi-linear preferences supposes that an agent gets utility from having unspent budget. This captures the idea that the bidder has outside options on which that money can be spent. (In our world with fiat money, money technically has no value beyond the fact that it can be spent on things.)

In contrast, an agent who prefers revenue does not care about how much money is left over insofar as constraints are not violated. Those constraints (ROI and budget) serve to make sure that the final outcome is acceptable to the advertiser.

In marketing, 



\subsection{Average-Centric Targets}

The metrics and tools used by advertisers correspond to revenue maximization, not profit maximization. A quick survey 

\begin{itemize}
\item Advertiser analysis tools universally report average costs
\item Yahoo
\item Google
\item ???
\end{itemize}


\subsection{Value Uncertainty}

The standard theory assumes 



==> proofs.tex <==
\section{Deferred Proofs.}\label{sec:proofs}

\begin{proof}[of Theorem~\ref{thm:vm-budget-char}.] Fix other bidders' values $v_{-i}$ and drop them for clarity.


{\em Necessity.} Fix a type $v_i$ and define
\[\mathcal{Z}^<=\{z|f(z)\prec_i^o f(v_i)\}\quad\mbox{and}\quad \mathcal{Z}^==\{z|f(z)\approx_i^o f(v_i)\}\]
to be the types that get a strictly less-preferred outcome to $f(v_i)$ and an equal outcome respectively. A value maximizer with budget $v_i$ will choose a bid $b_i$ that leads to the most preferred outcome subject to $p_i(b_i)\leq v_i$. Thus, for any $v_i$, $p_i(v_i)$ must be high enough that bidders who get a less-preferred outcome do not want to lie, i.e.
\[p_i(v_i)\geq \underline p_i\triangleq\sup \mathcal{Z}^<\enspace.\]
Similarly, all types who exactly get the outcome $f(v_i)$ must pay the same price, and it must be that any bidder who gets $x_i(v_i)$ must be willing to pay for it, so
\[p_i(v_i)\leq\overline p_i=\inf \mathcal{Z}^=\enspace.\]
Since $\sup\mathcal{Z}^<\geq\inf\mathcal{Z}^=$, it must be that $\underline p_i\geq\overline p_i$, and therefore to satisfy $\underline p_i\leq p_i(v_i)\leq \overline p_i$ a mechanism will be truthful if and only if $\underline p_i=\overline p_i=p_i(v_i)$ --- this happens if and only if $x$ is nondecreasing and is the price defined in the theorem.

{\em Sufficiency.} Note that for DSIC-AE we only need to prove sufficiency almost everywhere. We must consider three deviations: (1) a bidder underbids for a less-preferred outcome, (2) a bidder deviates for the same outcome at a lower price, and (3) a bidder overbids for a more-preferred outcome. Remark that deviation (1) will not happen because a value maximizer will always want the more-preferred outcome (since $p_i(v_i)\leq v_i$ by definition of $p_i$), and that  (2) cannot happen because all types who get the same allocation pay the same price.

It remains to show that bidders almost never have an incentive to raise a bid (3). Deviation (3) will only be beneficial if there exists a type $z>v_i$ such that $f(z)\succ_i^of(v_i)$ but $p_i(z)<v_i$. By definition of $p_i$, there exists a type $\underline b_i(z)\geq v_i$ such that
\[p_i(z)=\underline b_i(z)\enspace.\]
As long as $\underline b_i(z)>v_i$ this deviation cannot be beneficial. Unfortunately, when $b_i(z)=v_i$ then deviation (3) will be beneficial; however, this can only happen when $b_i(z)$ is a threshold at which the outcome changes. Since we assumed the outcome space to be countable, we get truthfulness in our almost-everywhere sense (DSIC-AE).
\end{proof}

==> roberts-proof-bkp-bkp.tex <==


\section{A ``Roberts's Theorem'' Proof for Value Maximizers}  \label{sec:roberts-proof}

Recap setup...
\begin{itemize}
\item Vector space $\U$ with addition $\oplus$ and subtraction $\ominus$.
\item outcome set $\O$ with $|\O|=m$, indexed by $j$
\item $n$ bidders with a value $v_i^j\in\U$ for item $j$ and utilities $u_i=v_i-p_i$
\item Define the notation $\delta^o,\epsilon^o\in\U^{mn}$ where all entries for $o$ are $\delta$ (respectively $\epsilon$) and other entries are 0, i.e.
\[\delta_i^{o_1}(o)=\begin{cases}
\delta&o=o_1\\
0&\mbox{otherwise.}
\end{cases}\]
\end{itemize}

%\subsection{DSIC}
%
%In order to deal with ``ties'' we introduce a map that (intuitively) identifies ``all reasonable outcomes for valuations $v$'':
%
%\begin{definition}
%The map extension $\bar f$ of a social choice function $f$ is the multi-valued map where $o\in \bar f(v)$ if and only if there is a sequence of values ${}^1v, {}^2v,\dots, {}^kv,\dots$ for which $f({}^kv)=o$ and the sequence converges to $v$.
%\end{definition}
%\begin{observation}
%\[f(v)\in \bar f(v)\]
%\end{observation}
%\begin{proof}
%Consider the sequence with ${}^kv=v$.
%\end{proof}
%
%We want to talk about when a map represents an affine maximizer. We frame it slightly differently, in terms of a linear function with an offset:
%\begin{definition}
%Let $g:\U^{nm}\rightarrow 2^{m}$ be a multi-valued map from $n$ valuation vectors to outcomes in $\O$. We say that the map $g$ {\em maximizes a linear function $h$} if
%\[g(v)=\argmax_j h(v^j)\enspace.\]
%We say that a map $g$ {\em maximizes a linear function $h$ with offset $c\in\U^{mn}$} if
%\[g(v)=\argmax_j h(v^j\ominus c^j)\enspace.\]
%We say that a function $f$ is a linear maximizer for $h$ (possibly with offset $c$) if $f\in g$.
%\end{definition}
%
%\begin{observation}
%A linear function $h$ with offset $c$ is equivalent to an affine maximizer.
%\end{observation}
%\begin{proof}
%By linearity, maximizing $h(v^j\ominus c^j)$ is equivalent to maximizing $h(v^j)\oplus h(c^j)$.
%\end{proof}
%
%Our first lemma gives us a concrete condition we can test to see if there is some linear function $h$ that is being maximized by a particular function or map:
%
%\begin{lemma}
%A multi-valued map $g$ maximizes some linear function $h$ with offset $c$ if and only if $g$ is upper hemicontinuous(? is this the right thing here?) and
%\[o\in g(v),g(v')\Rightarrow o\in g(v\oplus v'\ominus c)\]
%for some $c\in\U^{nm}$ and all $o$, $v$, and $v'$.
%\end{lemma}
%
%\begin{proof} {\em Only if.} Suppose that $g$ maximizes a linear function $h$ with offset $c$. Suppose that $o_1\in g(v),g(v')$ for some $v$ and $v'$. For any $o_2\neq o_1$, this implies $h(v(o_1)\ominus c(o_1))\geq h(v(o_2)\ominus c(o_2))$. By linearity of $h$ this implies $h(v(o_1))\oplus h(c(o_1)\geq h(v(o_2))\oplus h(c(o_2)$. Repeating for $v'$ gives $h(v'(o_1))\oplus h(c(o_1)\geq h(v'(o_2))\oplus h(c(o_2)$. Adding these together and leveraging linearity we have
%\[h((v(o_1)\oplus v'(o_1)\ominus c(o_1))\ominus c(o_1))\geq h((v(o_2)\oplus v'(o_2)\ominus c(o_2))\ominus c(o_2))\enspace.\]
%Since this is true for all $o_2\neq o_1$ we can conclude that $o_1\in g(v\oplus v'\ominus c)$.
%
%{\em If.} We must construct $h$. \textbf{Speculation: Upper hemicontinuity implies }
%
%we build it up as follows:
%\begin{enumerate}
%\item $h(x_1,0,\dots,0)=x_1$.
%\item $h(\dots,0,x_i,0,\dots)=\inf$
%\end{enumerate}
%\textbf{TODO.}
%
%\end{proof}
%
%
%
%\begin{claim}
%Let $f$ be the social choice function of a truthful mechanism for bidders with generalized utility functions $u_i(v_i,j,p_i)=v_i^j-p_i$ and $\bar f$ its map extension, then there exists a $c\in\U^{mn}$ such $\bar f(c)=\O$.
%\end{claim}
%\begin{proof}
%Set $v_{-1}=0$. By the taxation principle, we can write a price $p_1^j\in\U$ for each outcome. Take $c_1=p_1$ and $c_{-1}=0$.
%
%To prove that an outcome $o\in\bar f(c)$, we must exhibit a sequence of values converging to $c$. Remark that if $v_1=p_1$, then a quasilinear bidder is indifferent among all outcomes.  Thus, if we define ${}^kv_1^j$
%\[{}^kv_1^j=\begin{cases}
%p_1^j+{}^k\epsilon&j=o\\
%p_1^j&\mbox{otherwise}
%\end{cases}\]
%where $\{{}^k\epsilon\}$ is some sequence of values in $\U$ that converge to 0.
%we have that bidder 1 strictly prefers outcome 1 and therefore $f({}^kv_1,0)=o$ for every $k$. Thus, $o\in\bar f(c)$.
%\end{proof}
%
%\begin{claim}[PAD]
%Let $v$ be such that $f(v)=o_1$ and $v'$ such that for all $i$, and $o_2\neq o_1$, $v_i'(o_1)\ominus v_i(o_1)>v_i'(o_2)\ominus v_i(o_2)$. Then $f(v')=o_1$.
%\end{claim}
%\begin{proof}
%\textbf{Standard.}
%\end{proof}
%\begin{corollary}
%Let $v$ be such that $o_1\in\bar f(v)$ and $v'$ such that for all $i$, and $o_2\neq o_1$, $v_i'(o_1)\ominus v_i(o_1)>v_i'(o_2)\ominus v_i(o_2)$. Then $o_1\in\bar f(v')$.
%\end{corollary}
%\begin{proof}
%By definition of $\bar v$, there exists a $v''$ sufficiently close to $v$ for which $f(v'')=o_1$ that we can apply PAD to $v'$ and $v''$.
%\end{proof}
%
%\begin{corollary}
%Let $v$ be such that $f(v)=o_1$. Construct $v'$ as
%\[v_i'(o)=\begin{cases}
%v_i'(o)\oplus \epsilon_i&o=o_1\\
%v_i'(o)&\mbox{otherwise}
%\end{cases}\]
%where $\epsilon_i>0$. Then:
%\begin{enumerate}
%\item $f(v')=o_1$.
%\item There exists $\epsilon'$ such that for any $v''$ within the $\epsilon'$ ball centered at $v'$, $f(v'')=o_1$.
%\item $\bar f(v')=\{o_1\}$.
%\end{enumerate}
%\end{corollary}
%\begin{proof}
%(1) follows immediately from PAD. (2) follows because there is an $\epsilon'$ small enough that PAD applies to any $v''$ within the $\epsilon'$ ball around $v'$. (3) follows because if $f(v'')=o_1$ for all points in the $\epsilon'$ ball of (2), there can be no sequence converging to $v'$ for which $f\neq o_1$.
%\end{proof}
%
%\begin{claim}[NAD]
%Let $v$ be such that $o_1\not\in\bar f(v)$ and $v'$ such that for all $i$, and $o_2\neq o_1$, $v_i'(o_1)\ominus v_i(o_1)<v_i'(o_2)\ominus v_i(o_2)$. Then $o_1\not\in\bar f(v')$.\end{claim}
%\begin{proof}
%\textbf{TODO.}
%\end{proof}
%
%\begin{claim}
%Let $c$ be such that $\bar f(c)=\O$, and let $o_1$, $v$, and $v'$ be such that $o_1\not\in\bar f(v), \bar f(v')$. Then $o_1\not\in\bar f(v\oplus v'\ominus c)$.
%\end{claim}
%\begin{proof}
%\textbf{TODO.}
%\begin{enumerate}
%\item Pick an outcome $o''\neq o,o'$. Let $\delta=v^o\ominus v^{o'}$ and $\delta'=v'^o\ominus v'^{o'}$.
%\item Construct a valuation vector $x$ where $x^o\ominus x^{o''}$ is $\delta$. Use Lavi claim 3 reasoning from $c$ and $v$ to argue that $o''\not\in \bar f(x)$.
%\item Construct a valuation vector $y$ where $y^{o''}\ominus y^{o'}=\delta'$. Use Lavi claim 3 reasoning from $c$ and $v'$ to argue that $o'\not\in\bar f(y)$.
%\item Construct a valuation vector $z$ where $z^{o}\ominus z^{o'}=\delta\oplus\delta'$. Use Lavi claim 3 reasoning from $x$ and $y$ to argue that $o'\not\in\bar f(z)$.
%\item Use Lavi claim 1 reasoning from $z$ to say that $o'\not\in\bar f(v\oplus v'\ominus c)$.
%\end{enumerate}
%\textbf{Note 0: For intuition about using the vector $c$ in (b) and (c), imagine $c=0$, then these are basically the same as step (1) of the informal sketch in Lavi et al.}
%
%\textbf{Note 1: Consistent with Lavi reasoning, there will probably be some epsilons added. I'm not sure exactly where.}
%
%\textbf{Note 2: Ideally, the three invocations of Lavi logic could be condensed by understanding exactly which points were being compared.}
%\end{proof}
%
%
%\begin{lemma}
%Let $f$ be the social choice function of a truthful mechanism for bidders with generalized utility functions $u_i(v_i,j,p_i)=v_i^j-p_i$ and $\bar f$ its map extension, then there exists a $c\in\U^{mn}$ such that
%\[o\in\bar f(v),\bar f(v')\Rightarrow o\in \bar f(v\oplus v'\ominus c)\enspace.\]
%\end{lemma}
%
%\begin{proof}\textbf{TODO: write the proof.}
%...here's the way I think it goes...
%
%\textbf{First, think: Lavi claim 3 is a kind of transitivity...if you didn't take $o'$ when the difference between $o$ and $o'$ was $v^o-v^{o'}=\delta$ and you also didn't take $o''$ when the difference between $o'$ and $o''$ was $v^{o'}-v^{o''}=\delta'$, then you won't take $o''$ when $v^o-v^{o''}=\delta+\delta'$.}
%\begin{enumerate}
%\item Let $c$ be such that $\bar f(c)=\O$.
%\item Pick any $o_1$, $v$ and $v'$ such that $o_1\in\bar f(v),\bar f(v')$.
%\item Pick a sequence $\{{}^k\epsilon\}$ of positive values converging to zero. For each ${}^k\epsilon$...
%\begin{enumerate} 
%\item Add ${}^k\epsilon$ to $v_i(o_1)$ and $v_i'(o_1)$ for every $i$. Call the results $w$ and $w'$, and let ${}^ks=w\oplus w'\ominus c$.
%\item By claim~\ref{clm:???} it follows that $\{o_1\}=f(w)=\bar f(w')$.
%\item By claim~\ref{clm:???} it follows that $o_2\not\in\bar f({}^ks)$ for any $o_2\neq o_1$.
%\item Since $\bar f$ must contain $f$ and cannot contain any $o_2\neq o_1$, it must be that $f({}^ks)=o_1$.
%\end{enumerate}
%\item The sequence $\{{}^ks\}$ converges to $v\oplus v'\ominus c$ and has $f({}^ks)=o_1$, implying $o_1\in\bar f(v\oplus v'\ominus c$ as desired.
%\end{enumerate}
%
%
%\end{proof}
%
%\begin{corollary}
%If $f$ is DSIC, then $f$ is a linear maximizer for some function $h$ with some offset $v_0$.
%\end{corollary}

\subsection{DSIC 2}

\subsection{``Affine Maximizers''}

We want to talk about when a map represents an affine maximizer. We frame it slightly differently, in terms of a linear function with an offset:
\begin{definition}
Let $g:\U^{nm}\rightarrow 2^{m}$ be a multi-valued map from $n$ valuation vectors to outcomes in $\O$. We say that the map $g$ {\em maximizes a linear function $h$} if
\[g(v)=\argmax_o h(v(o))\enspace.\]
We say that a map $g$ {\em maximizes a linear function $h$ with offset $c\in\U^{mn}$} if
\[g(v)=\argmax_o h(v(o)\ominus c(o))\enspace.\]
We say that a function $f$ is a linear maximizer for $h$ (possibly with offset $c$) if $f\in g$.
\end{definition}

\begin{observation}
A linear function $h$ with offset $c$ is equivalent to an affine maximizer.
\end{observation}
\begin{proof}
By linearity, maximizing $h(v(o)\ominus c(o))$ is equivalent to maximizing $h(v(o))\ominus h(c(o))$.
\end{proof}

Our first lemma gives us a concrete condition we can test to see if there is some linear function $h$ that is being maximized by a particular function or map:

\begin{lemma}
A multi-valued map $g:\U^{mn}\rightarrow 2^\O$ maximizes some linear function $h$ with offset $c$ if and only if $g$ is nonempty, upper hemicontinuous, and satisfies the following for some $c\in\U^{nm}$:
\begin{enumerate}
\item $g(c)=\O$,
\item \label{itm:cond-mon} $o_1\in g(v)\Rightarrow \{o_1\}=g(v\oplus \epsilon^{o_1})$ for any $\epsilon>0$,
\item \label{itm:cond-diff} $g(v)=g(v\oplus(\delta,\dots,\delta))$ for any $\delta\in\U^n$ (adding the same thing to every outcome), and
\item\label{itm:cond-add} $g(v)= g(v')\Rightarrow g(v\oplus v'\ominus c)=g(v)= g(v')$
%for any $o$, the image $\mathcal I(o)=\{v|o\in g(v)\}$ is convex and the interiors of the images $\mathcal I(o)$ are disjoint.
\end{enumerate}
\end{lemma}

\begin{proof} {\em Only if.} Suppose that $g$ maximizes a linear function $h$ with offset $c$. It is easy to see that $g$ is nonempty and upper hemicontinuous. We argue the other four facts:
\begin{enumerate}
\item For every outcome $o$, we have $h(c(o)\ominus c(o))=h(0)$ and thus $\O=\argmax_o h(c(o)\ominus c(o)$.
\item Suppose that $o_1\in g(v)$.  For any $o_2\neq o_1$, this implies $h(v(o_1)\ominus c(o_1))\geq h(v(o_2)\ominus c(o_2))$, which implies $h(v(o_1)\oplus\epsilon\ominus c(o_1))> h(v(o_2)\ominus c(o_2))$ and therefore $o_2\not\in g(v\oplus\epsilon^{o_1})$. Repeating for every $o_2$ and using the nonemptyness of $g$ implies $g(v\oplus \epsilon^{o_1})=\{o_1\}$.
\item If we add $\delta$ to every outcome, we maximize $h(v(o)\oplus\delta\ominus c)=h(v(o)\ominus c)\oplus h(\delta)$, which is the same as maximizing $h(v(o)\ominus c)$.
\item Suppose that $o_1\in g(v),g(v')$ for some $v$ and $v'$. For any $o_2\neq o_1$, this implies $h(v(o_1)\ominus c(o_1))\geq h(v(o_2)\ominus c(o_2))$ and $h(v'(o_1)\ominus c(o_1))\geq h(v'(o_2)\ominus c(o_2))$. By linearity we have
\[h((v(o_1)\oplus v'(o_1)\ominus c(o_1))\ominus c(o_1))\geq h((v(o_2)\oplus v'(o_2)\ominus c(o_2))\ominus c(o_2))\enspace.\]
Since this is true for all $o_2\neq o_1$ and $g$ is nonempty we can conclude that $o_1\in g(v\oplus v'\ominus c)$. Analogous reasoning shows that $o_1\not\in  g(v\oplus v'\ominus c)$ when $o_1\not\in g(v)\cap g(v')$ but $o_2\in g(v),g(v')$. 
\end{enumerate}

{\em If.} Given $c$ we must construct $h$. Let $\mathcal I(o)=\{v|o\in g(v)\}$ be the image of $o$. We construct $h$ as follows:
\begin{enumerate}
\item[(a)] {\em $\mathcal I(o)$ is convex.} Let $x,y\in\U^{mn}$ be such that $g(x)=g(y)$. Applying condition~(\ref{itm:cond-add}) to $v=x$ and $v'=y$ says that $g(x\oplus y\ominus c)=g(v)=g(v')$. Moreover, applying the equation to $v=v'=\frac12(x+y)$ implies $g(\frac12(x+y))=g(x\oplus y\ominus c)=g(v)=g(v')$.

\item[(b)] {\em For any distinct $o_1,o_2$, the interiors of $\mathcal I(o_1)$ and $\mathcal I(o_2)$ are disjoint.} For contradiction, assume that there is a $v$ in the interior of $\mathcal I(o_1)$ such that $o_1,o_2\in g(v)$. Condition~(\ref{itm:cond-mon}) implies that $g(v\oplus \epsilon^{o_2})=\{o_2\}$. However, since $v$ is in the interior of $\mathcal (o_1)$, it follows that $v\oplus\epsilon^{o_2}$ is also in the interior for sufficiently small $\epsilon$, implying $o_1\in g(v\oplus\epsilon^{o_2})$. This is a contradiction.

\item[(c)] {\em For any distinct $o_1, o_2$, the sets $\mathcal I(o_1)$ and $\mathcal I(o_2)$ are separated by a hyperplane through $c$ defined by a linear function $H_{o_1,o_2}(x)$.} \textbf{Check on this...} Remark that $c\in\mathcal I(o)$ for all $o$, so $c$ must be on the boundary of all the $\mathcal I$ sets and a separating hyperplane must pass through it. A hyperplane through $c$ is defined by a linear function $H_{o_1,o_2}:\U^{mn}\rightarrow\U$ where $H_{o_1,o_2}(v\ominus c)$ is positive on one side of the hyperplane and negative on the other side.

\item[(d)] {\em Pick any distinct $o_1,o_2$ and take $h(x)=H_{o_1,o_2}(x, 0,\dots, 0)$. $g$ maximizes $h$ with offset $c$.} Suppose not, that is, there exists $v$ such that $g(v)\neq\argmax_o h(v(o)\ominus c(o))$. First suppose that $o_1\in g(v)$ but $o_1\not\in\argmax h(v(o)\ominus c(o))$. If $o_2\in g(v)$, this implies $h(v(o_1)-c(o_1))<4$


$h_{12}>0\cap h_{23}>0\Rightarrow h_{13}>0$

$dh_{12}(x(o_1)\ominus x(o_2,\dots,o_m))=a(x(o_1))\ominus b(x(o_2,\dots,o_m))$

\item[(d)] {\em All the $h_{o_1,o_2}$ are the same; pick any one as $h$.} Pick any $o_1$ and $o_2\neq o_1$. Let $h(x)=h_{o_1,o_2}(x)$. Clearly, 

\end{enumerate}

\end{proof}



\subsection{Consequences of IC}


\begin{definition}
For valuation profiles $v$ and $v'$ define $S_{\rightarrow}(v,v')$ as the set of valuation profiles progressively changing entries from $v$ to $v'$, i.e.
\[S(v,v')=\{v, (v'_1, v_2,\dots, v_n), (v'_1, v'_2, v_3,\dots, v_n), (v'_1,\dots, v'_{n-1}, v_n), v'\}\]
 
\end{definition}




\begin{claim}[PAD] Let $f$ be the social choice function of a mechanism $M$ and let $v$ be such that $f(v)=o_1$ and $v'$ such that for all $i$, and $o_2\neq o_1$, $v_i'(o_1)\ominus v_i(o_1)>v_i'(o_2)\ominus v_i(o_2)$. If truth-telling is a best response for every bidder in any valuation profile from $S_\rightarrow(v,v')$, then $f(v')=o_1$.
\end{claim}
\begin{proof}
By induction. Let $v^k$ be the valuation profile in which the first $k$ agents have values from $v'$ and the remaining $n-k$ have values from $v$, i.e.
\[v^k=(v'_1,\dots, v'_k, v_{k+1},\dots,v_n)\enspace.\]
By the conditions of the lemma $f(v^0)=o_1$. Suppose that $f(v^{k-1})=o_1$ and consider the preferences of bidder $k$ under $v'$. Invoke the taxation principle to write $p_k(o)$ as the price $k$ pays if the outcome is $o$ given $v_{-k}^{k}=v_{-k}^{k-1}$. Since $f(v^{k-1})=o_1$ we know that $v_k(o_1)-p_k(o_1)\geq v_k(o_2)-p_k(o_2)$ for any outcome $o_2\neq o_1$. Moreover, by the conditions of the lemma, we can assert that $v'_k(o_1)-v_k(o_1)> v'_k(o_2)-v_k(o_2)$ and therefore  $v'_k(o_1)-p_k(o_1)> v'_k(o_2)-p_k(o_2)$, implying that bidder $k$ strictly prefers outcome $o_1$ to any other outcome. This implies $f(v^k)=o_1$. Thus, by induction, we have $f(v')=f(v^n)=o_1$.
\end{proof}

\begin{claim}[NAD] Let $f$ be the social choice function of a mechanism $M$ and let $v$ be such that $o_1\neq f(v)$ and $v'$ such that for all $i$, and $o_2\neq o_1$, $v_i'(o_1)\ominus v_i(o_1)<v_i'(o_2)\ominus v_i(o_2)$. If no bidder has an incentive to lie when the valuation vector is any point in $S_\rightarrow(v,v')$, then $o_1\neq f(v')$.\end{claim}
\begin{proof}
By induction. Let $v^k$ be the valuation profile in which the first $k$ agents have values from $v'$ and the remaining $n-k$ have values from $v$, i.e.
\[v^k=(v'_1,\dots, v'_k, v_{k+1},\dots,v_n)\enspace.\]
By the conditions of the lemma $o_1\neq  f(v^0)$. Assume that $o_1\not\in f(v^{k-1})$ and consider the preferences of bidder $k$ under $v'$. Invoke the taxation principle to write $p_k(o)$ as the price $k$ pays if the outcome is $o$ given $v_{-k}^{k}=v_{-k}^{k-1}$. Since $f(v^{k-1})\neq o_1$ we know that $v_k(o_1)-p_k(o_1)\leq v_k(f(v^{k-1}))-p_k(f(v^{k-1}))$. Moreover, by the conditions of the lemma, we can assert that $v'_k(o_1)-v_k(o_1)< v'_k(o_2)-v_k(o_2)$ and therefore  $v'_k(o_1)-p_k(o_1)< v'_k(f(v^{k-1}))-p_k(f(v^{k-1}))$, implying that bidder $k$ strictly prefers outcome $f(v^{k-1})$ to $o_1$. This implies $f(v^k)\neq o_1$. Thus, by induction, we have $f(v')=f(v^n)\neq o_1$.
\end{proof}


\begin{lemma}\label{lem:f-add}
Let $c$ be such that $f(c\oplus \epsilon^o)=o$ for any $o$ and $\epsilon>0$, and let $o_1$, $v$, and $v'$ be such that $o_1=f(v)=f(v')$. Assuming $M$ is DSIC, then
\[o_1= f(v\oplus v'\ominus c\oplus 6\epsilon^{o_1})\]
for any $\epsilon\geq 0$.

Additionally, we can relax the DSIC requirement --- there exists a finite set of points $S_{\ref{lem:f-add}}(v,v',c,\epsilon)\subseteq \U^{mn}$ such that the lemma holds as long as truth-telling is a best-response for all bidders at all points in $S$.

\end{lemma}
\begin{proof}
Fix an $o_2$. We repeatedly apply PAD and NAD to show that $f(v\oplus v'\ominus c)\neq o_2$.
\begin{enumerate}
\item Pick outcomes $o_2,o_3\neq o_1$ and fix $\epsilon$.
\item Define the valuation profile $x$ by 
\[x_i(o)=\begin{cases}
v_i(o)\oplus 2\epsilon&o=o_1\\
v_i(o)\oplus\epsilon&o=o_2\\
v_i(o_2)\oplus c_i(o_3)\ominus c_i(o_2)&o=o_3\\
v_i(o)&\mbox{otherwise.}
\end{cases}\]
NAD implies $f(x)=o_1$. Specifically, NAD using $c\oplus\epsilon^{o_2}$ and $x$ implies that outcome $o_2$ is preferred to outcome $o_3$ and therefore $f(x)\neq o_3$ (recall that by assumption $f(c\oplus\epsilon^{o_2})=o_2$). NAD using $v$ and $x$ implies that outcome $o_1$ is preferred to all remaining outcomes, i.e. $f(x)\neq o_2$ and $f(x)\neq o'$ for any $o'\not\in\{o_1,o_2,o_3\}$.

\item Define the valuation profile $x'$ by 
\[x'_i(o)=\begin{cases}
v'_i(o)\oplus\epsilon&o=o_1\\
v'_i(o)&o=o_2\\
v'_i(o_1)\oplus c_i(o_3)\ominus c_i(o_1)\oplus2\epsilon&o=o_3\\
v'_i(o)&\mbox{otherwise.}
\end{cases}\]
NAD implies $f(x')=o_3$. Specifically, NAD using $c\oplus\epsilon^{o_3}$ and $x'$ implies that outcome $o_3$ is preferred to outcome $o_1$ and therefore $f(x)\neq o_1$ (recall that by assumption $f(c\oplus\epsilon^{o_3})=o_3$). NAD using $v'$ and $x$ implies that outcome $o_1$ is preferred to all remaining outcomes, i.e. $f(x)\neq o_2$ and $f(x)\neq o'$ for any $o'\not\in\{o_1,o_2,o_3\}$.

\item Define the valuation profile $y$ by
\[y_i(o)=\begin{cases}
v_i(o)\oplus v_i'(o)\ominus c_i(o)\oplus5\epsilon&o=o_1\\
v_i(o)\oplus v_i'(o)\ominus c_i(o)&o=o_2\\
v'_i(o_1)\oplus v_i(o_2)\ominus c_i(o_1)\oplus c_i(o_3)\ominus c_i(o^2) \oplus 2\epsilon&o=o_3\\
v_i(o)\oplus v_i'(o)\ominus c_i(o)&\mbox{otherwise.}
\end{cases}\]
NAD implies $f(y)=o_1$. Specifically, NAD using $x$ and $y$ implies that outcome $o_1$ is preferred to outcome $o_3$ and therefore $f(x)\neq o_1$. NAD using $v$ and $x$ implies that outcome $o_2$ is preferred to all remaining outcomes, i.e. $f(x)\neq o_2$ and $f(x)\neq o'$ for any $o'\not\in\{o_1,o_2,o_3\}$.

\item Define the valuation profile $z$ by
\[z_i(o)=\begin{cases}
v_i(o)\oplus v_i'(o)\ominus c_i(o)\oplus6\epsilon&o=o_1\\
v_i(o)\oplus v_i'(o)\ominus c_i(o)&\mbox{otherwise.}
\end{cases}=v\oplus v'\ominus c\oplus 6\epsilon^{o_1}\]
NAD with $y$ and $z$ implies that $o_1$ is preferred to $o_2$ and therefore $f(z)\neq o_2$.
\end{enumerate}

Repeating this logic for every $o_2\neq o_1$ implies that $f(v\oplus v'\ominus c\oplus6\epsilon^{o_1})=o_1$.
\end{proof}


%\begin{corollary}
%Let $c$ be such that $f(c\oplus \epsilon^o)=o$ for any $o$ and $\epsilon>0$, and let $o_1$, $v$, and $v'$ be such that $o_1=f(v)=f(v')$. Assuming $M$ is DSIC, then
%\[o_1= f\left(\frac12(v\oplus v')\oplus7\epsilon^{o_1}\right)\]
%for any $\epsilon\geq 0$.
%
%Additionally, we can relax the DSIC requirement --- there exists a finite set of points $S\subseteq \U^{mn}$ such that the lemma holds as long as truth-telling is a best-response for all bidders at all points in $S$. Moreover...
%\end{corollary}
%\begin{proof}
%By the lemma, $f(v\oplus v'\ominus c\oplus6\epsilon^{o_1})=o_1$. For contradiction, suppose that
%\[f\left(\frac12(v\oplus v')\oplus3(\epsilon^{o_1}-\epsilon^{o_2})\right)=o_2\neq o_1\enspace.\]
%Then applying the lemma we can conclude that $f(v\oplus v'\ominus c\oplus6\epsilon^{o_1})=o_2$, a contradiction.
%
%By NAD, we can then conclude that 
%\[o_1= f\left(\frac12(v\oplus v')\oplus7\epsilon^{o_1})\right)=o_1\enspace.\]
%The claims about $S_{\ref{lem:f-add}}$ follow by inspection of the proof --- it invokes PAD and NAD (each which require best-responses at points in a finite set $S_\rightarrow$) a finite number of times.
%\end{proof}


\subsection{DSIC}

In order to deal with ``ties'' we introduce a map that (intuitively) identifies ``all reasonable outcomes for valuations $v$'':

\begin{definition}
The map extension $\bar f$ of a social choice function $f$ is the multi-valued map where $o\in \bar f(v)$ if and only if there is a sequence of values $v^1, v^2,\dots, v^k,\dots$ for which $f(v^k)=o$ and the sequence converges to $v$.
\end{definition}
\begin{observation}
$\bar f$ is nonempty and upper hemicontinuous. Moreover, $f(v)\in \bar f(v)$.
\end{observation}
\begin{proof}
It is upper hemicontinuous by construction. For the claim about nonemptyness and $f(v)$, consider the sequence with $v^k=v$.
\end{proof}
\begin{observation}
If $f=o_1$ for all points in an $\epsilon$ ball around $v$ for a fixed $\epsilon$, then $\bar f(v)=\{o_1\}$.
\end{observation}

\begin{claim}[Extended PAD]
Let $f$ be the social choice function of a truthful mechanism for bidders with generalized utility functions $u_i(v_i,o,p_i)=v_i(o)-p_i$ and $\bar f$ its map extension, then $o_1\in\bar f(v)\Rightarrow \{o_1\}=\bar f(v\oplus \epsilon^{o_1})$. \textbf{Can be generalized to be parallel to PAD if necessary...}
\end{claim}
\begin{proof}
By definition of $\bar f$, there exists a value $v'$ in the $\frac12\epsilon$-ball around $v$ such that $f(v')=o_1$. Applying PAD to $v'$ all points in an $\frac12\epsilon$ ball around $v\oplus\epsilon^{o_1}$ implies that $f=o_1$ for all points in the ball and thereby $\{o_1\}=\bar f(v\oplus \epsilon^{o_1})$.
\end{proof}



\begin{claim}
Let $f$ be the social choice function of a truthful mechanism for bidders with generalized utility functions $u_i(v_i,o,p_i)=v_i(o)-p_i$ and $\bar f$ its map extension, then there exists a $c\in\U^{mn}$ such $\bar f(c)=\O$.
\end{claim}
\begin{proof}
Set $v_{-1}=0$. By the taxation principle, we can write a price $p_1(o)\in\U$ for each outcome $o$. Take $c=(p_1, v_{-i})$. Clearly, bidder 1 is indifferent among all outcomes at $c$, so if we increase agent 1's value for outcome $o_1$ by $\epsilon$ (i.e. set $c'_1(o_1)=p_1(o_1)\oplus\epsilon$) then we must have a point $c'$ where $f(c')=o_1$. Taking a sequence of $\epsilon$ that converge to 0 implies that $o_1\in\bar f(c)$; repeating for all $o$ shows $\bar f(c)=\O$.
\end{proof}


\begin{claim}
Let $f$ be the social choice function of a truthful mechanism for bidders with generalized utility functions $u_i(v_i,o,p_i)=v_i(o)-p_i$ and $\bar f$ its map extension, then $\bar f(v)=\bar f(v\oplus(\delta,\dots,\delta))$ for any $\delta\in\U^n$.
\end{claim}
\begin{proof}
Pick any $o_1\in\bar f(v)$. If $f(v)=o_1$, then by extended PAD, $f(v\oplus(\delta,\dots,\delta)\oplus\epsilon^{o_1})$ for any $\epsilon>0$. If $f(v)=o_1$, then for any 
\end{proof}


\begin{claim}
Let $f$ be the social choice function of a truthful mechanism for bidders with generalized utility functions $u_i(v_i,o,p_i)=v_i(o)-p_i$ and $\bar f$ its map extension, and $c$ satisfying $\bar f(c)=\O$, then $\bar f(v)= \bar f(v')\Rightarrow \bar f(v\oplus v'\ominus c)=\bar f(v)= \bar f(v')$
\end{claim}
\begin{proof}
First, we show that $o_1\in \bar f(v)\cap \bar f(v')\Rightarrow o_1\in \bar f(v\oplus v'\ominus c)$. By definition of $\bar f$, there are sequences $v^k$ and $v'^k$ that converge to $v$ and $v'$ respectively and have $f=o_1$ at every point in the sequence. By Lemma~\ref{lem:f-add} we know that $f(v^k\oplus v'^k\ominus c\oplus 6\epsilon^{o_1})=o_1$. This is a sequence converging to $v\oplus v'\ominus c$, implying $o_1\in\bar f(v\oplus v'\ominus c)$.

The other direction we need to argue is that if $o_1\not\in\bar f(v), \bar f(v')$ but t$\bar f(v)\cap\bar f(v')$, then $o_1\not\in\bar f(v\oplus v'\ominus c)$. Pick an $\epsilon$ sufficiently small that $f(x)\in\bar f(v)$ for every $x$ in the $2n\epsilon$ ball around $v$. Let $o_2=f(v\oplus\frac12\epsilon^{o_1}\ominus\frac12\epsilon^{o_2})\in\bar f(v)$.  Since $\bar f(v)=\bar f(v')$, there is an $x'$ arbitrarily close to $v'$ such that $f(x')=o_2$. Applying Lemma~\ref{lem:f-add} with $\epsilon'=\frac1{12}\epsilon$ implies that $f(v\oplus x'\ominus c\oplus \frac12\epsilon^{o_1})=o_2$. NAD then implies that $f(v\oplus v'\ominus c)\neq o_1$ and, moreover, that $f(y)\neq o_1$ for any in a sufficiently small ball around $v\oplus v'\ominus c$. By consequence we can conclude that $o_1\not\in \bar f(v\oplus v'\ominus c)$.

\end{proof}



\begin{lemma}
If $f$ is DSIC, then $f$ is a linear maximizer for some function $h$ with some offset $v_0$.
\end{lemma}
\begin{proof}
\begin{enumerate}
\item $g(c)=\O$,
\item $g(v)=g(v\oplus(\delta,\dots,\delta))$ for any $\delta\in\U^n$ (adding the same thing to every outcome), and
\item\label{itm:cond-3} $g(v)\cap g(v')\neq\emptyset\Rightarrow g(v\oplus v'\ominus c)=g(v)\cap g(v')$
%for any $o$, the image $\mathcal I(o)=\{v|o\in g(v)\}$ is convex and the interiors of the images $\mathcal I(o)$ are disjoint.
\end{enumerate}
\end{proof}




\subsection{DSIC-AE}
\begin{definition}
The essential map extension $\tilde f$ of a social choice function $f$ is the multi-valued map where $o\in \tilde f(v)$ if and only if there exists an $i$ such that for every $\epsilon\geq 0$ ($\epsilon\in\U$), the set of points for which $f=o$ has strictly positive measure in the ball of radius epsilon around $v_i$.
\end{definition}

\begin{observation}
For any fixed $v_{-i}$, $f\in\tilde f$ almost everywhere in $v_i$.
\end{observation}
\begin{proof}
\textbf{TODO: all.} Roughly, suppose $f(v)\not\in \tilde f(v)$, then there exists a ball of radius $\epsilon>0$ such that $f(v)$ occurs with measure 0 within $\tilde f(v)$. 
\end{proof}

\begin{lemma}
Let $f$ be the social choice function of a truthful mechanism for bidders with generalized utility functions $u_i(o,p_i)=v_i(o)-p_i$ and $\tilde f$ its essential extension, then there exists a $c\in\U^{mn}$ such that 
\[o\in\tilde f(v),\tilde f(v')\Rightarrow o\in \tilde f(v\oplus v'\ominus c)\enspace.\]
\end{lemma}

\begin{proof}\textbf{TODO: all.}
Same argument as before, just repeated for many points in the $\epsilon$ ball....maybe worry about exactly what the $\epsilon$ ball means?
\end{proof}

\begin{corollary}
If $f$ is DSIC-AE, then for any fixed $v_{-i}$, it maximizes a linear function $h$ with an offset $v_0$ almost everywhere in $v_i$.
\end{corollary}
\begin{proof}
We have that $\tilde f$ corresponds to a linear function $h$ with offset $v_0$, and since $f\in\tilde f$ almost everywhere the corollary follows.
\end{proof}





==> roberts-proof-bkp__1_.tex <==


\section{A ``Roberts's Theorem'' Proof for Value Maximizers}  \label{sec:roberts-proof}

Recap setup...
\begin{itemize}
\item Vector space $\U$ with addition $\oplus$ and subtraction $\ominus$.
\item outcome set $\O$ with $|\O|=m$, indexed by $j$
\item $n$ bidders with a value $v_i^j\in\U$ for item $j$ and utilities $u_i=v_i-p_i$
\item Define the notation $\delta^o,\epsilon^o\in\U^{mn}$ where all entries for $o$ are $\delta$ (respectively $\epsilon$) and other entries are 0, i.e.
\[\delta_i^{o_1}(o)=\begin{cases}
\delta&o=o_1\\
0&\mbox{otherwise.}
\end{cases}\]
\end{itemize}

\subsection{Definitions}

\begin{definition}[IIA with Sufficiency of Differences]
Let $g:\U^{mn}\rightarrow 2^\O$ be a social choice correspondence (multi-valued map) from valuation profiles to outcomes. We say that $g$ satisfies {\em independence of irrelevant alternatives (IIA) with sufficiency of differences} if for every pair of distinct outcomes $o_1$ and $o_2$ and $\Delta\in\U^n$, one of the following holds:
\begin{itemize}
\item $o_1\not\in g(v)$ for all $v$ where $v(o_1)-v(o_2)=\Delta$, i.e. $g$ strictly prefers $o_2$ to $o_1$ given $\Delta$, regardless of the valuations for other outcomes,
\item $o_2\not\in g(v)$ for all $v$ where $v(o_1)-v(o_2)=\Delta$, i.e. $g$ strictly prefers $o_1$ to $o_2$ given $\Delta$, regardless of the valuations for other outcomes, or
\item $o_1\in g(v)\Leftrightarrow o_2\in g(v)$ for all $v$ where $v(o_1)-v(o_2)=\Delta$, i.e. $g$ is indifferent between $o_1$ and $o_2$ given $\Delta$, regardless of the valuations for other outcomes.
\end{itemize}
\end{definition}

\begin{definition}
The map extension $\bar f$ of a social choice function $f$ is the multi-valued map where $o\in \bar f(v)$ if and only if there is a sequence of values $v^1, v^2,\dots, v^k,\dots$ for which $f(v^k)=o$ and the sequence converges to $v$.
\end{definition}
\begin{observation}
$\bar f$ is nonempty and upper hemicontinuous. Moreover, $f(v)\in \bar f(v)$.
\end{observation}
\begin{proof}
It is upper hemicontinuous by construction. For the claim about nonemptyness and $f(v)$, consider the sequence with $v^k=v$.
\end{proof}
\begin{observation}
If $f=o_1$ for all points in an $\epsilon$ ball around $v$ for a fixed $\epsilon$, then $\bar f(v)=\{o_1\}$.
\end{observation}

\subsection{``Affine Maximizers''}

We want to talk about when a map represents an affine maximizer. We frame it slightly differently, in terms of a linear function with an offset:
\begin{definition}
Let $g:\U^{nm}\rightarrow 2^{m}$ be a social choice correspondence from $n$ valuation vectors to outcomes in $\O$. We say that $g$ {\em maximizes a linear function $h$} if
\[g(v)=\argmax_o h(v(o))\enspace.\]
We say that a map $g$ {\em maximizes a linear function $h$ with offset $c\in\U^{mn}$} if
\[g(v)=\argmax_o h(v(o)\ominus c(o))\enspace.\]
We say that a function $f$ is a linear maximizer for $h$ (possibly with offset $c$) if $f\in g$.
\end{definition}

\begin{observation}
A linear function $h$ with offset $c$ is equivalent to an affine maximizer when $\U=\Re$.
\end{observation}
\begin{proof}
When $\U=\Re$, the linear functions are weighted sums, i.e. $h(x)=\sum_iw_ix_i$. By linearity, maximizing $h(v(o)-c(o))$ is equivalent to maximizing $h(v(o))- h(c(o))=\sum_iw_i v_i(o)-\gamma(o)$ for some weights $w_i$ and offsets $\gamma(o)$.
\end{proof}

Our first lemma gives us a concrete condition we can test to see if there is some linear function $h$ that is being maximized by a particular function or map:

\begin{lemma}
A multi-valued map $g:\U^{mn}\rightarrow 2^\O$ maximizes some linear function $h$ with offset $c$ if and only if $g$ is nonempty, upper hemicontinuous, and satisfies the following:
\begin{enumerate}
\item \label{itm:cond-mon} $o_1\in g(v)\Rightarrow \{o_1\}=g(v\oplus \epsilon^{o_1})$ for any $\epsilon>0$,
\item \label{itm:cond-iia} $g$ satisfies IIA with sufficiency of differences, and
%\item\label{itm:cond-add} $g(v)= g(v')\Rightarrow g(v\oplus v'\ominus c)=g(v)= g(v')$
\item \label{itm:cond-cvx} For any $o$, the image $\mathcal I(o)=\{v|o\in g(v)\}$ is convex.
\end{enumerate}
\end{lemma}

\begin{proof} {\em Only if.} Suppose that $g$ maximizes a linear function $h$ with offset $c$. It is easy to see that $g$ is nonempty and upper hemicontinuous. We argue the other four facts:
\begin{enumerate}
\item Suppose that $o_1\in g(v)$.  For any $o_2\neq o_1$, this implies $h(v(o_1)\ominus c(o_1))\geq h(v(o_2)\ominus c(o_2))$, which implies $h(v(o_1)\oplus\epsilon\ominus c(o_1))> h(v(o_2)\ominus c(o_2))$ and therefore $o_2\not\in g(v\oplus\epsilon^{o_1})$. Repeating for every $o_2$ implies $g(v\oplus \epsilon^{o_1})=\{o_1\}$.
\item If we add $\delta$ to every outcome, we maximize $h(v(o)\oplus\delta\ominus c)=h(v(o)\ominus c)\oplus h(\delta)$, which is the same as maximizing $h(v(o)\ominus c)$.
\item Suppose that $o_1\in g(v),g(v')$ for some $v$ and $v'$. For any $o_2\neq o_1$, this implies $h(v(o_1)\ominus c(o_1))\geq h(v(o_2)\ominus c(o_2))$ and $h(v'(o_1)\ominus c(o_1))\geq h(v'(o_2)\ominus c(o_2))$. By linearity we have
\[h((\alpha v(o_1)\oplus (1-\alpha)v'(o_1)\ominus c(o_1))\ominus c(o_1))\geq h((\alpha v(o_2)\oplus (1-\alpha)v'(o_2)\ominus c(o_2))\ominus c(o_2))\enspace.\]
Since this is true for all $o_2\neq o_1$ we can conclude that
\[o_1\in \argmax h((\alpha v\oplus (1-\alpha)v'\ominus c)\ominus c)=g(\alpha v\oplus (1-\alpha)v'\ominus c)\enspace.\]
Analogous reasoning shows that $o_1\not\in  g(v\oplus v'\ominus c)$ when $o_1\not\in g(v)\cap g(v')$ but $o_2\in g(v),g(v')$. 
\end{enumerate}

{\em If.} We must construct $h$ and $c$. Let $\mathcal I(o)=\{v|o\in g(v)\}$ be the image of $o$. We construct $h$ as follows:
\begin{enumerate}
\item {\em For any distinct $o_1,o_2$, the interiors of $\mathcal I(o_1)$ and $\mathcal I(o_2)$ are disjoint.}

For contradiction, assume that there is a $v$ in the interior of $\mathcal I(o_1)$ such that $o_1,o_2\in g(v)$. Condition~(\ref{itm:cond-mon}) implies that $g(v\oplus \epsilon^{o_2})=\{o_2\}$. However, since $v$ is in the interior of $\mathcal (o_1)$, it follows that $v\oplus\epsilon^{o_2}$ is also in the interior for sufficiently small $\epsilon$, implying $o_1\in g(v\oplus\epsilon^{o_2})$. This is a contradiction.

\item {\em For any distinct $o_1, o_2$, we can write a constant $c_{o_1,o_2}\in\U^n$ and a linear function $H_{o_1,o_2}:\U^n\rightarrow\U$ such that $H_{o_1,o_2}(v(o_1)\ominus v(o_2)\ominus c_{o_1,o_2})\geq0$ for all $v\in\mathcal I(o_1)$ and $H_{o_1,o_2}(v(o_1)\ominus v(o_2)\ominus c_{o_1,o_2})\leq$ for all $v\in\mathcal I(o_2)$.}

Fix distinct $o_1,o_2$. Since the sets $\mathcal I(o_1)$ and $\mathcal I(o_2)$ are convex and their interiors are disjoint, there is a separating hyperplane defined by a linear function $\hat H$ and constant $\hat c$ such that $\hat H(v\ominus \hat c)\geq 0$ if $v\in\mathcal I(o_1)$ and $\leq0$ for $v\in\mathcal I(o_2)$.

Moreover, since $g$ satisfies IIA with sufficiency of differences, we can write an equivalent $c$ and $H$ simply in terms of the difference between $o_1$ and $o_2$. Specifically, define $v^\Delta$ by $v^\Delta(o_1)=\Delta$ and $v^\Delta(o)=0$ otherwise. Now let $c_{o_1,o_2}=\hat c(o_1)\ominus\hat c(o_2)$ and $H_{o_1,o_2}(\Delta)=\hat H(v^\Delta\ominus\hat c)$. By IIA with sufficiency of differences, $H_{o_1,o_2}(v(o_1)\ominus v(o_2)\ominus c_{o_1,o_2})$ must still separate $\mathcal I(o_1)$ and $\mathcal I(o_2)$.

\item {\em There exists a $c\in\U^{mn}$ and a linear function $h:\U^n\rightarrow\U$ such that for any distinct $o_1,o_2$, $h(v(o_1)\ominus c(o_1)\geq h(v(o_2)\ominus c(o_2))$ for all $v\in\mathcal I(o_1)$ and $\leq0$ for $v\in\mathcal I(o_2)$.}

Remark that the planes defined by $H$ must be consistent. In particular, suppose that $v$ is such that $v(o_2)\ominus v(o_3)=c_{o_2,o_3})$, so $\H_{o_2,o_3}(v(o_2)\ominus v(o_3)\ominus c_{o_2,o_3})=0$. Then supposing $H_{o_1,o_2}(v(o_1)\ominus v(o_2)\ominus c_{o_1,o_2})>0$ , it must be that $H_{o_1,o_3}(v(o_1)\ominus v(o_3)\ominus c_{o_2,o_3})>0$. This implies that 
\[H_{o_1,o_3}(v(o_1)\ominus v(o_2)\ominus(v(o_3)-v(o_2)\ominus c_{o_2,o_3}\oplus c_{o_1,o_3}))=H_{o_1,o_3}(v(o_1)\ominus v(o_2)\ominus c_{o_1,o_2})>0\]
and thus that $H_{o_1,o_3}$ defines the same hyperplane in $(v(o_1)\ominus v(o_2))$ that is defined by $H_{o_1,o_2}$ and $c_{o_1,o_2}$.

This implies that the $H$ are the same hyperplane. Thus, pick any labeling of the $m$ outcomes $o_1,\dots,o_m$ and define
\[h(x)=H_{o_1,o_2}(x)\]
and
\[c(o)=\begin{cases}0& o=o_1\\ \ominus\sum_{j=2}^mc_{o_{j-1},o_j}&\mbox{otherwise.}\end{cases}\]
\todo{Fix this up, also verify $c$?}

\item {\em $g$ maximizes $h$ with offset $c$.} Immediate from last point.

\end{enumerate}

\end{proof}



\subsection{Consequences of IC}


\begin{definition}
For valuation profiles $v$ and $v'$ define $S_{\rightarrow}(v,v')$ as the set of valuation profiles progressively changing entries from $v$ to $v'$, i.e.
\[S(v,v')=\{v, (v'_1, v_2,\dots, v_n), (v'_1, v'_2, v_3,\dots, v_n), (v'_1,\dots, v'_{n-1}, v_n), v'\}\]
 
\end{definition}




\begin{claim}[PAD, Roberts~\cite{roberts79}] Let $f$ be the social choice function of a mechanism $M$ and let $v$ be such that $f(v)=o_1$ and $v'$ such that for all $i$, and $o_2\neq o_1$, $v_i'(o_1)\ominus v_i(o_1)>v_i'(o_2)\ominus v_i(o_2)$.  If $M$ is DSIC, then $f(v')=o_1$.
%If truth-telling is a best response for every bidder in any valuation profile from $S_\rightarrow(v,v')$, then $f(v')=o_1$.
\end{claim}
\begin{proof}
By induction. Let $v^k$ be the valuation profile in which the first $k$ agents have values from $v'$ and the remaining $n-k$ have values from $v$, i.e.
\[v^k=(v'_1,\dots, v'_k, v_{k+1},\dots,v_n)\enspace.\]
By the conditions of the lemma $f(v^0)=o_1$. Suppose that $f(v^{k-1})=o_1$ and consider the preferences of bidder $k$ under $v'$. Invoke the taxation principle to write $p_k(o)$ as the price $k$ pays if the outcome is $o$ given $v_{-k}^{k}=v_{-k}^{k-1}$. Since $f(v^{k-1})=o_1$ we know that $v_k(o_1)-p_k(o_1)\geq v_k(o_2)-p_k(o_2)$ for any outcome $o_2\neq o_1$ in its menu. Moreover, by the conditions of the lemma, we can assert that $v'_k(o_1)-v_k(o_1)> v'_k(o_2)-v_k(o_2)$ and therefore  $v'_k(o_1)-p_k(o_1)> v'_k(o_2)-p_k(o_2)$, implying that bidder $k$ strictly prefers outcome $o_1$ to any other outcome. This implies $f(v^k)=o_1$. Thus, by induction, we have $f(v')=f(v^n)=o_1$.
\end{proof}

\begin{claim}[NAD, Lavi et al.~\cite{lavi}] \textbf{Note: switched $v$ and $v'$ relative to Lavi.} Let $f$ be the social choice function of a mechanism $M$ and let $v$ be such that $o_1\neq f(v)$ and $v'$ such that for all $i$, $v_i'(o_1)\ominus v_i(o_1)<v_i'(f(v))\ominus v_i(f(v))$. If $M$ is DSIC, then $o_1\neq f(v')$.
%If no bidder has an incentive to lie when the valuation vector is any point in $S_\rightarrow(v,v')$, then $o_1\neq f(v')$.
\end{claim}
\begin{proof}
For contradiction suppose that $f(v')=o_1$. Let $\Delta=v(o_1)\ominus v'(o_1)\oplus v'(f(v))\ominus v(f(v))$ and define the valuation profile $x$ by
\[x(o)=\begin{cases}
v'(o)&o=o_1\\
v'(o)-\frac12\Delta&o=f(v)\\
\min(v'(o), v(o)\oplus v'(f(v))\ominus v(f(v)))-\Delta,&\mbox{otherwise.}
\end{cases}\]
Comparing $x$ to $v'$ with $f(v')=o_1$ implies $f(x)=o_1$ by PAD; however, comparing $x$ to $v$ implies $f(x)=f(v)$, a contradiction.
\end{proof}


\begin{claim}
If $o_1\in \bar f(v)$, then $\{o_1\}=\bar f(v\oplus(\frac1n\epsilon)^{o_1})$.
\end{claim}
\begin{proof}
Let $x$ be a point in the $\frac12\epsilon$ ball around $v$ with $f(x)=o_1$. By PAD, every point in the $\frac12\epsilon$ ball around $v\oplus\epsilon^{o_1}$ must have $f=o_1$, implying the claim.
\end{proof}


\begin{claim}[Extended PAD]
Let $\bar f$ be the extended social choice map of a DSIC mechanism $M$. Fix $v$ and $o_1\in\bar f(v)$. If $\Delta\in\U^{mn}$ is such that $\Delta_i(o_1)\geq\Delta_i(o_2)$ for all $o_2\neq o_1$, then $o_1\in\bar f(v\oplus\Delta)$.
\end{claim}
\begin{proof}
We must show that there is a sequence of valuation profiles with $f=o_1$ converging to $v\oplus\Delta$. By definition of $\bar f$ there exists a sequence $\{v^k\}$ converging to $v$ with $f(v^k)=o_1$. Consider the sequence $\{y^k\}=\{v^k\oplus\Delta\oplus(\epsilon^k)^{o_1}\}$ where $\epsilon^k$ is a sequence converging to 0 and therefore $\{y^k\}$ converges to $v\oplus\Delta$. By applying PAD to each pair of terms $y^k$ and $v^k$ we see that $f(y^k)=o_1$, demonstrating that $o_1\in\bar f(v\oplus\Delta)$.
\end{proof}

%\begin{claim}[Extended PAD]
%Let $\bar f$ be the extended social choice map of a DSIC mechanism $M$. Fix $v$ and $o_1\in\bar f(v)$. If $\Delta\in\U^{mn}$ is such that $\Delta(o_1)\geq\Delta(o_2)$ for all $o_2\neq o_1$, then $o_1\in\bar f(v\oplus\Delta)$. Moreover, if $\Delta_i(o_1)>\Delta_i(o_2)$ for all $i$, then $o_2\not\in\bar f(v\oplus\Delta)$.
%\end{claim}
%\begin{proof}
%To show $o_o\in\bar f(v\oplus\Delta)$ we must show that there is a sequence of valuation profiles with $f=o_1$ converging to $v\oplus\Delta$. By definition of $\bar f$ there exists a sequence $\{v^k\}$ converging to $v$ with $f(v^k)=o_1$. Consider the sequence $\{y^k\}=\{v^k\oplus\Delta\oplus(\epsilon^k)^{o_1}\}$ where $\epsilon^k$ is a sequence converging to 0 and therefore $\{y^k\}$ converges to $v\oplus\Delta$. By applying PAD to each pair of terms $y^k$ and $v^k$ we see that $f(y^k)=o_1$, demonstrating that $o_1\in\bar f(v\oplus\Delta)$.
%
%Next, we show that when $\Delta(o_2)<\Delta(o_1)$, then $o_2\not\in\bar f(v\oplus\Delta)$. Let $\Delta_12=\Delta(o_1)-\Delta(o_2)$. 
%
%\end{proof}




\begin{claim}[Extended NAD]
Let $\bar f$ be the extended social choice map of a DSIC mechanism $M$. Fix $v$ and $o_1\not\in\bar f(v)$. If $\Delta\in\U^{mn}$ is such that $\Delta_i(o_1)\leq\Delta_i(o_2)$ for some $o_2\in\bar f(v)$, then $o_1\not\in\bar f(v'\oplus\Delta)$.
\end{claim}
\begin{proof} By extended PAD, $o_1\in\bar f(v\oplus\epsilon^{o_2}\oplus\epsilon^{o_1})$. 

By definition of $\bar f$, there exists an $\epsilon$ such that $f(x)\neq o_1$ for any $x$ in the $\epsilon$ ball around $v$. Consider the point $x=v\oplus(\frac1{2n}\epsilon)^{o_1}$. For contradiction, suppose that $o_1\in\bar f(v')$. Then there exists an $x'$ in the $\frac14\epsilon$ ball around $v'$ such that $f(x')=o_1$. 



since the outcome space is finite there must be an $\epsilon$ such that $f(x)\in\bar f(v)$ for any $x$ in the $\epsilon$ ball around $v$. Moreover, the ball of radius $\frac12\epsilon$ around the point $v\oplus(\frac1{2n}\epsilon)^{o_1}$ lies entirely within this ball around $v$, implying that 
\end{proof}






\begin{claim}[IIA with Sufficiency of Differences]
The extended social choice map $\bar f$ of a DSIC mechanism $M$ satisfies IIA with sufficiency of differences.
\end{claim}
\begin{proof}
Pick any distinct outcomes $o_1,o_2$ and difference $\Delta$. Let $v$ and $v'$ be such that $v(o_1)-v(o_2)=v'(o_1)-v'(o_2)=\Delta$, and define $x$ as follows:
\[x_i(o)=\begin{cases}\max(v_i(o),v_i'(o))&o\in\{o_1,o_2\}\\
\min(v_i(o),v_i'(o))&\mbox{otherwise.}\end{cases}\]
By extended PAD, $o_1\in\bar f(v)\Rightarrow o_1\in\bar f(v'')$ and $o_1\in\bar f(v')\Rightarrow o_1\in\bar f(v'')$. Similar reasoning for $o_2$ thus implies that $\bar f(x)\cap\{o_1,o_2\}\supset (\bar f(v)\cup\bar f(v'))\cap\{o_1,o_2\}$.


\end{proof}


\begin{lemma}\label{lem:f-add}
If $g:\U^{mn}\rightarrow 2^\O$ is a map satisfying extended PAD and extended NAD and $c$ is a valuation profile with $g(c)=\O$, then
\[g(v)=g(v')\Rightarrow g(v\oplus v'\ominus c)=g(v)=g(v').\]
for all $v$ and $v'$
\end{lemma}
\begin{proof}
Fix an $o_2\not\in\bar g(v)$. We repeatedly apply extended PAD (EPAD) and extended NAD (ENAD) to show that $f(v\oplus v'\ominus c)\neq o_2$.
\begin{enumerate}
\item Pick outcomes $o_2,o_3\neq o_1$ and fix $\epsilon$.
\item Define the valuation profile $x$ by 
\[x_i(o)=\begin{cases}
v_i(o)&o=o_1\\
v_i(o)&o=o_2\\
v_i(o_2)\oplus c_i(o_3)\ominus c_i(o_2)&o=o_3\\
v_i(o)&\mbox{otherwise.}
\end{cases}\]
ENAD implies $g(x)=g(v)$. Specifically, ENAD as $c\rightarrow x$ implies that outcome $o_3$ can't be in $\bar f(x)$ unless $o_2$ is in $\bar f(x)$. is preferred to outcome $o_3$ and therefore $f(x)\neq o_3$ (recall that by assumption $f(c\oplus\epsilon^{o_2})=o_2$). NAD using $v$ and $x$ implies that outcome $o_1$ is preferred to all remaining outcomes, i.e. $f(x)\neq o_2$ and $f(x)\neq o'$ for any $o'\not\in\{o_1,o_2,o_3\}$.

\item Define the valuation profile $x'$ by 
\[x'_i(o)=\begin{cases}
v'_i(o)&o=o_1\\
v'_i(o)&o=o_2\\
v'_i(o_1)\oplus c_i(o_3)\ominus c_i(o_1)&o=o_3\\
v'_i(o)&\mbox{otherwise.}
\end{cases}\]
ENAD implies $f(x')=o_3$. Specifically, ENAD using $c$ and $x'$ implies that outcome $o_3$ is preferred to outcome $o_1$ and therefore $f(x)\neq o_1$ (recall that by assumption $f(c)=o_3$). NAD using $v'$ and $x$ implies that outcome $o_1$ is preferred to all remaining outcomes, i.e. $f(x)\neq o_2$ and $f(x)\neq o'$ for any $o'\not\in\{o_1,o_2,o_3\}$.

\item Define the valuation profile $y$ by
\[y_i(o)=\begin{cases}
v_i(o)\oplus v_i'(o)\ominus c_i(o)&o=o_1\\
v_i(o)\oplus v_i'(o)\ominus c_i(o)&o=o_2\\
v'_i(o_1)\oplus v_i(o_2)\ominus c_i(o_1)\oplus c_i(o_3)\ominus c_i(o^2)&o=o_3\\
v_i(o)\oplus v_i'(o)\ominus c_i(o)&\mbox{otherwise.}
\end{cases}\]
NAD implies $f(y)=o_1$. Specifically, NAD using $x$ and $y$ implies that outcome $o_1$ is preferred to outcome $o_3$ and therefore $f(x)\neq o_1$. NAD using $v$ and $x$ implies that outcome $o_2$ is preferred to all remaining outcomes, i.e. $f(x)\neq o_2$ and $f(x)\neq o'$ for any $o'\not\in\{o_1,o_2,o_3\}$.

\item Define the valuation profile $z$ by
\[z_i(o)=\begin{cases}
v_i(o)\oplus v_i'(o)\ominus c_i(o)&o=o_1\\
v_i(o)\oplus v_i'(o)\ominus c_i(o)&\mbox{otherwise.}
\end{cases}=v\oplus v'\ominus c\]
NAD with $y$ and $z$ implies that $o_1$ is preferred to $o_2$ and therefore $f(z)\neq o_2$.
\end{enumerate}

Repeating this logic for every $o_2\neq o_1$ implies that $f(v\oplus v'\ominus c\oplus)=o_1$.
\end{proof}


%\begin{corollary}
%Let $c$ be such that $f(c\oplus \epsilon^o)=o$ for any $o$ and $\epsilon>0$, and let $o_1$, $v$, and $v'$ be such that $o_1=f(v)=f(v')$. Assuming $M$ is DSIC, then
%\[o_1= f\left(\frac12(v\oplus v')\oplus7\epsilon^{o_1}\right)\]
%for any $\epsilon\geq 0$.
%
%Additionally, we can relax the DSIC requirement --- there exists a finite set of points $S\subseteq \U^{mn}$ such that the lemma holds as long as truth-telling is a best-response for all bidders at all points in $S$. Moreover...
%\end{corollary}
%\begin{proof}
%By the lemma, $f(v\oplus v'\ominus c\oplus6\epsilon^{o_1})=o_1$. For contradiction, suppose that
%\[f\left(\frac12(v\oplus v')\oplus3(\epsilon^{o_1}-\epsilon^{o_2})\right)=o_2\neq o_1\enspace.\]
%Then applying the lemma we can conclude that $f(v\oplus v'\ominus c\oplus6\epsilon^{o_1})=o_2$, a contradiction.
%
%By NAD, we can then conclude that 
%\[o_1= f\left(\frac12(v\oplus v')\oplus7\epsilon^{o_1})\right)=o_1\enspace.\]
%The claims about $S_{\ref{lem:f-add}}$ follow by inspection of the proof --- it invokes PAD and NAD (each which require best-responses at points in a finite set $S_\rightarrow$) a finite number of times.
%\end{proof}


\subsection{DSIC}

In order to deal with ``ties'' we introduce a map that (intuitively) identifies ``all reasonable outcomes for valuations $v$'':

\begin{definition}
The map extension $\bar f$ of a social choice function $f$ is the multi-valued map where $o\in \bar f(v)$ if and only if there is a sequence of values $v^1, v^2,\dots, v^k,\dots$ for which $f(v^k)=o$ and the sequence converges to $v$.
\end{definition}
\begin{observation}
$\bar f$ is nonempty and upper hemicontinuous. Moreover, $f(v)\in \bar f(v)$.
\end{observation}
\begin{proof}
It is upper hemicontinuous by construction. For the claim about nonemptyness and $f(v)$, consider the sequence with $v^k=v$.
\end{proof}
\begin{observation}
If $f=o_1$ for all points in an $\epsilon$ ball around $v$ for a fixed $\epsilon$, then $\bar f(v)=\{o_1\}$.
\end{observation}

\begin{claim}[Extended PAD]
Let $f$ be the social choice function of a truthful mechanism for bidders with generalized utility functions $u_i(v_i,o,p_i)=v_i(o)-p_i$ and $\bar f$ its map extension, then $o_1\in\bar f(v)\Rightarrow \{o_1\}=\bar f(v\oplus \epsilon^{o_1})$. \textbf{Can be generalized to be parallel to PAD if necessary...}
\end{claim}
\begin{proof}
By definition of $\bar f$, there exists a value $v'$ in the $\frac12\epsilon$-ball around $v$ such that $f(v')=o_1$. Applying PAD to $v'$ all points in an $\frac12\epsilon$ ball around $v\oplus\epsilon^{o_1}$ implies that $f=o_1$ for all points in the ball and thereby $\{o_1\}=\bar f(v\oplus \epsilon^{o_1})$.
\end{proof}



\begin{claim}
Let $f$ be the social choice function of a truthful mechanism for bidders with generalized utility functions $u_i(v_i,o,p_i)=v_i(o)-p_i$ and $\bar f$ its map extension, then there exists a $c\in\U^{mn}$ such $\bar f(c)=\O$.
\end{claim}
\begin{proof}
Set $v_{-1}=0$. By the taxation principle, we can write a price $p_1(o)\in\U$ for each outcome $o$. Take $c=(p_1, v_{-i})$. Clearly, bidder 1 is indifferent among all outcomes at $c$, so if we increase agent 1's value for outcome $o_1$ by $\epsilon$ (i.e. set $c'_1(o_1)=p_1(o_1)\oplus\epsilon$) then we must have a point $c'$ where $f(c')=o_1$. Taking a sequence of $\epsilon$ that converge to 0 implies that $o_1\in\bar f(c)$; repeating for all $o$ shows $\bar f(c)=\O$.
\end{proof}


\begin{claim}
Let $f$ be the social choice function of a truthful mechanism for bidders with generalized utility functions $u_i(v_i,o,p_i)=v_i(o)-p_i$ and $\bar f$ its map extension, then $\bar f(v)=\bar f(v\oplus(\delta,\dots,\delta))$ for any $\delta\in\U^n$.
\end{claim}
\begin{proof}
Pick any $o_1\in\bar f(v)$. If $f(v)=o_1$, then by extended PAD, $f(v\oplus(\delta,\dots,\delta)\oplus\epsilon^{o_1})$ for any $\epsilon>0$. If $f(v)=o_1$, then for any 
\end{proof}


\begin{claim}
Let $f$ be the social choice function of a truthful mechanism for bidders with generalized utility functions $u_i(v_i,o,p_i)=v_i(o)-p_i$ and $\bar f$ its map extension, and $c$ satisfying $\bar f(c)=\O$, then $\bar f(v)= \bar f(v')\Rightarrow \bar f(v\oplus v'\ominus c)=\bar f(v)= \bar f(v')$
\end{claim}
\begin{proof}
First, we show that $o_1\in \bar f(v)\cap \bar f(v')\Rightarrow o_1\in \bar f(v\oplus v'\ominus c)$. By definition of $\bar f$, there are sequences $v^k$ and $v'^k$ that converge to $v$ and $v'$ respectively and have $f=o_1$ at every point in the sequence. By Lemma~\ref{lem:f-add} we know that $f(v^k\oplus v'^k\ominus c\oplus 6\epsilon^{o_1})=o_1$. This is a sequence converging to $v\oplus v'\ominus c$, implying $o_1\in\bar f(v\oplus v'\ominus c)$.

The other direction we need to argue is that if $o_1\not\in\bar f(v), \bar f(v')$ but t$\bar f(v)\cap\bar f(v')$, then $o_1\not\in\bar f(v\oplus v'\ominus c)$. Pick an $\epsilon$ sufficiently small that $f(x)\in\bar f(v)$ for every $x$ in the $2n\epsilon$ ball around $v$. Let $o_2=f(v\oplus\frac12\epsilon^{o_1}\ominus\frac12\epsilon^{o_2})\in\bar f(v)$.  Since $\bar f(v)=\bar f(v')$, there is an $x'$ arbitrarily close to $v'$ such that $f(x')=o_2$. Applying Lemma~\ref{lem:f-add} with $\epsilon'=\frac1{12}\epsilon$ implies that $f(v\oplus x'\ominus c\oplus \frac12\epsilon^{o_1})=o_2$. NAD then implies that $f(v\oplus v'\ominus c)\neq o_1$ and, moreover, that $f(y)\neq o_1$ for any in a sufficiently small ball around $v\oplus v'\ominus c$. By consequence we can conclude that $o_1\not\in \bar f(v\oplus v'\ominus c)$.

\end{proof}



\begin{lemma}
If $f$ is DSIC, then $f$ is a linear maximizer for some function $h$ with some offset $v_0$.
\end{lemma}
\begin{proof}
\begin{enumerate}
\item $g(c)=\O$,
\item $g(v)=g(v\oplus(\delta,\dots,\delta))$ for any $\delta\in\U^n$ (adding the same thing to every outcome), and
\item\label{itm:cond-3} $g(v)\cap g(v')\neq\emptyset\Rightarrow g(v\oplus v'\ominus c)=g(v)\cap g(v')$
%for any $o$, the image $\mathcal I(o)=\{v|o\in g(v)\}$ is convex and the interiors of the images $\mathcal I(o)$ are disjoint.
\end{enumerate}
\end{proof}




\subsection{DSIC-AE}
\begin{definition}
The essential map extension $\tilde f$ of a social choice function $f$ is the multi-valued map where $o\in \tilde f(v)$ if and only if there exists an $i$ such that for every $\epsilon\geq 0$ ($\epsilon\in\U$), the set of points for which $f=o$ has strictly positive measure in the ball of radius epsilon around $v_i$.
\end{definition}

\begin{observation}
For any fixed $v_{-i}$, $f\in\tilde f$ almost everywhere in $v_i$.
\end{observation}
\begin{proof}
\textbf{TODO: all.} Roughly, suppose $f(v)\not\in \tilde f(v)$, then there exists a ball of radius $\epsilon>0$ such that $f(v)$ occurs with measure 0 within $\tilde f(v)$. 
\end{proof}

\begin{lemma}
Let $f$ be the social choice function of a truthful mechanism for bidders with generalized utility functions $u_i(o,p_i)=v_i(o)-p_i$ and $\tilde f$ its essential extension, then there exists a $c\in\U^{mn}$ such that 
\[o\in\tilde f(v),\tilde f(v')\Rightarrow o\in \tilde f(v\oplus v'\ominus c)\enspace.\]
\end{lemma}

\begin{proof}\textbf{TODO: all.}
Same argument as before, just repeated for many points in the $\epsilon$ ball....maybe worry about exactly what the $\epsilon$ ball means?
\end{proof}

\begin{corollary}
If $f$ is DSIC-AE, then for any fixed $v_{-i}$, it maximizes a linear function $h$ with an offset $v_0$ almost everywhere in $v_i$.
\end{corollary}
\begin{proof}
We have that $\tilde f$ corresponds to a linear function $h$ with offset $v_0$, and since $f\in\tilde f$ almost everywhere the corollary follows.
\end{proof}





==> roberts-proof.tex <==


\section{A ``Roberts's Theorem'' Proof for $\U$-Space Agents}  \label{sec:roberts-proof}

Our generalization of Roberts's Theorem will apply to the following setting:
\begin{itemize}
\item $\U$ is a normed vector space with addition $\oplus$ and subtraction $\ominus$, as well as the associated ordering $\geq$. (For our lexicographic space $\U$, define $||u||=|u|$ and for $\U^n$ define it as $||u||=|\sum u_i|$, where $|\cdot|$ denotes the standard absolute value of a function.)
\item $n$ bidders, each with a value $v_i(o)\in\U$ for outcome $o$ and utilities $u_i(v_i,o,p_i)=v_i(o)-p_i$.
\end{itemize}
For notation, let $\delta^o,\epsilon^o\in\U^{mn}$ where all entries for $o$ are $\delta$ (respectively $\epsilon$) and other entries are 0, i.e.
\[\delta_i^{o_1}(o)=\begin{cases}
\delta&o=o_1\\
0&\mbox{otherwise.}
\end{cases}\]

\subsection{Definitions}

We follow Proof 1 from Lavi et al~\cite{lavi08}, with modifications. In particular, instead of working with the social choice function $f$, we work with a map that captures tied outcomes:

\begin{definition}
The map extension $\bar f$ of a social choice function $f$ is the multi-valued map where $o\in \bar f(v)$ if and only if there is a sequence of values $v^1, v^2,\dots, v^k,\dots$ for which $f(v^k)=o$ and the sequence converges to $v$.
\end{definition}
\begin{observation}\label{obs:map-exclusive}
$\bar f$ is nonempty and upper hemicontinuous. Moreover, $f(v)\in \bar f(v)$.
\end{observation}
\begin{proof}
It is upper hemicontinuous by construction. For the claim about nonemptyness and $f(v)$, consider the sequence with $v^k=v$.
\end{proof}
\begin{observation}\label{obs:map-monotone}
If $f=o_1$ for all points in an $\epsilon$ ball around $v$ for a fixed $\epsilon$, then $\bar f(v)=\{o_1\}$.
\end{observation}

We want to talk about when a map represents an affine maximizer. We frame it slightly differently, in terms of a linear function with an offset:
\begin{definition}
Let $g:\U^{nm}\rightarrow 2^{m}$ be a social choice correspondence from $n$ valuation vectors to outcomes in $\O$. We say that $g$ {\em maximizes a linear function $h$} if
\[g(v)=\argmax_o h(v(o))\enspace.\]
We say that a map $g$ {\em maximizes a linear function $h$ with offset $\gamma\in\U^{m}$} if
\[g(v)=\argmax_o h(v(o))\ominus\gamma(o)\enspace.\]
We say that a function $f$ is a linear maximizer for $h$ (possibly with offset $\gamma$) if $f\in g$.
\end{definition}

%\begin{claim}
%If $o_1\in \bar f(v)$, then $\{o_1\}=\bar f(v\oplus(\frac1n\epsilon)^{o_1})$.
%\end{claim}
%\begin{proof}
%Let $x$ be a point in the $\frac12\epsilon$ ball around $v$ with $f(x)=o_1$. By PAD, every point in the $\frac12\epsilon$ ball around $v\oplus\epsilon^{o_1}$ must have $f=o_1$, implying the claim.
%\end{proof}

\subsection{Monotonicity}

First, we introduce the key monotonicity properties used by Lavi et al.~\cite{lavi08}. Once we generalize them appropriately to our map extension $\bar f$, many steps of the proof will go through quickly.

\begin{claim}[PAD~\cite{roberts79}] Let $f$ be the social choice function of a mechanism $M$ and let $v,v'$ be valuation profiles. If $f(v)=o_1$ and for all $i$ and $o_2\neq o_1$ the outcome $o_1$ has a larger difference $v_i'(o_1)\ominus v_i(o_1)>v_i'(o_2)\ominus v_i(o_2)$, then $f(v')=o_1$.
\end{claim}
\begin{proof}
By induction. Let $v^k$ be the valuation profile in which the first $k$ agents have values from $v'$ and the remaining $n-k$ have values from $v$, i.e.
\[v^k=(v'_1,\dots, v'_k, v_{k+1},\dots,v_n)\enspace.\]
By the conditions of the lemma $f(v^0)=o_1$. Suppose that $f(v^{k-1})=o_1$ and consider the preferences of bidder $k$ under $v'$. Invoke the taxation principle to write $p_k(o)$ as the price $k$ pays if the outcome is $o$ given $v_{-k}^{k}=v_{-k}^{k-1}$. Since $f(v^{k-1})=o_1$ we know that $v_k(o_1)\ominus p_k(o_1)\geq v_k(o_2)\ominus p_k(o_2)$ for any outcome $o_2\neq o_1$ in its menu. Moreover, by the conditions of the lemma, we can assert that $v'_k(o_1)\ominus v_k(o_1)> v'_k(o_2)\ominus v_k(o_2)$ and therefore  $v'_k(o_1)\ominus p_k(o_1)> v'_k(o_2)\ominus p_k(o_2)$, implying that bidder $k$ strictly prefers outcome $o_1$ to any other outcome in its menu. This implies $f(v^k)=o_1$. Thus, by induction, we have $f(v')=f(v^n)=o_1$.
\end{proof}

\begin{claim}[Extended PAD]
Let $\bar f$ be extended map of a mechanism $M$ and let $v,v'$ be valuation profiles. If $o_1\in \bar f(v)$ and for all $i$ and $o_2\neq o_1$ the outcome $o_1$ has a larger difference $v_i'(o_1)\ominus v_i(o_1)>v_i'(o_2)\ominus v_i(o_2)$, then $\bar f(v')=\{o_1\}$.
\end{claim}

\begin{proof}
Choose $\epsilon<\frac12\min_{o_2\neq o_1,i}(v_i'(o_1)\ominus v_i(o_1)\ominus(v_i'(o_2)\ominus v_i(o_2)))$. By definition of $\bar f$, there exists an $x$ in the $\epsilon$ ball around $v$ such that $f(x)=o_1$. Moreover, for any $y$ in the $\epsilon$ ball around $v'$, ordinary PAD implies $f(y)=o_1$. Applying Observation~\ref{obs:map-exclusive} then implies that $\bar f(v')=\{o_1\}$.

%Choose $\epsilon$ small enough that $v'\ominus \epsilon^{o_1}$ still satisfies the conditions of PAD with respect to $v$ (note that this subtracts $\epsilon$ from each bidder, so this point will lie on the boundary of the $n\epsilon$ ball around $v'$). By the definition of $\bar f$, there exists an $x$ in the $\frac n2\epsilon$ ball around $v$. Applying PAD to $x$ and $v'\ominus\epsilon^{o_1}$ implies $f(v'\ominus\epsilon^{o_1})=o_1$. Moreover, for any point $y$ in the $\frac n4\epsilon$ ball around $v'$, PAD from $v'\ominus\epsilon^{o_1}$ to $y$ implies that $f(y)=o_1$. Using Observation~\ref{obs:map-monotone} then implies that $\bar f(v')=o_1$.
\end{proof}

\begin{claim}[NAD~\cite{lavi08}] Let $f$ be the social choice function of a mechanism $M$. Let $v$ and $v'$ be valuation profiles and $o_1$ and $o_2$ outcomes such that $f(v')=o_1$ and $v_i'(o_2)\ominus v_i(o_2)>v_i'(o_1)\ominus v_i(o_1)$, then $f(v)\neq o_2$.
\end{claim}
\begin{proof}
For contradiction suppose that $f(v)=o_2$. Let $\Delta=v'(o_2)\ominus v(o_2)\oplus v(o_1)\ominus v'(o_1)$ and define the valuation profile $x$ by
\[x(o)=\begin{cases}
v(o)&o=o_2\\
v(o)\ominus\frac12\Delta&o=o_1\\
\min(v'(o), v'(o)\oplus v(o_1)\ominus v'(o_1))\ominus\Delta,&\mbox{otherwise.}
\end{cases}\]
Comparing $x$ to $v$ with $f(v)=o_2$ implies $f(x)=o_2$ by PAD; however, comparing $x$ to $v'$ implies $f(x)=o_1$, a contradiction.
\end{proof}

\begin{claim}[Extended NAD] Let $\bar f$ be the extended map of a mechanism $M$. Let $v$ and $v'$ be valuation profiles and $o_1$ and $o_2$ outcomes such that $o_1\in\bar f(v')$ and $v_i'(o_2)\ominus v_i(o_2)>v_i'(o_1)\ominus v_i(o_1)$, then $o_2\not\in\bar f(v)$.
\end{claim}
\begin{proof}
Similar to the proof of extended PAD, choose $\epsilon<\min_i(v_i'(o_2)\ominus v_i(o_2)\ominus(v_i'(o_1)\ominus v_i(o_1)))$. By definition of $\bar f$, there exists a $y$ in the $\epsilon$ ball around $o_1$ such that $f(y)=o_1$. Moreover, for any $x$ in the $\epsilon$ ball around $v$, ordinary NAD implies $f(x)\neq o_2$. By definition of $\bar f$ this implies that $o_2\not\in\bar f(v)$.
\end{proof}

\subsection{Sets of Differences and Manipulating PAD and NAD}

To proceed with the proof, we need to define the key sets $P(o_1,o_2)$ as follows:
\[P(o_1,o_2)=\{\Delta\in\U^n|\exists v\mbox{ s.t. }v(o_1)-v(o_2)=\Delta\mbox{ and }o_1\in\bar f(v)\}\]
With this definition in hand, the following claims depend only on PAD and NAD. Using our extensions of PAD and NAD these go through effectively without comment by replacing $f(v)=o$ statements with $o\in\bar f(v)$ as appropriate:
\begin{claim}[Lavi et al. Claim 2]\label{clm:lavi-2}
For every $\Delta,\epsilon\in\U^n$ where $\epsilon>0$:
\begin{enumerate}
\item $\Delta\ominus\epsilon\in P(o_1,o_2)\Rightarrow \ominus\Delta\not\in P(o_2,o_1)$
\item $\Delta\not\in P(o_1,o_2)\Rightarrow\ominus\Delta\in P(o_2,o_1)$
\end{enumerate}
\end{claim}

\begin{claim}[Lavi et al. Claim 3]\label{clm:lavi-3}
For every $\Delta^{1-2},\Delta^{2-3},\epsilon^{1-2},\epsilon^{2-3}\in\U^n$ where $\epsilon\geq 0$,
\[\Delta^{1-2}\ominus\epsilon^{1-2}\in P(o_1,o_2)\mbox{ and }\Delta^{2-3}\ominus\epsilon^{2-3}\in P(o_2,o_3)\Rightarrow \Delta^{1-2}\oplus\Delta^{2-3}\ominus\frac12(\epsilon^{1-2}\oplus\epsilon^{2-3})\in P(o_1,o_3)\]
\end{claim}


The next step in Lavi et al.~\cite{lavi08} shifts the $P$ sets so they are identical. Their approach is to find $\gamma(o_1,o_2)=\inf\{p|p\rightarrow\vec 1\in P(o_1,o_2)\}$. Unfortunately, we cannot assume that the infimum exists in a general topological vector space (indeed, in our case it does not). Instead, we identify equivalent {\em vectors} $\gamma$ that will serve our purposes.

The key property of the $\gamma(o_1,o_2)$ values is that the vector $\gamma(o_1,o_2)\vec1$ lies on the boundary of the $P(o_1,o_2)$ sets. We will show that such boundary points must exist for $\bar f$.

\begin{definition}
Given an arbitrary labeling of outcomes $o_1,\dots,o_m$, we define vectors $\gamma(o_j,o_k)\in\U^n$ as follows:
\begin{enumerate}
\item Let $G$ be a graph where the outcomes are the vertices and there is an edge between $o_j$ and $o_k$ if and only if we have found a value for $\gamma(o_j,o_k)$.
\item Let $H$ be a graph where the outcomes are the vertices and there is an edge between $o_j$ and $o_k$ if and only if there is a bidder $i$ and a setting of values $v_{-i}$ such that $f(v_i,v_{-i})=o_j$ for some value $v_i$ and $f(v_i',v_{-i})=o_k$ for another value $v_i'$.
\item While $G$ has more than one connected component, identify an edge in $H$ that does not induce a cycle. This edge corresponds to a bidder $i$ and setting of others' values $v_{-i}$. Invoking the taxation principle, $i$'s menu includes outcome $o_1$ at a price $p_i(o_j)$ and outcome $o_k$ at a price $p_i(o_k)$. Set
\[\gamma(o_j,o_k)=\ominus\gamma(o_k,o_j)=p_i(o_j)\ominus p_i(o_k)\]
note this with an edge in $G$.
\item While $G$ is not the complete graph, identify a triangle that can be completed, i.e. identify $o_j,o_k,o_l$ such that $\gamma(o_j,o_k)$ is not set but $\gamma(o_j,o_l)$ and $\gamma(o_l,o_k)$ are both set. Set
\[\gamma(o_j,o_k)=\ominus\gamma(o_k,o_j)=\gamma(o_j,o_l)\oplus\gamma(o_l,o_k)\]
\end{enumerate}
\end{definition}
\begin{claim}
This defines all $\gamma$.
\end{claim}
\begin{proof}
It is sufficient to prove that $H$ is connected. Remark that for any outcome pair $o_j,o_k$, there exist valuations $v$ and $v'$ such that $f(v)=o_j$ and $f(v')=o_k$. If we change bidders values from $v_i$ to $v_i'$ one by one, any time the outcome changes we get an edge in $H$. Since we start at $o_j$ and end at $o_k$, this implies there is a path from $o_j$ to $o_k$ in $H$ for any such pair, and therefore $H$ is connected.
\end{proof}

We need to prove that when $\gamma$ was defined in step (2) we got a point on the boundary (this was by construction in Lavi et al.):
\begin{claim}
$\gamma(o_j,o_k)\in P(o_j,o_k)$ and $\ominus\gamma(o_j,o_k)\in P(o_k,o_j)$
\end{claim}
\begin{proof}
Fix $o_j,o_k$ and consider the step when $\gamma(o_j.o_k)$ was set. Assuming all previously set $\gamma(o_j,o_k)$ satisfy the claim, then $\gamma(o_j,o_k)$ does as well. The full claim then follows by induction.

Suppose $\gamma(o_j,o_k)$ was set in step (1). Fixing $v_{-i}$, let $v_i''$ be any valuation vector with $v_i''(o_j)=p_i(o_j)$ and $v_i''(o_k)=p_i(o_k)$. This is an indifference point for bidder $i$, so there is clearly a sequence converging from the region in which $i$ prefers $o_j$ and one from which it prefers $o_k$, e.g. take $v^k=v''\oplus\epsilon^{o_j}$ or $v^k=v''\oplus\epsilon^{o_k}$ as $\epsilon\rightarrow0$. This implies that $o_j,o_k\in\bar f(v_i,v_{-i})$ and therefore $\gamma(o_j,o_k)$ is on the boundary between $P(o_j,o_k)$ and $\ominus P(o_k,o_j)$.

If $\gamma$ was set in step (2), we use Claim~\ref{clm:lavi-3}. By the inductive hypothesis, $\gamma(o_j,o_l)$, $\gamma(o_l,o_j)$, $\gamma(o_k,o_l)$, and $\gamma(o_l,o_k)$ are in their respective sets $P$. Then Claim~\ref{clm:lavi-3} implies that $\gamma(o_1,o_3)\oplus\epsilon^{o_1}\in P(o_1,o_3)$ and $\gamma(o_3,o_1)\oplus\epsilon^{o_3}\in P(o_3,o_1)$ for any $\epsilon$. It then follows that $\gamma(o_1,o_3)\in P(o_1,o_3)$ and $\gamma(o_3,o_1)\in P(o_3,o_1)$ by upper hemicontinuity of $\bar f$.
\end{proof}
Whereas the previous claim was by construction in Lavi et al., they prove the following claim that we get by construction:
\begin{claim}
For all $o_1,o_2,o_3$:
\begin{itemize}
\item $\gamma(o_1,o_2)=-\gamma(o_2,o_1)$
\item $\gamma(o_1,o_3)=\gamma(o_1,o_2)\oplus\gamma(o_2,o_3)$.
\end{itemize}
\end{claim}

We can now shift the sets as in Lavi et al.~\cite{lavi08}. We define $C(o_1,o_2)$ as follows:
\[C(o_1,o_2)=P(o_1,o_2)\ominus\gamma(o_1,o_2)\]
and let $\mathring C$ denote the interior. The following claims now goes through without substantial comment:
\begin{claim}[Lavi et al. Claim 5]
$\mathring C(o_1,o_2)=\mathring C(o_3,o_4)=\mathring C$ for every $o_1,o_2,o_3,o_4\in\O$ where $o_1\neq o_2$ and $o_3\neq o_4$.
\end{claim}
\begin{claim}
$\mathring C$ is convex.
\end{claim}



\subsection{Separating Hyperplanes}

To complete the proof, we must invoke the separating hyperplane theorem. We use an infinite dimensional version~\cite{borderNotes}:

\begin{claim}
There exists a monotone linear function $h:\U^n\rightarrow\U$ and offsets $\gamma:\O\rightarrow\U$ such that $\bar f$ maximizes $h$ with offset $\gamma$.
\end{claim}
\begin{proof}
Claim~\ref{clm:lavi-2} implies that $C(o_1,o_2)\cup (\ominus C(o_2,o_1))$ cover $\U^n$. Moreover, by construction of $\gamma$ we know that these sets overlap on their boundary. Thus, since $C(o_1,o_2)=C(o_2,o_1)=C$, the separating hyperplane theorem tells us that there is a linear function $h:\U^n\rightarrow\U$ such that $h(\Delta)>0$ for $\Delta\in \mathring C$, $h(\Delta)<0$ for $\Delta\in\ominus\mathring C$, and $h(\Delta)=0$ for $\Delta\in C\cap(\ominus C)$.

Unraveling the sets $P(o_1,o_2)$, we find that $\Delta\in P(o_1,o_2)$ if and only if $h(\Delta\ominus\gamma(o_1,o_2))\geq 0$, which by linearity of $h$ corresponds to $h(v(o_1))\ominus h(\gamma(o_1,o_2))\geq h(v(o_2))$ for a valuation profile $v$.

Finally, we define $\gamma(o_j)=h(\sum_{k=2}^j\gamma(o_{k-1},o_k)$. We can then equivalently write $\Delta\in P(o_1,o_2)$ if and only if $h(v(o_1))\ominus \gamma(o_1)\geq h(v(o_2))\ominus\gamma(o_2)$, i.e. $\bar f$ corresponds to maximizing the linear function $h$ with offsets $\gamma$. Recalling that $f\in\bar f$ proves that $f$ must be an affine maximizer.
\end{proof}


%\subsection{DSIC-AE}
%
%Thus far we have extended Roberts's theorem to our topological vector space, but we are not done because we need to relax it to match DSIC-AE. To do this we replace $\bar f$ with a map $\tilde f$ that smooths over any measure-0. This works for bidders with values in $\Re$, though it will not immediately extend to arbitrary topological vector spaces because they 
%
%\begin{definition}
%The essential map extension $\tilde f$ of a social choice function $f$ is the multi-valued map where $o\in \tilde f(v)$ if and only if for every $\epsilon$, the outcome $o$ occurs with positive measure in the ball of radius $\epsilon$ around $v$.
%\end{definition}
%
%\begin{observation}
%$\tilde f$ is upper hemicontinuous.
%\end{observation}
%\begin{proof}
%Pick any $v$ and neighborhood $\mathcal N$ of $v$ with positive measure. Suppose there is a sequence $\{v^k\}\rightarrow v$, and outcome $o_1$ such that $o_1\in\tilde f(v^k)$. Pick any $v^k\in\mathcal N$. Since $\mathcal N$ is also a neighborhood of $v^k$ and $o_1\in\tilde f(v^k)$, we can conclude that the set of points in $\mathcal N$ where $f=o_1$ has strictly positive measure.
%\end{proof}
%
%\begin{observation}\label{obs:f=fae}
%For any fixed $v_{-i}$, $f\in\tilde f$ almost everywhere in $v_i$.
%\end{observation}
%\begin{proof} It is sufficient to prove the lemma for an open subset $(z^l,z^h)^m\subset v_i$. First, fix any outcome $o_1$. For contradiction, suppose that there is a set $X\subseteq(o,u)^m$ of measure $>0$ such that $f(x)=o_1$ and $f\not\in\tilde f$ for all $x\in X$.  Pick any $z'\in(z^l,z^h)$ such that (1) the measure of $(z^l,z')$ and $(z',z^h)$ are both strictly positive in $\U$, and (2) the  so all of the $2^m$ sets defined by splitting each dimension of $v_i$ at $z'$ must also have strictly positive measure. Moreover, one of htose $2^m$ sets must contain a subset of $X$ with strictly positive measure. Recursing gives an arbitrarily small interval. Let $z^*$ be a point in all intervals (\textbf{TODO: show this exists}). By construction, 
%\end{proof}
%
%The first step is proving essential PAD/NAD for $\tilde f$. \textbf{TODO: tighten up AE in PAD/NAD. For example, it talks about AE in a ball in $\U^{mn}$, not in an individual bidder's value space.}
%
%\begin{claim}[Essential PAD]
%Let $\tilde f$ be extended map of a mechanism $M$ and let $v,v'$ be valuation profiles. If $o_1\in \tilde f(v)$ and for all $i$ and $o_2\neq o_1$ the outcome $o_1$ has a larger difference $v_i'(o_1)\ominus v_i(o_1)>v_i'(o_2)\ominus v_i(o_2)$, then $\tilde f(v')=\{o_1\}$.
%\end{claim}
%\begin{proof}
%Choose $\epsilon<\frac12\min_{o_2\neq o_1,i}(v_i'(o_1)\ominus v_i(o_1)\ominus(v_i'(o_2)\ominus v_i(o_2)))$. By definition of $\tilde f$, the set of points $X$ in the $\epsilon$ ball around $v$ where $f(x)=o_1$ has positive measure. Supposing no violations of incentive compatibility, we pick any $y$ in the $\epsilon$ ball around $v'$, and use ordinary PAD implies $f(y)=o_1$. If a violation of incentive compatibility occurs, it can be for at most a subset of $X$ with measure zero and a subset of the $\epsilon$ ball around $v'$ with measure zero. As a result, we can conclude that $f(y)=o_1$ almost everywhere within the $\epsilon$ ball around $v'$ and therefore $\tilde f(v')=\{o_1\}$.
%\end{proof}
%
%
%\begin{claim}[Essential NAD] Let $\tilde f$ be the extended map of a mechanism $M$. Let $v$ and $v'$ be valuation profiles and $o_1$ and $o_2$ outcomes such that $o_1\in\tilde f(v')$ and $v_i'(o_2)\ominus v_i(o_2)>v_i'(o_1)\ominus v_i(o_1)$, then $o_2\not\in\tilde f(v)$.
%\end{claim}
%\begin{proof}
%Similar to the proof of extended PAD, choose $\epsilon<\min_i(v_i'(o_2)\ominus v_i(o_2)\ominus(v_i'(o_1)\ominus v_i(o_1)))$. By definition of $\tilde f$, there is a set of points $Y$ in the $\epsilon$ ball around $o_1$ such that $f(y)=o_1$ and $Y$ has positive measure. Moreover, for any $x$ in the $\epsilon$ ball around $v$, ordinary NAD implies $f(x)\neq o_2$. Since violations of NAD can only occur on a set with measure zero, we can conclude that $f(x)\neq o_2$ almost everywhere in the $\epsilon$ ball around $v$ and therefore $o_2\not\in\tilde f(v)$.
%\end{proof}
%
%Next, we redefine $P$:
%\[P(o_1,o_2)=\{\Delta\in\U^n|\exists v\mbox{ s.t. }v(o_1)-v(o_2)=\Delta\mbox{ and }o_1\in\tilde f(v)\}\]
%The claims which rely on PAD/NAD go through, so now we need to show that we can construct the vectors $\gamma(o_1,o_2)$. We replace the definition as follows:
%\begin{definition}
%Given an arbitrary labeling of outcomes $o_1,\dots,o_m$, we define vectors $\gamma(o_j,o_k)\in\U^n$ as follows:
%\begin{enumerate}
%\item Let $G$ be a graph where the outcomes are the vertices and there is an edge between $o_j$ and $o_k$ if and only if we have found a value for $\gamma(o_j,o_k)$.
%\item Let $H$ be a graph where the outcomes are the vertices and there is an edge between $o_j$ and $o_k$ if and only if there is a bidder $i$ and a setting of values $v_{-i}$ such that $f(v_i,v_{-i})=o_j$ for a set of values $V_i$ with positive measure and $f(v_i',v_{-i})=o_k$ for another set of values $V_i'$ with positive measure.
%\item While $G$ has more than one connected component, identify an edge in $H$ that does not induce a cycle. This edge corresponds to a bidder $i$ and setting of others' values $v_{-i}$. Invoking the taxation principle, $i$'s menu includes outcome $o_1$ at a price $p_i(o_j)$ and outcome $o_k$ at a price $p_i(o_k)$. Set
%\[\gamma(o_j,o_k)=\ominus\gamma(o_k,o_j)=p_i(o_j)\ominus p_i(o_k)\]
%note this with an edge in $G$.
%\item While $G$ is not the complete graph, identify a triangle that can be completed, i.e. identify $o_j,o_k,o_l$ such that $\gamma(o_j,o_k)$ is not set but $\gamma(o_j,o_l)$ and $\gamma(o_l,o_k)$ are both set. Set
%\[\gamma(o_j,o_k)=\ominus\gamma(o_k,o_j)=\gamma(o_j,o_l)\oplus\gamma(o_l,o_k)\]
%\end{enumerate}
%\end{definition}
%\begin{claim}
%This defines all $\gamma$.
%\end{claim}
%\begin{proof} \textbf{TODO.}
%It is sufficient to prove that $H$ is connected. Remark that for any outcome pair $o_j,o_k$, there exist valuations $v$ and $v'$ such that $f(v)=o_j$ and $f(v')=o_k$. If we change bidders values from $v_i$ to $v_i'$ one by one, any time the outcome changes we get an edge in $H$. Since we start at $o_j$ and end at $o_k$, this implies there is a path from $o_j$ to $o_k$ in $H$ for any such pair, and therefore $H$ is connected.
%\end{proof}
%\begin{claim}
%$\gamma(o_j,o_k)\in P(o_j,o_k)$ and $\ominus\gamma(o_j,o_k)\in P(o_k,o_j)$
%\end{claim}
%\begin{proof}
%Suppose $\gamma$ was set in step (1). Fixing $v_{-i}$, let $v_i''$ be any valuation vector with $v_i''(o_j)=p_i(o_j)$ and $v_i''(o_k)=p_i(o_k)$. This is an indifference point for bidder $i$, so the sets of points where $i$ prefers $o_j$ and $o_k$ will have positive measure in any neighborhood of $v$.
%
%If $\gamma$ was set in step (2), the same reasoning as before applies since $\tilde f$ is upper hemicontinouous.
%\end{proof}
%
%
%
%
%Finally, we once again reference Observation~\ref{obs:f=fae} at the end to conclude that $f$ is an affine maximizer almost everywhere.
%










%
%\subsection{DSIC-AE TRY 2}
%
%Thus far we have extended Roberts's theorem to our topological vector space, but we are not done because we need to relax it to match DSIC-AE. To do this we study a ``smoothed'' mechanism that differs 
%
%\begin{definition}
%The smoothed mechanism $\tilde M$ for a mechanism $M$ is defined as follows:
%\begin{enumerate}
%\item For each $i$, $v_{-i}$ and $o$, let $\tilde p_i(o)$ be the minimum price $i$ pays
%\[\tilde p_i(o)=\min\{p_i(v_i,v_{-i})|f(v_i,v_{-i})=o\}\]
%\item For a vector $v$ and outcome $o$, say that $o$ is in the demand set $d(v)\subseteq\O$ if there exists a bidder $i$ and bid $b_i$ such that $b_i$ is a best response given $v_i$, $v_{-i}$, and $\tilde p_i$, and $f(b_i,v_{-i})=o$. We then say that the outcome $o$ is in the social choice correspondence $\tilde f(v)\in\O$ if there is a sequence of values $\{v^k\}\rightarrow v$ such that $o\in d(v^k)$ for all $k$.
%\end{enumerate}
%\end{definition}
%
%\begin{observation}
%$\tilde f$ is upper hemicontinuous by construction.
%\end{observation}
%
%\begin{observation}\label{obs:f=fae}
%For any fixed $v_{-i}$, $f\in\tilde f$ almost everywhere in $v_i$.
%\end{observation}
%\begin{proof} Fix $v_{-i}$. If truth-telling is a best response when $i$'s value is $v_i$, then $f(v)\in d(v)$ and the sequence $v^k=v$ proves that $f(v)\in\tilde f(v)$.
%\end{proof}
%\begin{corollary}
%$f\in\tilde f$ almost everywhere in $v$.
%\end{corollary}
%
%The first step is proving essential PAD/NAD for $\tilde f$. \textbf{TODO: tighten up AE in PAD/NAD. For example, it talks about AE in a ball in $\U^{mn}$, not in an individual bidder's value space.}
%
%\begin{claim}[Essential PAD]
%Let $\tilde f$ be extended map of a mechanism $M$ and let $v,v'$ be valuation profiles. If $o_1\in \tilde f(v)$ and for all $i$ and $o_2\neq o_1$ the outcome $o_1$ has a larger difference $v_i'(o_1)\ominus v_i(o_1)>v_i'(o_2)\ominus v_i(o_2)$, then $\tilde f(v')=\{o_1\}$.
%\end{claim}
%\begin{proof}
%Choose $\epsilon<\frac12\min_{o_2\neq o_1,i}(v_i'(o_1)\ominus v_i(o_1)\ominus(v_i'(o_2)\ominus v_i(o_2)))$. By definition of $\tilde f$, the set of points $X$ in the $\epsilon$ ball around $v$ where $f(x)=o_1$ has positive measure. Supposing no violations of incentive compatibility, we pick any $y$ in the $\epsilon$ ball around $v'$, and use ordinary PAD implies $f(y)=o_1$. If a violation of incentive compatibility occurs, it can be for at most a subset of $X$ with measure zero and a subset of the $\epsilon$ ball around $v'$ with measure zero. As a result, we can conclude that $f(y)=o_1$ almost everywhere within the $\epsilon$ ball around $v'$ and therefore $\tilde f(v')=\{o_1\}$.
%\end{proof}
%
%
%\begin{claim}[Essential NAD] Let $\tilde f$ be the extended map of a mechanism $M$. Let $v$ and $v'$ be valuation profiles and $o_1$ and $o_2$ outcomes such that $o_1\in\tilde f(v')$ and $v_i'(o_2)\ominus v_i(o_2)>v_i'(o_1)\ominus v_i(o_1)$, then $o_2\not\in\tilde f(v)$.
%\end{claim}
%\begin{proof}
%Similar to the proof of extended PAD, choose $\epsilon<\min_i(v_i'(o_2)\ominus v_i(o_2)\ominus(v_i'(o_1)\ominus v_i(o_1)))$. By definition of $\tilde f$, there is a set of points $Y$ in the $\epsilon$ ball around $o_1$ such that $f(y)=o_1$ and $Y$ has positive measure. Moreover, for any $x$ in the $\epsilon$ ball around $v$, ordinary NAD implies $f(x)\neq o_2$. Since violations of NAD can only occur on a set with measure zero, we can conclude that $f(x)\neq o_2$ almost everywhere in the $\epsilon$ ball around $v$ and therefore $o_2\not\in\tilde f(v)$.
%\end{proof}
%
%Next, we redefine $P$:
%\[P(o_1,o_2)=\{\Delta\in\U^n|\exists v\mbox{ s.t. }v(o_1)-v(o_2)=\Delta\mbox{ and }o_1\in\tilde f(v)\}\]
%The claims which rely on PAD/NAD go through, so now we need to show that we can construct the vectors $\gamma(o_1,o_2)$. We replace the definition as follows:
%\begin{definition}
%Given an arbitrary labeling of outcomes $o_1,\dots,o_m$, we define vectors $\gamma(o_j,o_k)\in\U^n$ as follows:
%\begin{enumerate}
%\item Let $G$ be a graph where the outcomes are the vertices and there is an edge between $o_j$ and $o_k$ if and only if we have found a value for $\gamma(o_j,o_k)$.
%\item Let $H$ be a graph where the outcomes are the vertices and there is an edge between $o_j$ and $o_k$ if and only if there is a bidder $i$ and a setting of values $v_{-i}$ such that $f(v_i,v_{-i})=o_j$ for a set of values $V_i$ with positive measure and $f(v_i',v_{-i})=o_k$ for another set of values $V_i'$ with positive measure.
%\item While $G$ has more than one connected component, identify an edge in $H$ that does not induce a cycle. This edge corresponds to a bidder $i$ and setting of others' values $v_{-i}$. Invoking the taxation principle, $i$'s menu includes outcome $o_1$ at a price $p_i(o_j)$ and outcome $o_k$ at a price $p_i(o_k)$. Set
%\[\gamma(o_j,o_k)=\ominus\gamma(o_k,o_j)=p_i(o_j)\ominus p_i(o_k)\]
%note this with an edge in $G$.
%\item While $G$ is not the complete graph, identify a triangle that can be completed, i.e. identify $o_j,o_k,o_l$ such that $\gamma(o_j,o_k)$ is not set but $\gamma(o_j,o_l)$ and $\gamma(o_l,o_k)$ are both set. Set
%\[\gamma(o_j,o_k)=\ominus\gamma(o_k,o_j)=\gamma(o_j,o_l)\oplus\gamma(o_l,o_k)\]
%\end{enumerate}
%\end{definition}
%\begin{claim}
%This defines all $\gamma$.
%\end{claim}
%\begin{proof} \textbf{TODO.}
%It is sufficient to prove that $H$ is connected. Remark that for any outcome pair $o_j,o_k$, there exist valuations $v$ and $v'$ such that $f(v)=o_j$ and $f(v')=o_k$. If we change bidders values from $v_i$ to $v_i'$ one by one, any time the outcome changes we get an edge in $H$. Since we start at $o_j$ and end at $o_k$, this implies there is a path from $o_j$ to $o_k$ in $H$ for any such pair, and therefore $H$ is connected.
%\end{proof}
%\begin{claim}
%$\gamma(o_j,o_k)\in P(o_j,o_k)$ and $\ominus\gamma(o_j,o_k)\in P(o_k,o_j)$
%\end{claim}
%\begin{proof}
%Suppose $\gamma$ was set in step (1). Fixing $v_{-i}$, let $v_i''$ be any valuation vector with $v_i''(o_j)=p_i(o_j)$ and $v_i''(o_k)=p_i(o_k)$. This is an indifference point for bidder $i$, so the sets of points where $i$ prefers $o_j$ and $o_k$ will have positive measure in any neighborhood of $v$.
%
%If $\gamma$ was set in step (2), the same reasoning as before applies since $\tilde f$ is upper hemicontinouous.
%\end{proof}
%
%
%
%
%Finally, we once again reference Observation~\ref{obs:f=fae} at the end to conclude that $f$ is an affine maximizer almost everywhere.
%
%
%


==> roberts-sketch.tex <==


\section{Value Maximizers as Quasilinear Agents}  \label{sec:roberts}

In Section~\ref{sec:value-max} we saw that transformed greedy mechanisms are generally truthful, even in the most complex valuation models. In this section, we offer evidence that we cannot expect to find mechanisms far outside this class. In the process, we show how our greedy mechanisms can be interpreted as ``affine maximizers'' in an appropriate vector space, shedding light on the parallels between our greedy mechanisms and VCG/affine maximizers.

From the perspective of a social planner, these can be seen as negative results. They imply that the planner can do little more than satisfy the agent who achieves the maximum value, leading to provably-poor welfare guarantees.

The key idea behind our results in this section is that we can write a {\em quasilinear utility function} that represents value maximizing behavior when values and prices are drawn from a set $\U$ instead of $\Re$:
\begin{definition*}[Informal.]
The topological vector space $\U$ is a lexicographically ordered function space in which quasilinear utilities correspond to value maximizing preferences.
\end{definition*}
Once we are working with quasilinear utilities in $\U$ we can generalize existing results. Specifically, we generalize Roberts's Theorem, which states that whenever there are at least 3 distinct outcomes and each bidder's valuation is unrestricted, the only DSIC mechanisms are affine maximizers:
\begin{theorem*}[Informal.]
The only deterministic truthful mechanisms ($|\O|\geq 3$) for bidders with unrestricted quasilinear utilities in $\U$ (rather than $\Re$), the only truthful mechanisms are generalized affine maximizers.
\end{theorem*}
\begin{observation*}[Informal.]
Generalized affine maximizers for the vector space $\U$ correspond with transformed greedy mechanisms.
\end{observation*}
We also need to relate mechanisms in $\U$ space to mechanisms for regular value maximizers. The mapping between $\U$ and $\Re$ is inherently lossy, necessitating that we work with DSIC-AE mechanisms as follows:
%\begin{theorem*}[Informal.]
%The only deterministic DSIC-AE mechanisms ($|\O|\geq3$) for bidders with quasilinear utilities in $\Re$ are affine maximizers.
%\end{theorem*}
\begin{lemma*}[Informal.]
A DSIC-AE mechanism for value maximizers is DSIC-``AE'' for $\U$-space bidders when values and prices are transformed according to a natural mapping, and vice-versa.
\end{lemma*}
Together, these results clearly demonstrate that greedy mechanisms are the central truthful mechanisms for value maximizers; however, we fall short of proving that they are the only truthful mechanisms because we are at present unable to bridge the gap between DSIC and DSIC-``AE'' for $\U$-space mechanisms.\footnote{Generalizing Roberts's Theorem to DSIC-AE is doable for ordinary quasilinear bidders, but an analogous result in $\U$ space would use the wrong measure and therefore fail to characterize DSIC-``AE'' mechanisms.}



\subsection{The Utility Space}

First, we introduce the vector space that will allow us to write quasilinear utilities for value maximizers:
\begin{definition}
The {\em utility space} $\U$ is the function space over functions $u:\Re\rightarrow\Re$ that are non-zero at a finite number of non-negative inputs combined with the standard addition ($\oplus$), subtraction ($\oplus$), multiplication by a scalar, and lexicographic ordering ($\geq$) for functions.
\end{definition}
If we write an element $u$ as a function $u(x)$, the operations of addition and subtraction, as well as the ordering, can be thus written as follows:
\begin{itemize}
\item {\em Addition ($\oplus$) and subtraction ($\ominus$):} $u_3=u_1\oplus u_2$ if and only if $u_3(x)=u_1(x)+u_2(x)$ for all $x$.
\item {\em Multiplication ($\times$) by a scalar $s\in\Re$:} $u_2=s\times u_1$ if and only if $u_2(x)=s\times u_1(x)$ for all $x$.
\item {\em Ordering ($\geq$):} Let $u_1,u_2$ be elements of $\U$ and $x_1=\max\{x|u_1(x)\neq u_2(x)\}$ be the maximum value at which the two functions differ,\footnote{They can only differ at a finite number of points $x$ since they are nonzero only on a finite number of points, hence $x_1$ is well-defined.} then $u_1\geq u_2$ if and only if $u_1(x_1)\geq u_2(x_1)$.
\end{itemize}
Instead of writing $u$ as a function, we often write it as a finite set of pairs $\{(x_k,w_k)\}$ where $x_k$ represents the point at which the function $u(x)$ is nonzero and $w_k\in\Re$ denotes the value of the function $u(x_k)$. We index the pairs so $x_1>x_2>\dots\geq 0$.


The most important feature of $\U$ is that an agent who maximizes utility in $\U$ space will have lexicographic preferences like a value maximizer:
\begin{observation}
Given a finite set of outcome-price pairs $(o,p_i(o))$ where $p_i(o)\in\U$, an agent with values $v_i(o)\in\U$ who maximizes $v_i(o)\ominus p_i(o)$ will behave exactly like a value maximizer except when $v_i(o)=p_i(o)$ (here the quasilinear bidder is indifferent, the value maximizer is not).
\end{observation}
This is easiest to intuit through an example:
\begin{example}
Suppose there are two outcomes $o_1$ and $o_2$. Let $i$'s value be $v_i(o_1)=\{(2,1)\}$ and $v_i(o_2)=\{(1,1)\}$, and let prices be $p_i(o_1)=\{(1.5,1)\}$ and $p_i(o_2)=\{(0.25,1)\}$. We can then write $v_i(o_1)\ominus p_i(o_1)=\{(2,1),(1.5,-1)\}$ and $v_i(o_2)\ominus p_i(o_2)=\{(1,1),(0.25,-1)\}$. According to the lexicographic ordering, $o_1$ is preferred because $(2,1)>(1.5,1)$.
\end{example}



Another useful insight is that is that our greedy mechanisms are like ``VCG mechanisms'' in $\U$ space in the sense that they maximize $\sum_iv_i(o)$ and charge externality payments:
\begin{observation}
The non-transformed greedy mechanism (informally) maximizes $\U$-welfare and charges $\U$-externality prices.
\end{observation}
Again, this is easiest to intuit through an example. (We will establish a formal relationship later.) We revisit Example~\ref{ex:greedy} in $\U$-space:

%\begin{example}\label{ex:greedy}
%Suppose there are three outcomes $\{o_1,o_2,o_3\}$ and four bidders with values $v_1=\{3,3,1\}$, $v_2=\{0.5,1,1\}$, $v_3=\{2,1,0\}$, and $v_4=\{0.5,0.5,0.5\}$.
%
%The greedy maximizing auction for value maximizers chooses outcome $o_1$ as follows:
%\begin{enumerate}
%\item The value of the highest-value bidder is maximized by taking either outcome $o_1$ or $o_2$ ($v_1=3$).
%\item Among outcomes $o_1$ and $o_2$, the value of the second-highest-value bidder is maximized by taking $o_1$ ($v_3=2$).
%\end{enumerate}
%To compute prices, observe that the auction would still choose $o_1$ if bidder 1, 2, or 4 were removed from the auction, so these bidders pay $p_{\{1,2,4\}}=0$. For bidder 3, notice that the outcome would be $o_2$ if it were removed ($v_2=1$). Neither bidder 1 nor bidder 4 care whether the outcome is $o_1$ or $o_2$, but bidder 2 gets $v_2=1$ from $o_2$ instead of $v_2=0$ from $o_1$. The price bidder 3 pays is bidder 2's value for $o_2$, i.e. $p_3=v_2(o_2)=1$.
%\end{example}

\begin{example}
Suppose there 3 bidders and 4 outcomes, with values summarized in the following table:
\begin{center}
\begin{tabular}{rcccc}
Bidder&1&2&3&4\\
$v_i(o_1)$&$\{(3,1)\}$&$\{(0.5,1)\}$&$\{(2,1)\}$&$\{(0.5,1)\}$\\
$v_i(o_2)$&$\{(3,1)\}$&$\{(1,1)\}$&$\{(1,1)\}$&$\{(0.5,1)\}$\\
$v_i(o_3)$&$\{(1,1)\}$&$\{(1,1)\}$&$\{\}$&$\{(0.5,1)\}$
\end{tabular}
\end{center}
A ``welfare''-maximizing mechanism in $\U$ space computes the $\U$-welfare for each outcome as
\begin{align*}
W(o_1)&=\sum_iv_i(o_1)=\{(3,1),(2,1),(0.5,2)\}\\
W(o_2)&=\sum_iv_i(o_2)=\{(3,1),(1,2),(0.5,1)\}\\
W(o_3)&=\sum_iv_i(o_3)=\{(1,2),(0.5,1)\}
\end{align*}
and then chooses $o_1$ since $W(o_1)$ is lexicographically maximum. This coincides with the choice of the greedy mechanism in Example~\ref{ex:greedy}.

The $\U$-space mechanism then computes prices as externalities. Again, the only bidder whose presence changes the outcome of the auction is bidder 3 --- without bidder 3 the outcome would be $o_2$. We can compute bidder 3's externality price as
\[p_3=(\{(3,1)\}\oplus\{(1,1)\}\oplus\{(0.5,1\})\ominus(\{(3,1)\}\oplus\{(0.5,2)\})=\{(1,1),(0.5,-1)\}\]
The $(1,1)$ term will generally dominate in arithmetic and ordering, so this is analogous to the greedy mechanism that charged $p_3=1$.
\end{example}
%\begin{example}
%Suppose there 3 bidders and 3 outcomes, summarized in the following table:
%\begin{center}
%\begin{tabular}{rccc}
%Bidder&1&2&3\\
%$v_i(o_1)$&$\{(5,1)\}$&$\{(3,1)\}$&$\{(1,1)\}$\\
%$v_i(o_2)$&$\{(1,1)\}$&$\{(4,1)\}$&$\{(1,1)\}$\\
%$v_i(o_3)$&$\{(5,1)\}$&$\{(1,1)\}$&$\{(2,1)\}$
%\end{tabular}
%\end{center}
%The greedy mechanism chooses $o_1$ because $v_1(o_1)=\{(5,1)\}$ and then $v_2(o_1)=\{(3,1)\}$. Notice that the $\U$ welfare for $o_1$ is $W(o_1)=\sum_iv_i(o_1)=\{(5,1),(3,1),(1,1)\}$, which is lexicographically greater than $W(o_2)=\{(4,1),(1,2)\}$ and $W(o_3)=\{(5,1),(2,1),(1,1)\}$. Thus, it matches the greedy choice.
%
%Computing the externality for bidder 1, the greedy/$\U$-welfare optimal outcome without bidder 1 would be $o_2$ because $v_2(o_2)=\{(4,1)\}$. We can thus write bidder 1's externality as
%\[ext_1=(\{(4,1)\}\oplus\{(1,1)\})\ominus(\{(3,1)\}\oplus\{(1,1)\})=\{(4,1),(3,-1)\}\]
%The $(4,1)$ term will generally dominate in arithmetic and ordering, this is analogous to our greedy mechanism that charges 4.
%
%Computing an externality or bidder 2, the greedy/$\U$-welfare optimal outcome without bidder 2 would be $o_3$ because $v_3(o_3)=\{(2,1)\}$. We can thus write bidder 2's externality as
%\[ext_1=(\{(5,1)\}\oplus\{(1,1)\})\ominus(\{(5,1)\}\oplus\{(2,1)\})=\{(2,1),(1,-1)\}\]
%By comparison, our greedy mechanism would charge 2 because, though bidder 1 had the highest value for $o_3$, its value for $o_3$ was the same as its value for $o_1$. This is equivalent to the dominant $(2,1)$ term.
%\end{example}

\subsection{Proving a ``Roberts's Theorem'' for $\U$}

Next, we need to characterize mechanisms in $\U$ space. For traditional quasilinear bidders, Roberts characterizes truthful mechanisms in unrestricted domains as affine maximizers, that is, there exist weights $w_i$ and offsets $\gamma(o)$ such that the mechanism always picks $o\in\argmax \sum_iw_iv_i(o)-\gamma(o)$. To generalize affine maximization to $\U$ we must define it terms of linear functions: 
\begin{definition}
We say that a mechanism is a {\em generalized affine maximizer} if there are linear functions $h_i$ with offsets $\gamma(o)$ such that the mechanism always picks $o\in\argmax \sum_ih_i(v_i(o))\ominus\gamma(o)$.
\end{definition}
Existing results are known to generalize to various topological vector spaces (e.g.~\cite{Carbajal13}), but we are unaware of any version that explicitly considers payments and values that are not in real numbers, so we present a generalization following first proof of Lavi et al.~\cite{lavi08}. The resulting theorem, proven in Appendix~\ref{sec:roberts-proof}, leverages an infinite-dimensional version of the separating hyperplane theorem~\cite{borderNotes}:
\begin{theorem}\label{thm:vm-rt}
When $3\leq |\O|<\infty$ and both values and payments may be arbitrary values in $\U$, the only mechanisms that are DSIC are generalized affine maximizers.
\end{theorem}

\subsection{Mapping Between $\Re$ and $\U$}

To move between $\Re$ and $\U$ we need to define a mapping from values in $\Re$ to values in $\U$ and back again:
\begin{itemize}
\item $\tau:\Re\rightarrow\U$ maps $x\in\Re$ to $\tau(x)=\{(x,1)\}$.
\item $\tau^{-1}:\U\rightarrow\Re$ maps $\{(a^k,b^k)\}\in\U$ to a real number as $\tau^{-1}(\{(a^k,b^k)\})=sign(w_1)\times a_1$
\end{itemize}
When applied to a vector in $\U^m$ we apply $\tau$ or $\tau^{-1}$ to each coordinate individually. We can now talk about running a mechanism for $\U$-space maximizers when bidders are actually real-space value maximizers, or vice versa, simply by converting values and prices with $\tau$ and $\tau^{-1}$.


\subsection{Generalized Affine Maximizers in $\U$}

Theorem~\ref{thm:vm-rt} is initially somewhat opaque --- while it is useful to know that mechanisms must be generalized affine maximizers, it is initially unclear what exactly that means. It turns out that, when mapped back to value maximizers, they correspond to our greedy mechanisms.

First, we note that linear functions in $\U$ are substantially more diverse than linear functions in $\Re$:
\begin{observation}\label{obs:u-linear}
A function $h:\U\rightarrow\U$ is linear if and only if it can be written as $h(u)=\sum_{k} w_k\times z(a_{k})$ where $z(x):\Re\rightarrow\U$ maps each real number with an element of $\U$.\footnote{So see this, let $z(x)=h(\{(x,1)\})$.} $h$ is monotone if and only if each $z(a_{k})$ is monotone in $a_{k}$.
\end{observation}
This diversity explains the apparent contrast between Roberts's characterization of mechanisms as affine maximizers and our transformed greedy maximizers. Roberts's affine maximizers scaled bidders' values by weights, but other transformations were forbidden, whereas our greedy mechanism is truthful for arbitrary monotone transformations of value, since the space of linear transformations is more diverse.

We can now informally map generalized affine maximizers back to mechanisms for value maximizers (a formal relationship follows later):
\begin{observation}
A generalized affine maximizer for $\U$-space bidders (informally) corresponds to our transformed greedy mechanism.
\end{observation}
\begin{proof}[Proof sketch.]
Let $z_i(x)$ denote the function $z(x)$ associated with the monotone linear function $h_i$ following Observation~\ref{obs:u-linear}. 

First, suppose that $\tau^{-1}(z_i(x))$ is strictly increasing in $x$. This implies the dominant term of $h_i(v_i(o))$ is strictly increasing in $v_i$. Since the lexicographic ordering is dominated by the highest-order term, we can intuitively ``drop'' everything except the dominant term of $h_i(v_i(o))$. Writing $\theta_i(x)=\tau^{-1}(z_i(x))$ we then claim
\[h_i(v_i(o))\sim \{(\theta_i(a_1),1)\}\]
A mechanism that maximizes $h_i(v_i(o))$ is therefore like the greedy mechanism with $\theta_i(x)=\tau^{-1}(z_i(x))$.

When $\tau^{-1}(z_i(x))$ is not strictly increasing in $x$, it means that low-order terms of $x_i(x)$ break the tie ($z_i(x)$ is strictly increasing in $x$). Since the domain of $z_i$ is the reals, it is straightforward to show that we can construct $\theta_i$ functions that preserve the ordering between bidders.
\end{proof}







\subsection{Reducing Between $\Re$ and $\U$}

We have seen that, informally, we can relate mechanisms for value maximizers and mechanisms for $\U$-bidders. Here, we formalize this connection through the transformation $\tau$. To do this, we first need to introduce an equivalent to DSIC-AE in $\U$ space that will be compatible with DSIC-AE for regular value maximizers: 
\begin{definition}
A mechanism for quasilinear bidders in $\U$ space is DSIC-``AE'' if and only if, for any $v_{-i}$, the set
\[X=\{x\in\Re^m|\exists v_i\mbox{ such that }x=\tau^{-1}(v_i)\mbox{ and truth-telling is not a best-response for $i$\}}\]
has measure 0 according to the standard Lebesgue measure on $\Re^m$.
\end{definition}
In essence, this definition focuses on the dominant terms $\tau^{-1}(v_i(o))$ and says that according to the standard measure, the set of values on which there is an incentive to lie should be zero.


Using this definition, we can show that mechanisms for value maximizers are equivalent to mechanisms for $\U$-space bidders. The following lemma says that using the natural mapping $\tau$ between $\Re$ and $\U$, a mechanism for value maximizers can be converted to a mechanism for $\U$-space bidders and vice versa:
\begin{lemma}
A DSIC-AE mechanism for value maximizers is DSIC-``AE'' for $\U$-space bidders when values and prices are transformed according to $\tau$, and vice-versa.
\end{lemma}
\begin{corollary}\label{cor:u-reduction}
If the only DSIC-``AE'' mechanisms for $\U$-space bidders are transformed greedy mechanisms (almost everywhere), then the only DSIC-AE mechanisms for value maximizers are also transformed greedy mechanisms (almost everywhere).
\end{corollary}

\begin{proof}
We first prove that a mechanism that is DSIC-AE for value maximizers is DSIC-``AE'' for $\U$-space bidders, since this direction is required for Corollary~\ref{cor:u-reduction} and is perhaps more surprising. The converse argument will be analogous.

Let $M$ be a mechanism that is DSIC-AE for value maximizers. We run $M$ for $\U$-space bidders as follows:
\begin{enumerate}
\item Solicit bids $b_i\in\U^m$. Transform them to bids $\beta_i\in\Re^m$ as $\beta_i=\tau^{-1}(b_i)$.
\item Run $M$ on the bids $\beta_i$ to get an outcome $o^*$ and prices $\pi_i\in\Re$.
\item Transform prices $\pi_i$ into $p_i\in\U$ as $p_i=\tau(\pi_i)$.
\end{enumerate}
We want to analyze when a bidder $i$ might prefer to lie. Fix reports $b_{-i}$, and suppose that $v_i$ is such that truth-telling is a best-response for $i$ assuming it was a value maximizer with true value $\tau^{-1}(v_i)$. By the taxation principle, we can write $\pi_i(o)\in\Re$ and $p_i(o)\in\U$ as the prices that bidder $i$ would pay if the outcome is $o$, and we talk about $i$ choosing from this menu. There are only a handful of scenarios in which $i$ might wish to choose an outcome other than $o^*$ (i.e. to lie):
\begin{itemize}
\item If $\beta_i(o^*)\geq p_i(o^*)$...
\begin{itemize}
\item An outcome $o^+\neq o^*$ where $v_i(o^+)>v_i(o^*)$ was not a profitable deviation in $M$ because $\beta_i(o^+)<\pi_i(o)$; however after the transformation it becomes profitable $v_i(o)\geq p_i(o)$. {\em This is impossible.}
\item The optimal outcome $o^*$ was a best-response in $M$ with $\beta_i(o^*)\geq \pi_i(o^*)$, but after the transformation $v_i(o)<p_i(o)$ and so it is no longer $i$'s preferred outcome. {\em This can only happen if $\tau^{-1}(v_i(o))=\pi_i(o)$.}
\item An outcome $o^+\neq o^*$ where $v_i(o^+)>v_i(o^*)$ had $\beta_i(o^+)\leq\beta_i(o^*)$ because of information loss in $\tau^{-1}$. {\em This can only happen when $\tau^{-1}(v_i(o^+))=\tau^{-1}(v_i(o^*))$.}
\end{itemize}
\item If $\beta_i(o^*)< p_i(o^*)$...
\begin{itemize}
\item An outcome $o^+\neq o^*$ had $\beta_i(o^+)<p_i(o^+)$ but after the transformation has $v_i(o^+)\geq p_i(o^+)$. {\em This is impossible.}
\item An outcome $o^+\neq o^*$ had $\pi_i(o^+)> \pi_i(o^*)$ but after the transformation has $p_i(o^+)< p_i(o^*)$. {\em This is impossible.}
\item An outcome $o^+\neq o^*$ had $\pi_i(o^+)=\pi_i(o^*)$ and $\beta_i(o^+)=\beta_i(o^*)$ but $v_i(o^+)>v_i(o^*)$. {\em This can only happen when $\tau^{-1}(v_i(o^+))=\tau^{-1}(v_i(o^*))$.}
\end{itemize}
\end{itemize}
The three scenarios above that are possible each happen for very specific dominant terms in $v_i$, and specifically with measure 0 over the space of $\tau^{-1}(v_i)$. Thus, their union has measure zero.

One scenario remains --- that $(\beta_{-i},\tau^{-1}(v_i))$ is a valuation for which truth-telling was not a best response for $i$ in $M$. By definition of DSIC-AE, this happens with measure 0 as well.
\end{proof}




Unfortunately, this does not close the loop because we have not characterized DSIC-``AE'' mechanisms as would be required to apply Corollary~\ref{cor:u-reduction}. Thus, it remains possible that DSIC-``AE'' mechanisms exist which are somehow different from generalized affine maximizers in $\U$. However, our results are strong evidence that even if a gap exists, our greedy mechanisms are the canonical mechanisms for value maximizers and any others are unlikely to be far from the generalized affine maximizers of $\U$.


==> roberts-sketch2-short.tex <==


\section{Value Maximizers as Quasilinear Agents}  \label{sec:roberts-short}

We have seen how value maximizers behave quite differently from traditional quasilinear agents. In this final section we will explore a connection between them: value maximizers act like agents with quasilinear utilities in an alternative vector space. Recall that the VCG mechanism for quasilinear bidders will maximize $OBJ(o)=\sum_iv_i(o)$ while the greedy mechanism for value maximizers will maximize $OBJ(o)=\max_i v_i(o)$. Intuitively, we will rewrite preferences and mechanisms replacing `$+$' with `$\max$'. Executing this substitution requires that we introduce a new vector space with a lexicographic ordering; when values and payments are elements in this vector space, quasilinear ``utilities'' look like value maximizers and greedy mechanisms look like VCG; a more detailed treatment can be found in the full version of the paper. %Appendix~\ref{sec:roberts}.

Formally, let $\U$ be a vector space containing all functions $u:\Re_+\rightarrow\Re$ that are non-zero at a finite number of inputs. The operations of addition ($\oplus$), subtraction ($\ominus$), and multiplication by a scalar ($\times$) are defined in the usual way for functions:
\[c=x\times a\ominus y\times b\quad\Leftrightarrow\quad\forall s:\enspace c(s)=x a(s)-y b(s)\]
where $a,b,c\in\U$ are functions and $x,y\in\Re$ are real numbers. Distinct elements $a,b\in\U$ are ordered according to the standard lexicographic ordering on $\U$: let $s^+=\max\{s|a(s)\neq b(s)\}$ (this is well-defined because we required $a$ and $b$ to have a finite number of non-zero entries), then
\[a\geqslant b\quad\Leftrightarrow\quad a(s^+)\geq b(s^+)\enspace.\]

A value maximizer's preference among a menu of value-price pairs $(v^k,p^k)$ can be expressed by a quasilinear utility in $\U$ space. Each real value $v^k$ and price $p^k$ is mapped to a function in $\U$ space that is 1 at $v^k$ (resp. $p^k$) and zero everywhere else; the utility of each pair is the difference of the value and price:
%
\begin{align*}
u^k(s) = \;&\left(\begin{cases}1&s=v^k\\0&\textrm{otherwise}\end{cases}\right)-\left(\begin{cases}1&s=p^k\\0&\textrm{otherwise}\end{cases}\right)
\\ =\; &\begin{cases}1&s=v^k\\-1&s=p^k\\0&\textrm{otherwise}\end{cases}\enspace.
\end{align*}
%
The lexicographic ordering over $u^k$ corresponds to a value maximizer's preference over value-price pairs as long as $v^k\neq p^k$. Moreover, the greedy mechanism (and transformed variants) can be implemented as follows: transform values into $\U$-space functions, run VCG  in $\U$ space using $\oplus$ and $\ominus$ to compute each outcome's welfare and bidders' externality payments, and finally transform the payments back by identifying the largest input at which the price function is nonzero. %A worked example can be seen in Appendix~\ref{sec:roberts-examples}.


More generally, we can construct nearly-truthful mechanisms for value
maximizers from truthful mechanisms for $\U$-space agents and vice-versa. When
we transform a real number $x\in\Re$ to or from a function $a\in\U$, $x$
corresponds to the largest input to $a$ that is non-zero, i.e.,
$x=\max\{s|a(s)\neq 0\}$, the most-significant term of $a$. As long as they are
distinct, these most-significant terms will uniquely determine the ordering of
elements of $\U$ and therefore the preferences of a $\U$-space bidder. Thus,
when values and payments are transformed appropriately, a mechanism that is
truthful for $\U$ space bidders will be truthful for value maximizers under
most valuation profiles (in a technical sense that we elaborate in a longer version of the paper). %, see Appendix~\ref{sec:roberts}).
Likewise, a mechanism for value maximizers will yield a truthful mechanism for
$\U$-space agents under most valuations.

Finally, viewing value maximizers as quasilinear agents raises a tantalizing
question: {\em does an analog of Roberts's theorem hold for value maximizers?}
Roberts's Theorem says in certain quasilinear domains, the only mechanisms that
can be implemented truthfully are a generalization of VCG known as affine
maximizers. In a longer version of the paper \if Appendix~\ref{sec:roberts-roberts} \fi we show that this generalizes
to $\U$-space, where affine maximizers are related to our transformed greedy
mechanisms. Tying this characterization back to mechanisms for value maximizers
stands as an open question, and would show that transformed greedy mechanisms
are the only truthful mechanisms for value maximizers.



==> roberts-sketch2.tex <==


\section{More on Value Maximizers as Quasilinear Agents}  \label{sec:roberts}

In Section~\ref{sec:roberts} we showed how value maximizers could be viewed as quasilinear agents in an alternative vector space. In this section we formalize many of the ideas mentioned earlier.

\subsection{Wishful Thinking and Intuition}

We start with an observation and a bit of wishful thinking. A welfare-maximizing mechanism for quasilinear bidders will maximize $OBJ(o)=\sum_iv_i(o)$ while the greedy mechanism will maximize $OBJ(o)=\max_i v_i(o)$. Given that `$\max$' is commutative and associative like `$+$', {\em can we apply the standard theory by substituting `$\max$' for `$+$' as appropriate?} Unfortunately, simply replacing `$+$' with `$\max$' is too simple, but it sets up our approach: we identify an abstract addition operation $\oplus$ for which quasilinear utilities behave like value maximizing preferences.

The primary obstacle to this naive approach is that `$\max$' discards information about low-order terms. For example, $\max(1,2)=\max(1.5,2)=2$, so we lose information about whether the smaller term was 1 or 1.5. This obstacle manifests itself in two ways. First, blindly substituting `$\max$' fails to break ties in the way the greedy mechanism does: when $\max_iv_i(o)=\max_iv_i(o')$ for distinct outcomes $o$ and $o'$, the greedy mechanism looks at the next-highest value, if there is a tie in the next-highest value it looks at the third-highest, and so on; writing $OBJ(o)=v_1(o)\oplus\dots\oplus v_n(o)=\max_iv_i(o)$ does not contain enough information to do this. Second, using `$\max$' we cannot write quasilinear utilities $u=v\ominus p$. For example, we would want $(1\oplus 2)\ominus2=1$ and $(1.5\oplus2)\ominus 2=1.5$, but  since $\max(1,2)=\max(1.5,2)=2$ this is impossible.

To make progress, we must encode not only the max element but also low-order terms, as well as accommodating negative values. In effect, $a\oplus b\oplus c$ must correspond to the set $\{a,b,c\}$ and, to allow subtraction, $a\oplus b\ominus a\ominus c$ must be something like $\{b,-c\}$. This motivates the structure that we will formally define below: we treat values and prices as weighted sets, where the weights represent the number of occurrences (possibly negative) and  $\oplus$ and $\ominus$ are the operations that perform natural addition/subtraction on the weights; weighted sets are compared lexicographically.

\subsection{The Vector Space $\U$: Definition and Preliminaries}

Our first technical step is to introduce a vector space $\U$ in which value maximizers have quasilinear preferences. As motivated above, each element $u\in\U$ will be a weighted set of non-negative real numbers. Below we formalize $\U$ in two equivalent ways and introduce the standard operations ($\oplus$, $\ominus$, $\times$), the ordering $\geqslant$, and a transformation for mapping between $\Re$ and $\U$.

\paragraph{Sparse Representation of $u\in\U$.} Our intuition above suggests a sparse representation where an element $u\in\U$ is written as a finite list of number-weight pairs $(s,w)$ where $s$ represents the number in the set and $w$ its associated weight:
\[u=\{(s^1,w^1),\dots,(s^k,w^k),\dots,(s^K,w^K)\}\enspace.\]
Since the values $s^k$ represent a set they are distinct, and WLOG we label them so that $s^1>s^2>\dots s^K>0$.

\paragraph{Dense Representation of $u\in\U$.} In dense form, an element $u\in\U$ is a function $u:\Re^+\rightarrow\Re$ that is non-zero at a finite number of inputs. For example, if $u=\{(s^1,w^1),\dots,(s^k,w^k),\dots,(s^K,w^K)\}$ in sparse form, then
\[u(s)=\begin{cases}w^k&s=s^k\\0&\mbox{otherwise.}\end{cases}\]
From this perspective $\U$ contains all functions in the function space $\Re^+\rightarrow\Re$ having a finite number of non-zero values.

\paragraph{Addition and Subtraction ($\oplus$/$\ominus$) on $\U$.} Addition and subtraction correspond to adding subtracting the weights associated with the set variables $s^k$. They are most easily defined through the dense representation, where they are simply the natural addition and subtraction operations on functions:
\[c=a\oplus b\quad\Leftrightarrow\quad \forall s:\enspace c(s)=a(s)+b(s)\]
where $a,b,c\in\U$. Likewise $c=a\ominus b\Leftrightarrow\forall s: c(s)=a(s)-b(s)$.

\paragraph{Multiplication by a Scalar ($\times$) on $\U$.} A scalar multiplier is applied to the weights, i.e. if $a,b\in\U$ and $x\in\Re$, then
\[b=x\times a\quad\Leftrightarrow\quad\forall s:\enspace b(s)=x\times a(s)\enspace.\]

\paragraph{Ordering ($\geqslant$) on $\U$.} Elements of $u$ are ordered lexicographically. Let $a$ and $b$ be distinct elements of $\U$ and let $s^+=\max\{s|a(s)\neq b(s)\}$.\footnote{$s^+$ is well-defined because we stipulate that $a(s),b(s)\neq0$ at a finite number of points.} Using the dense representation we say
\[a\geqslant b\quad\Leftrightarrow a(s^+)\geq b(s^+)\enspace.\]
This is the natural lexicographic ordering on $\U$.\footnote{The lexicographic ordering is not generally a total ordering over the function space $\Re^+\rightarrow\Re$, it is a total ordering when the space is restricted to functions with a finite number of non-zero elements.}


\paragraph{Transforming $\Re\leftrightarrow\U$.} Since our initial setting has values as real numbers, i.e. $v_i(o)\in\Re$, we will need a mapping $\tau:\Re\rightarrow\U$ to transform a real number into an element of $\U$, as well as a pseudo-inverse $\tau^{-1}$ to transform the other direction:
\begin{itemize}
\item $\tau:\Re\rightarrow\U$ maps $x\in\Re$ to $\tau(x)=\{(x,1)\}$.
\item $\tau^{-1}:\U\rightarrow\Re$ maps $\{(s^k,w^k)\}\in\U$ to a real number as $\tau^{-1}(\{(s^k,w^k)\})=sign(w^1)\times a_1$
\end{itemize}
When applied to a vector in $\U^m$ we apply $\tau$ or $\tau^{-1}$ to each coordinate individually.

%We can now talk about running a mechanism for $\U$-space maximizers when bidders are actually real-space value maximizers, or vice versa, simply by converting values and prices with $\tau$ and $\tau^{-1}$.

\subsection{Examples of $\U$-Quasilinear Preferences and Mechanisms}\label{sec:roberts-examples}

Some intuition for $\U$ can be gained through examples. First, we remark that a $\U$-space agent with quasilinear preferences looks like a value maximizer:
\begin{observation}
Given a finite set of outcome-price pairs $(o,p_i(o))$ where $p_i(o)\in\U$, an agent with values $v_i(o)\in\U$ who maximizes $v_i(o)\ominus p_i(o)$ will pick an outcome-price pair maximizing $v_i(o)$ subject to the constraint that $v_i(o)>p_i(o)$, that is, she will behave exactly like a value maximizer except when $v_i(o)=p_i(o)$ (here the quasilinear bidder is indifferent to non-participation, the value maximizer is not).
\end{observation}
\begin{example}
Suppose there are two outcomes $o_1$ and $o_2$. Let $i$'s value be $v_i(o_1)=\{(2,1)\}$ and $v_i(o_2)=\{(1,1)\}$, and let prices be $p_i(o_1)=\{(1.5,1)\}$ and $p_i(o_2)=\{(0.25,1)\}$. We can then write $v_i(o_1)\ominus p_i(o_1)=\{(2,1),(1.5,-1)\}$ and $v_i(o_2)\ominus p_i(o_2)=\{(1,1),(0.25,-1)\}$. According to the lexicographic ordering, $o_1$ is preferred because $(2,1)>(1,1)$.
\end{example}

Another useful insight is that is that our greedy mechanisms are strongly related to ``VCG mechanisms'' in $\U$ space:
\begin{observation}
The following mechanism for value maximizers is equivalent (outcome and payments) to the non-transformed greedy mechanism:
\begin{enumerate}
\item Transform bids into $\U$ space as $\tau(b_i(o))$.
\item Find an outcome maximizing W(o)=$\tau(b_1(o))\oplus\dots\tau(b_n(o))$.
\item Compute externality payments in $\U$ space in the natural way to get $p_1,\dots,p_n$.
\item Transform payments back into real numbers as $\tau^{-1}(p_i)$; charge these payments to the bidders.
\end{enumerate}
\end{observation}
For an example we revisit Example~\ref{ex:greedy}:

%\begin{example}\label{ex:greedy}
%Suppose there are three outcomes $\{o_1,o_2,o_3\}$ and four bidders with values $v_1=\{3,3,1\}$, $v_2=\{0.5,1,1\}$, $v_3=\{2,1,0\}$, and $v_4=\{0.5,0.5,0.5\}$.
%
%The greedy maximizing auction for value maximizers chooses outcome $o_1$ as follows:
%\begin{enumerate}
%\item The value of the highest-value bidder is maximized by taking either outcome $o_1$ or $o_2$ ($v_1=3$).
%\item Among outcomes $o_1$ and $o_2$, the value of the second-highest-value bidder is maximized by taking $o_1$ ($v_3=2$).
%\end{enumerate}
%To compute prices, observe that the auction would still choose $o_1$ if bidder 1, 2, or 4 were removed from the auction, so these bidders pay $p_{\{1,2,4\}}=0$. For bidder 3, notice that the outcome would be $o_2$ if it were removed ($v_2=1$). Neither bidder 1 nor bidder 4 care whether the outcome is $o_1$ or $o_2$, but bidder 2 gets $v_2=1$ from $o_2$ instead of $v_2=0$ from $o_1$. The price bidder 3 pays is bidder 2's value for $o_2$, i.e. $p_3=v_2(o_2)=1$.
%\end{example}

\begin{example}
We have 3 bidders and 4 outcomes. After applying $\tau$ we get the following $\U$-space values:
\begin{center}
\begin{tabular}{rcccc}
Bidder&1&2&3&4\\
$v_i(o_1)$&$\{(3,1)\}$&$\{(0.5,1)\}$&$\{(2,1)\}$&$\{(0.5,1)\}$\\
$v_i(o_2)$&$\{(3,1)\}$&$\{(1,1)\}$&$\{(1,1)\}$&$\{(0.5,1)\}$\\
$v_i(o_3)$&$\{(1,1)\}$&$\{(1,1)\}$&$\{\}$&$\{(0.5,1)\}$
\end{tabular}
\end{center}
A ``welfare''-maximizing mechanism in $\U$ space computes the $\U$-welfare for each outcome as
\begin{align*}
W(o_1)&=\sum_iv_i(o_1)=\{(3,1),(2,1),(0.5,2)\}\\
W(o_2)&=\sum_iv_i(o_2)=\{(3,1),(1,2),(0.5,1)\}\\
W(o_3)&=\sum_iv_i(o_3)=\{(1,2),(0.5,1)\}
\end{align*}
and then chooses $o_1$ since $W(o_1)$ is lexicographically maximum. This coincides with the choice of the greedy mechanism in Example~\ref{ex:greedy}.

The $\U$-space mechanism then computes prices as externalities. Again, the only bidder whose presence changes the outcome of the auction is bidder 3 --- without bidder 3 the outcome would be $o_2$. We can compute bidder 3's externality price as
\[p_3=(\{(3,1)\}\oplus\{(1,1)\}\oplus\{(0.5,1\})\ominus(\{(3,1)\}\oplus\{(0.5,2)\})=\{(1,1),(0.5,-1)\}\]
Applying the inverse transformation yields a payment of $\tau^{-1}(p_3)=1$, just as in Example~\ref{ex:greedy}.
\end{example}
%\begin{example}
%Suppose there 3 bidders and 3 outcomes, summarized in the following table:
%\begin{center}
%\begin{tabular}{rccc}
%Bidder&1&2&3\\
%$v_i(o_1)$&$\{(5,1)\}$&$\{(3,1)\}$&$\{(1,1)\}$\\
%$v_i(o_2)$&$\{(1,1)\}$&$\{(4,1)\}$&$\{(1,1)\}$\\
%$v_i(o_3)$&$\{(5,1)\}$&$\{(1,1)\}$&$\{(2,1)\}$
%\end{tabular}
%\end{center}
%The greedy mechanism chooses $o_1$ because $v_1(o_1)=\{(5,1)\}$ and then $v_2(o_1)=\{(3,1)\}$. Notice that the $\U$ welfare for $o_1$ is $W(o_1)=\sum_iv_i(o_1)=\{(5,1),(3,1),(1,1)\}$, which is lexicographically greater than $W(o_2)=\{(4,1),(1,2)\}$ and $W(o_3)=\{(5,1),(2,1),(1,1)\}$. Thus, it matches the greedy choice.
%
%Computing the externality for bidder 1, the greedy/$\U$-welfare optimal outcome without bidder 1 would be $o_2$ because $v_2(o_2)=\{(4,1)\}$. We can thus write bidder 1's externality as
%\[ext_1=(\{(4,1)\}\oplus\{(1,1)\})\ominus(\{(3,1)\}\oplus\{(1,1)\})=\{(4,1),(3,-1)\}\]
%The $(4,1)$ term will generally dominate in arithmetic and ordering, this is analogous to our greedy mechanism that charges 4.
%
%Computing an externality or bidder 2, the greedy/$\U$-welfare optimal outcome without bidder 2 would be $o_3$ because $v_3(o_3)=\{(2,1)\}$. We can thus write bidder 2's externality as
%\[ext_1=(\{(5,1)\}\oplus\{(1,1)\})\ominus(\{(5,1)\}\oplus\{(2,1)\})=\{(2,1),(1,-1)\}\]
%By comparison, our greedy mechanism would charge 2 because, though bidder 1 had the highest value for $o_3$, its value for $o_3$ was the same as its value for $o_1$. This is equivalent to the dominant $(2,1)$ term.
%\end{example}

\subsection{Characterizing Truthful Mechanisms in $\U$ Space}\label{sec:roberts-roberts}


We just saw how ``VCG'' in $\U$ space looks like a greedy mechanism; to proceed formally, we need to characterize mechanisms in $\U$ space. For traditional quasilinear bidders, Roberts characterizes truthful mechanisms in unrestricted domains as affine maximizers, that is, there exist weights $w_i$ and offsets $\gamma(o)$ such that the mechanism always picks $o\in\argmax \sum_iw_iv_i(o)-\gamma(o)$. To generalize affine maximization to $\U$ we must define it terms of linear functions: 
\begin{definition}
We say that a mechanism is a {\em generalized affine maximizer} if there are linear functions $h_i$ with offsets $\gamma(o)$ such that the mechanism always picks $o\in\argmax \sum_ih_i(v_i(o))\ominus\gamma(o)$.
\end{definition}
Existing results are known to generalize to various topological vector spaces (e.g.~\cite{Carbajal13}), but we are unaware of any version that explicitly considers payments and values that are not in real numbers, so we present a generalization following first proof of Lavi et al.~\cite{lavi08}. The resulting theorem, proven in Appendix~\ref{sec:roberts-proof}, leverages an infinite-dimensional version of the separating hyperplane theorem~\cite{borderNotes}:
\begin{theorem}\label{thm:vm-rt}
When $3\leq |\O|<\infty$ and both values and payments may be arbitrary values in $\U$, the only mechanisms that are DSIC are generalized affine maximizers.
\end{theorem}

Theorem~\ref{thm:vm-rt} is initially somewhat opaque --- while it is useful to know that mechanisms must be generalized affine maximizers, it is initially unclear what exactly that means. It turns out that, when mapped back to value maximizers, they correspond to our greedy mechanisms.

First, we note that linear functions in $\U$ are substantially more diverse than linear functions in $\Re$:
\begin{observation}\label{obs:u-linear}
A function $h:\U\rightarrow\U$ is linear if and only if it can be written as $h(u)=\sum_{k} w_k\times z(a_{k})$ where $z(x):\Re\rightarrow\U$ maps each real number with an element of $\U$.\footnote{So see this, let $z(x)=h(\{(x,1)\})$.} $h$ is monotone if and only if each $z(a_{k})$ is monotone in $a_{k}$.
\end{observation}
This diversity explains the apparent contrast between Roberts's characterization of mechanisms as affine maximizers and our transformed greedy maximizers. Roberts's affine maximizers scaled bidders' values by weights, but other transformations were forbidden, whereas our greedy mechanism is truthful for arbitrary monotone transformations of value, since the space of linear transformations is more diverse.

We can now map generalized affine maximizers back to mechanisms for value maximizers:
\begin{observation}
A generalized affine maximizer for $\U$-space bidders (informally) corresponds to our transformed greedy mechanism.
\end{observation}
\begin{proof}[Proof sketch.]
Let $z_i(x)$ denote the function $z(x)$ associated with the monotone linear function $h_i$ following Observation~\ref{obs:u-linear}. 

First, suppose that $\tau^{-1}(z_i(x))$ is strictly increasing in $x$. This implies the dominant term of $h_i(v_i(o))$ is strictly increasing in $v_i$. Since the lexicographic ordering is dominated by the highest-order term, we can intuitively ``drop'' everything except the dominant term of $h_i(v_i(o))$. Writing $\theta_i(x)=\tau^{-1}(z_i(x))$ we then claim
\[h_i(v_i(o))\sim \{(\theta_i(a_1),1)\}\]
A mechanism that maximizes $h_i(v_i(o))$ is therefore like the greedy mechanism with $\theta_i(x)=\tau^{-1}(z_i(x))$.

When $\tau^{-1}(z_i(x))$ is not strictly increasing in $x$, it means that low-order terms of $x_i(x)$ break the tie ($z_i(x)$ is strictly increasing in $x$). Since the domain of $z_i$ is the reals, it is straightforward to show that we can construct $\theta_i$ functions that preserve the ordering between bidders.
\end{proof}




\subsection{Relating Mechanisms for Value Maximizers to $\U$-Bidders}
We have seen that there are strong connections between mechanisms for value maximizers and for $\U$ bidders. Here, we attempt to relate them formally by thinking of value maximizing preferences as a discretization of $\U$-space quasilinear utilities. We start with an observation:
\begin{observation}
Fix a bidder $i$. Let $v_i(o),p_i(o)\in\U$ denote $i$'s value for outcome $o$ and (invoking the taxation principle) the price $i$ would pay if the mechanism chose outcome $o$ given others' bids. If the values $\tau^{-1}(v_i(o))$ and $\tau^{-1}(p_i(o))$ are all distinct, then $i$'s preference over value-payment pairs is the same as if the values and payments were $\tau(\tau^{-1}(v_i(o)))$ and $\tau(\tau^{-1}(p_i(o)))$, i.e. they are the same as if we dropped all low-order terms from the values and payments.
\end{observation}
This hints at our result in this section: since value maximizing preferences are like $\U$-space quasilinear utilities with low-order terms ignored, it follows that any mechanism that is truthful for value maximizers can be used to construct a mechanism that is truthful in $\U$ space as long as the high-order terms of values and prices are distinct.

We now formalize this idea.
\begin{definition}
A mechanism for quasilinear bidders in $\U$ space is discretized-DSIC-AE if and only if, for any $v_{-i}$, the set
\[X=\{x\in\Re^m|\exists v_i\mbox{ such that }x=\tau^{-1}(v_i)\mbox{ and truth-telling is not a best-response for $i$\}}\]
has measure 0 according to the standard Lebesgue measure on $\Re^m$.
\end{definition}

\begin{lemma}
A DSIC-AE mechanism for value maximizers can be used to construct a Discretized-DSIC-AE for $\U$-space bidders as follows:
\begin{enumerate}
\item Solicit bids $b_i\in\U^m$. Transform them to bids $\beta_i\in\Re^m$ as $\beta_i=\tau^{-1}(b_i)$.
\item Run $M$ on the bids $\beta_i$ to get an outcome $o^*$ and prices $\pi_i\in\Re$.
\item Transform prices $\pi_i$ into $p_i\in\U$ as $p_i=\tau(\pi_i)$.
\end{enumerate}
\end{lemma}
%\begin{corollary}\label{cor:u-reduction}
%If the only discretized-DSIC-AE mechanisms for $\U$-space bidders are transformed greedy mechanisms (almost everywhere), then the only DSIC-AE mechanisms for value maximizers are also transformed greedy mechanisms (almost everywhere).
%\end{corollary}

\begin{proof}
We want to analyze when a bidder $i$ might prefer to lie. Fix reports $b_{-i}$, and suppose that $v_i$ is such that truth-telling is a best-response for $i$ assuming it was a value maximizer with true value $\tau^{-1}(v_i)$. By the taxation principle, we can write $\pi_i(o)\in\Re$ and $p_i(o)\in\U$ as the prices that bidder $i$ would pay if the outcome is $o$, and we talk about $i$ choosing from this menu. There are only a handful of scenarios in which $i$ might wish to choose an outcome other than $o^*$ (i.e. to lie):
\begin{itemize}
\item If $\beta_i(o^*)\geq p_i(o^*)$...
\begin{itemize}
\item An outcome $o^+\neq o^*$ where $v_i(o^+)>v_i(o^*)$ was not a profitable deviation in $M$ because $\beta_i(o^+)<\pi_i(o)$; however after the transformation it becomes profitable $v_i(o)\geq p_i(o)$. {\em This is impossible.}
\item The optimal outcome $o^*$ was a best-response in $M$ with $\beta_i(o^*)\geq \pi_i(o^*)$, but after the transformation $v_i(o)<p_i(o)$ and so it is no longer $i$'s preferred outcome. {\em This can only happen if $\tau^{-1}(v_i(o))=\pi_i(o)$.}
\item An outcome $o^+\neq o^*$ where $v_i(o^+)>v_i(o^*)$ had $\beta_i(o^+)\leq\beta_i(o^*)$ because of information loss in $\tau^{-1}$. {\em This can only happen when $\tau^{-1}(v_i(o^+))=\tau^{-1}(v_i(o^*))$.}
\end{itemize}
\item If $\beta_i(o^*)< p_i(o^*)$...
\begin{itemize}
\item An outcome $o^+\neq o^*$ had $\beta_i(o^+)<p_i(o^+)$ but after the transformation has $v_i(o^+)\geq p_i(o^+)$. {\em This is impossible.}
\item An outcome $o^+\neq o^*$ had $\pi_i(o^+)> \pi_i(o^*)$ but after the transformation has $p_i(o^+)< p_i(o^*)$. {\em This is impossible.}
\item An outcome $o^+\neq o^*$ had $\pi_i(o^+)=\pi_i(o^*)$ and $\beta_i(o^+)=\beta_i(o^*)$ but $v_i(o^+)>v_i(o^*)$. {\em This can only happen when $\tau^{-1}(v_i(o^+))=\tau^{-1}(v_i(o^*))$.}
\end{itemize}
\end{itemize}
The three scenarios above that are possible each happen for very specific dominant terms in $v_i$, and specifically with measure 0 over the space of $\tau^{-1}(v_i)$. Thus, their union has measure zero.

One scenario remains --- that $(\beta_{-i},\tau^{-1}(v_i))$ is a valuation for which truth-telling was not a best response for $i$ in $M$. By definition of DSIC-AE, this happens with measure 0 as well.
\end{proof}




%Unfortunately, this does not close the loop because we have not characterized discretized-DSIC-AE mechanisms as would be required to apply Corollary~\ref{cor:u-reduction}. Thus, it remains possible that discretized-DSIC-AE mechanisms exist which are somehow different from generalized affine maximizers in $\U$. However, our results are strong evidence that even if a gap exists, our greedy mechanisms are the canonical mechanisms for value maximizers and any others are unlikely to be far from the generalized affine maximizers of $\U$.





==> rt.tex <==


\section{Roberts's Theorem for Linearly Ordered Groups} \label{sec:a-rt}
Let $(\U,\ag,\plus)$ be a \emph{linearly ordered group} (and let $\minus$ denotes the corresponding subtraction), which means $(\U,\plus)$ forms an algebraic group with zero element $\zero$, $(\U,\ag)$ is a totally ordered set, and $a\minus b\ageq \zero$ iff $a\ageq b$ for every $a,b\in \U$. Moreover, define $\Up\triangleq\{u\in\U:u\ageq \zero\}$. We use this algebraic structure for \emph{utilities}. 

Consider the unrestricted domain auction design problem. Let $\O$ be the set of possible outcomes, and let $\lvert\O\rvert\geq 3$, and suppose there are $n$ bidders with value functions $v_i:\O\rightarrow \Up$ for $i\in[n]$. An auction receives the bid function $b_i:\O\rightarrow \Up$ from each bidder $i$, and it then picks an outcome $o(\mathbf{b})\in \mathcal{O}$, and charges each bidder $i$ with the payment $p_i(\mathbf{b})\in\U$. $o(.)$ is called the \emph{allocation} function and $\{p_i(.)\}_{i\in[n]}$ are called \emph{payment} functions. Bidder $i$'s utility $u_i\in\U$ from outcome $(o,p_i)$ is then computed by
\begin{equation}
u_i(o,p_i)=v_i(o)\minus p_i
\end{equation}

\begin{definition} \label{def:IC}
An auction $\left(o(.),\{p_i(.)\}_{i\in[n]}\right)$ is truthful iff  $\forall i\in[n]$, $\forall \mathbf{v}, v'_i:$
\begin{equation}
v_i(o(\mathbf{v}))\minus p_i(\mathbf{v})\ageq v_i(o(v'_i,\mathbf{v}_{-i}))\minus p_i(v'_i,\mathbf{v}_{-i})
\end{equation}
and allocation $o(.)$ is said to be truthfully implementable if there exists payments $\{p_i\}_{i\in[n]}$ such that $\left(o(.),\{p_i(.)\}_{i\in[n]}\right)$ would be a truthful auction.
\end{definition}
We define a property of allocation functions, known as W-MON in the literature~\cite{}, which can be shown (in a straightforward fashion) to hold for allocations that are truthfully implementable in our setting. 
\begin{definition}[Weak Monotonicity (W-MON)] 
\label{def:wmon}For all $i\in[n]$ and $\forall v_i,v'_i$ and $\mathbf{v}_{-i}$, if $o(v_i,\mathbf{v}_{-i})=x$ and $o(v'_i,\mathbf{v}_{-i})=y$, then
\[v'_i(y)\minus v_i(y)\ageq v'_i(x)\minus v_i(x)\]
\end{definition}
We also define a stronger property of allocation functions, known as S-MON in the literature~\cite{}, which is known to be a substitute to W-MON when one tries to characterize truthfully implantable allocations for quasi-linear setting~\cite{}.

\begin{definition}[Strong Monotonicity (S-MON)] 
\label{def:smon}For all $i\in[n]$ and $\forall v_i,v'_i$ and $\mathbf{v}_{-i}$, if $o(v_i,\mathbf{v}_{-i})=x$, $o(v'_i,\mathbf{v}_{-i})=y$, and $x\neq y$, then
\[v'_i(y)\minus v_i(y)\ag v'_i(x)\minus v_i(x)\]
\end{definition}
We also define \emph{player decisiveness}, which is a property of allocation functions that has been used in~\cite{} to have a simple proof of Roberts' theorem for quasi-linear bidders. In quasi-linear setting, it is known that this property holds when allocations are truthfully implementable~\cite{}. 

\begin{definition}[Player Decisiveness] Player $i$ is decisive for allocation function $o(.)$ if for every $x\in\O$ and $\mathbf{v}_{-i}$, there exists $v_i:\O\rightarrow \Up$ such that $o(v_i,\mathbf{v}_{-i})=x$.
\end{definition}
\subsection{ A Generalized Roberts' Theorem}
In a very straightforward fashion, we can prove the following theorem which generalizes Robert's theorem to linearly ordered sets. 
\begin{theorem}
Suppose allocation $o(.)$ satisfies S-MON and player-1 decisiveness. Then there exist monotone non-decreasing functions $h_j:\U\rightarrow\U$ for each bidder $j\in[n]$ and a function $C:\O\rightarrow \U$, such that
\begin{itemize}
\item $\forall j\in [n]$, $h^j$ is distributive with respect to the addition $\plus$, i.e. $h_j(u_1\plus u_2)=h_j(u_1)\plus h_j(u_2)$.
\item $\forall j\in [n]$, $h^j(\zero)=\zero$. 
\item $ o(\mathbf{v})\in \underset{o'\in\O}{\operatorname{argmax}} ~~\left(\bigoplus_{j\in [n]} h_j(v_j(o'))\right) \plus C(o')$
\end{itemize}
\end{theorem}
\begin{proof}[Proof sketch.] Fix bidder 1 and define (as in~\cite{}):
\[\forall x,y\in\O:~~\d{x}{y}\triangleq\underset{v'_1(.):~o(v'_1,\mathbf{v}_{-1})=x}{\inf}\left\{v'_1(x)\minus v'_1(y)\right\}\]
Note that due to player 1 being decisive $\d{x}{y}$ is well-defined, because for every $\mathbf{v}_{-1}$ there exists $v''_1$ such that $o(v''_1,\mathbf{v}_{-1})=y$. Now let $v'_i$ be such that $o(v'_1,\mathbf{v}_{-1})=x$. Then, due to S-MON,  $v''_1(y)\minus v'_1(y) \ageq v''_1(x)\minus v'_1(x)$, or equivalently $v'_1(x)\minus v'_1(y) \ageq v''_1(x)\minus v''_1(y)$. Therefore, $\d{x}{y}$ is infimum of a bounded sequence in a totally ordered set and therefore exists. Now, by following the same steps as in~\cite{} (proof of Theorem~3, Claims 7-12), one can prove the following properties of $\d{x}{y}$ even in our setting:
\begin{itemize}
\item $\forall x,y\in\O$, $\d{x}{y}$ is a monotone non-increasing function of $\mathbf{v}_{-1}(x)-\mathbf{v}_{-1}(y)=\mathbf{r}\in\U^{n-1}$. Let $\di{x}{y}{\mathbf{r}}\equiv\d{x}{y}$.
\item For every $\mathbf{r},\mathbf{t}\in\U^{n-1}$, and distinct $x,y,z\in\O:$ $\di{x}{y}{\mathbf{r}}\plus\di{x}{y}{\mathbf{\zero}\minus \mathbf{t}}=\zero $, and $\di{x}{y}{\mathbf{r}}\plus\di{y}{z}{\mathbf{t}}\plus\di{z}{x}{\mathbf{\zero}\minus \mathbf{r}\minus \mathbf{t}}=\zero$.
\end{itemize}
First, we show that for distinct $x,y,z\in\O$, $\di{x}{y}{\mathbf{r}\plus \mathbf{s}}\minus\di{x}{y}{\mathbf{r}}=\di{z}{y}{\mathbf{t}\plus \mathbf{s}}\minus\di{z}{y}{\mathbf{t}}$. This simply holds because

\[\di{x}{y}{\mathbf{r}\plus \mathbf{s}}\minus\di{x}{y}{\mathbf{r}}=\di{z}{y}{\mathbf{t}\plus \mathbf{s}}\plus \left(\di{x}{z}{\mathbf{r}\minus \mathbf{t}}\plus\di{y}{x}{\mathbf{\zero}\minus\mathbf{r}}\right)=\di{z}{y}{\mathbf{t}\plus \mathbf{s}}\minus\di{z}{y}{\mathbf{t}}\]

Now, suppose for every $u\in \U$, $\mathbf{e}^{u}_j\in\U^{n-1}$ be a vector with $j$'s coordinate equal to $u$ and all other coordinates equal to $\zero$. Define $h^j_{xy}:\U\rightarrow\U$ as following.
\[\forall j\neq 1,\forall u\in\U: h^j_{xy}(u)=\di{x}{y}{\mathbf{\zero}}\minus\di{x}{y}{\mathbf{e}^u_j}\]
Note that by the properties of $\di{x}{y}{.}$, we have the following:
\begin{align}
\label{eq:dist}
h^j_{xy}(u_1\plus u_2)&=\di{x}{y}{\mathbf{\zero}}\minus\di{x}{y}{ \mathbf{e}_i^{u_1\plus u_2}}=\di{x}{y}{\mathbf{\zero}}\minus\di{x}{y}{ \mathbf{e}_j^{u_1}\plus \mathbf{e}_j^{u_2}}\nonumber\\
&=\di{x}{y}{\mathbf{\zero}}\plus\di{y}{z}{\mathbf{\zero}\minus\mathbf{e}_j^{u_2}}\plus \di{z}{x}{\mathbf{\zero}\minus\mathbf{e}_j^{u_1}}\nonumber\\
&=\left(\di{x}{z}{\mathbf{\zero}}\minus\di{x}{z}{\mathbf{e}_j^{u_1}}\right)\plus \left(\di{z}{y}{\mathbf{\zero}}\minus\di{z}{y}{\mathbf{e}_j^{u_2}}\right)=h^j_{xz}(u_1)\plus h^j_{zy}(u_2)
\end{align}
Now, pick an arbitrary $\mathbf{r}\in \U^{n-1}$.  Lets define $\mathbf{r}^j\triangleq(\zero,\ldots,\zero,r_j,r_{j+1},\ldots,r_{n-1})$ and $\mathbf{r}^{n}\triangleq \mathbf{\zero}$ . Then for distinct $x,y,z\in\O$, we have 
\begin{align}
\di{x}{y}{\rb}\minus\di{x}{y}{\mathbf{\zero}}&=\bigoplus_{j=1}^{n-1}\di{x}{y}{\mathbf{r}^j}\minus\di{x}{y}{\mathbf{r}^{j+1}}=\bigoplus_{j=1}^{n-1}\di{x}{y}{\mathbf{r}^{j+1}\plus\mathbf{e}_j^{r_j}}\minus\di{x}{y}{\mathbf{r}^{j+1}}\nonumber\\
&\label{eq:h-fun}
=\bigoplus_{j=1}^{n-1}\di{z}{y}{\mathbf{e}_j^{r_j}}\minus \di{z}{y}{\mathbf{\zero}}=\zero\minus \bigoplus_{j=1}^{n-1} h^j_{zy}(r_j)
\end{align}
Note that $h^j_{zy}(\zero)=\zero$, and therefore from~(\ref{eq:h-fun}), we have $h^j_{zy}(r)=\di{x}{y}{\mathbf{e}_j^r}\minus \di{x}{y}{\mathbf{\zero}} $. So, $h^j_{zy}=h^j_{wy}$. Also, from definition of $h^j$, $h^{j}_{yz}(r)=\zero\minus h^{j}_{zy}(r)=\zero\minus h^j_{wy}(r)=h^j_{yw}(r)$. Combining those, $h^j_{xy}=h^j_{zw}$, which shows $h^j_{xy}$ does not depend on the choice of $x$ and $y$ (from now on, we call this function $h^j$). Following (\ref{eq:dist}), $h^j$ is also distributive with respect to $\plus$ for every $j\neq 1$. Moreover, following the fact that $\di{x}{y}{\rb}$ is a monotone non-increasing function of $\rb$, $h^j$ is monotone non-decreasing for every $j\neq 1$. Let $h^1(r)\triangleq r$.

Now, fix an arbitrary outcome $w\in\O$ and let $C(x)=\di{w}{x}{\mathbf{\zero}}$ for every outcome $x\neq w$, and let $C_w=\zero$. Now, for a value profile $\mathbf{v}$ suppose $o(\mathbf{v})=x$. By using (\ref{eq:h-fun}), for every $y\neq x$, $v_1(x)\minus v_1(y)\ageq\d{x}{y}=\di{x}{y}{\mathbf{\zero}}\minus \bigoplus_{j=1}^{n-1} h^j(v_j(x)\minus v_j(y))$. Since $\di{x}{y}{\mathbf{\zero}}=\di{x}{w}{\mathbf{\zero}}\plus \di{w}{y}{\mathbf{\zero}}$, $\di{x}{w}{\mathbf{\zero}}=\zero\minus \di{w}{x}{\mathbf{\zero}}$, and $h^j$ distributes with respect to the addition, by rearranging the terms we get
\[C(x)\plus \bigoplus_{j=1}^{n} h^j(v_j(x))\geq C(y)\plus \bigoplus_{j=1}^{n} h^j(v_j(y)) \]
which completes the proof.
\end{proof}

\subsection{Continuous Addition}
\begin{definition}
\label{def:add}
Fix a function $\mathcal{H}:\mathcal{R}^2\rightarrow \mathcal{R}$ that has the following properties:
\begin{itemize}
\item (\textbf{Monotonicity}) $\h(a,b)$ is monotone increasing with respect to $a$ and $b$.
\item (\textbf{Continuity}) $\h(a,b)$ is continuous with respect to $a$ and $b$.
\item (\textbf{Associative}) $\forall a,b,c\in \mathcal{R}:~ \h(\h(a,b),c)=\h(a,\h(b,c))$.
\item (\textbf{Commutative}) $\forall a,b\in \mathcal{R}:~\h(a,b)=\h(b,a)$. 
\item (\textbf{Identity Element}) $\exists~\mathbf{1}\in\mathcal{R}$ such that $\forall a\in\mathcal{R}:~\h(a,\mathbf{1})=a$.
\item (\textbf{Inverse Operator}) $\forall a\in \mathbb{R}:~\h(a,-a)=\mathbf{1}$.
\
\end{itemize}
Then $a\plus b \triangleq \h(a,b)$ and $a\minus b \triangleq \h(a,-b)$.
\end{definition}
\label{def:hpower}
Also define $x\hgeq y \iff x\minus y\geq \mathbf{1}$, and $\h(a)\triangleq\h(a,\mathbf{1})$. We further assume $\mathcal{R}$ has the property that if $x\in\mathcal{R}$ and $y\hgeq x$ then $y\in\mathcal{R}$. Let $\mathcal{R}_+\triangleq \{x\in\mathcal{R}:x\hgeq \mathbf{1}\}$.

\begin{definition} Using function $\h$ as in Definition~\ref{def:add}, we have the followings:
\begin{itemize}
\item  $\forall p\in \mathbb{N}, a\in\mathcal{R}: ~~\h^{p}(a)\triangleq a\plus a\plus \ldots (\text{p times})\ldots \plus a$. Moreover, $\h^{0}\triangleq \mathbf{1}$.
\item $\forall q\in \mathbb{N}, a\in \mathcal{R}: ~~\h^{q^{-1}}(a)\triangleq (\h^q)^{-1}(a)$.
\item $\forall x=\frac{p}{q},$ where $p\in\mathbb{Z}_{+},q\in\mathbb{N}$, let $\h^x(a)\triangleq \h^p \circ \h^{q^{-1}} (a)$.
\item $\forall x\in \mathcal{R}:~\h^x\triangleq \underset{\frac{p_n}{q_n}\rightarrow x}{\lim} \h^{\frac{p_n}{q_n}}$, where $p_n\in\mathbb{Z}_+, q_n\in\mathbb{N}$ and $\{\frac{p_n}{q_n}\}$ lies in $\mathcal{R}$.
\end{itemize}
\end{definition}
\begin{remark} $\h^x$ can be defined for $x\in\mathcal{R}$ as in Definition\ref{def:hpower}, because $\mathcal{R}$ is compact and $\h$ is continuous and monotone (and hence is invertible).
\end{remark}
\begin{remark}
We further assume there always exist an special element $e\in\mathcal{R}_+$ such that $\forall \delta\in\mathcal{R}_+:\h^\delta(e)=\delta$.
\end{remark}

In this document we try to generalize Roberts Theorem, i.e. the characterization of truthful mechanisms,  for this class of utility functions. Our result is based on the following notion of truthfulness.

\subsection{Generalized Roberts Theorem for Continuous}
\begin{theorem}
An allocation  $o(.)$ is truthfully implementable by some payment rule $\{p_i(.)\}_{i\in\mathcal{N}}$ iff there exists $w_i\in\mathcal{R}_+$ for all $ i\in\mathcal{N}$ and $C(.):\mathcal{O}\rightarrow \mathcal{R}$, s.t.
\begin{equation}
o(\mathbf{v})\in \underset{o'\in\mathcal{O}}{\operatorname{argmax}} ~~\left(\bigoplus_{i\in \mathcal{N}} \h^{w_i}(v_i(o'))\right) \plus C(o')
\end{equation}
\end{theorem}
\begin{example} Suppose $u_i=\frac{v_i}{p_i}$. It is easy to check this satisfies all the conditions of Definition~\ref{def:add} for $\h(a,b)=ab$. Further, $\h^x(a)=a^x$. Hence, the set of all truthful mechanisms will be all the maximizers of some function $C(o)\prod_{i\in\mathcal{N}}{v_i(o)^{w_i}}$.
\end{example}
\subsection{Two Technical Lemmas}
Before going through the proof, we start by two technical lemmas which are the key in proving the new modification of Roberts theorem. 
\begin{lemma} Suppose $g:\mathcal{R}_{+}\rightarrow \mathcal{R}$ is monotone non-decreasing (with respect to operator $\plus$) and there exist $h:\mathbb{R}_{+}\rightarrow \mathcal{R}_+$ s.t. $\forall r\in \mathcal{R}_+$ and $ \delta\in \mathbb{R}_+$ we have $g(r\plus\delta)\minus g(r)=h(\delta)$. Then there exists $w\in \mathcal{R}_+$ such that $h(\delta)=\h^w(\delta)$.
\end{lemma}
\begin{proof}
Consider any element $e\hg \1$. Due to strict monotonicity and continuity,  the following is true:
\[\forall x\in\mathcal{R}_+,\exists y\in \mathcal{R}_+:\h^y(e)=x\]
For every $x\in\mathcal{R}_+$, let define $\hlog(x)\triangleq y$ if $y\in\mathcal{R}$ is the unique element such that $\h^y=x$.  
For any integer $q\in\mathcal{R}_+$ we have: 
\begin{align*}
h(e)&=g(\1\plus e)\minus g(\1)=\h\left( g(\h(\1,e)),-g(\h(\1,\1))  \right)\nonumber\\
&=\bigoplus_{i=0}^{q-1}\h\left( g\left(\h(\1,\h^{\frac{(i+1)}{q}}(e))\right),-g\left(\h(\1,\h^{\frac{i}{q}}(e))\right)  \right)\nonumber\\
&=\bigoplus_{i=0}^{q-1}\ g\left(\h(\1,\h^{\frac{(i+1)}{q}}(e))\right)\minus g\left(\h(\1,\h^{\frac{i}{q}}(e))\right) \nonumber\\
&=\bigoplus_{i=0}^{q-1}h(\h^{\frac{1}{q}}(e))=\h^q\left(h(\h^{\frac{1}{q}}(e)\right)
\end{align*}
which basically means $h(\h^{\frac{1}{q}}(e))=\h^{\frac{1}{q}}(h(e))$. Similarly, we will also have $h(\h^{\frac{p}{q}}(e))=\h^p\left(h(\h^{\frac{1}{q}}(e)\right)$. Combining both, we get $h(\frac{p}{q})=h(\h^{\frac{p}{q}}(e))=\h^{\frac{p}{q}}(h(e))$. By a simple continuity argument, due to the fact that $\mathcal{R}_+$ is compact, we have:
\[\forall y\in\mathcal{R}: h(\h^y(e))=\h^y(h(e))\]
Now, let $x=\h^y(e)$ (and so $y=\hlog(x)$) and $w=\hlog(h(e))$. We then have:
\[h(x)=\h^{\hlog(x)}(\h^w(e))=\h^w(\h^{\hlog(x)}(e))=\h^w(x)\]
which proves the lemma.
\end{proof}



==> sp-revenue-a.tex <==


\section{The Optimal Revenue Single-Agent Mechanism}
\label{appendix:OPT-SA-DP}
Here we give a polynomial-time algorithm to compute the optimal mechanism for selling $k$ items to a simple value maximizing agent. Note that for a deterministic mechanism, Theorem~\ref{THM:SPDSIC} implies that we need only choose the thresholds $t_j$ at which the allocation level increases from $j-1$ to $j$ for all $j$ from $1$ to $k$. For simplicity of exposition, we assume the value distribution $F$ is finitely supported on a set $v_1,\ldots,v_n$, with probability mass function given by $f(\cdot)$. Label this set such that $v_1 < v_2 < \ldots < v_n$. Extending our algorithm to continuous distributions is straightforward for most standard models for distributional access.

Corollary~\ref{COR:CRITICALPAY} implies that the expected revenue of a mechanism with thresholds $t_1\leq t_2\leq\ldots\leq t_k$ is given by:
\begin{equation}
\label{eq:optobjective}
\sum_{\ell=1}^k \ell\cdot t_\ell(F(t_{\ell+1})-F(t_\ell)),
\end{equation}
where $F(v_i)$ is given by $\sum_{j=1}^{i-1} f(v_i)=\text{Pr}[v<v_i]$, and where $F(v_{n+1})$ is defined to be $1$.

Define $\text{OPT}(i, j)$ to be the maximum attainable revenue from only selling to values at least $v_j$, and only selling $i$ or more items in the event of a sale. Then the value of (\ref{eq:optobjective}) with the optimal thresholds is equal to $\text{OPT}(1,1)$. Moreover, we have the following recurrence relation:
\begin{equation}
\label{eq:recurrence}
\text{OPT}(i,j)=\max_{\ell\geq j}\left[iv_j(F(v_\ell)-F(v_j))+OPT(i+1,\ell)\right]
\end{equation}

This yields a straightforward two-dimensional dynamic program. For $i=k$, we have $\text{OPT}(i,j)=kv_j(1-F(v_j))$ for all $j\leq n$. For $j=n+1$, we have $OPT(i,j)=0$ for all $i$. The remaining values of $OPT(i,j)$ can be computed by filling a memoization table starting with high values of $i$ and $j$ and moving to low values.

==> sp-revenue-long.tex <==


\section{Maximizing Revenue from a Single Agent}\label{sec:sp-revenue}

In this section, we consider the problem of maximizing expected revenue in
selling to a single simple value maximizer agent with single-dimensional type,
where the type is a {\em value} drawn from a distribution $F$. In particular,
we consider deterministic, DSIC mechanisms for selling $k$ identical
items.\footnote{The same problem for randomized mechanisms is ill-posed without
a model for how value maximizers evaluate lotteries over allocation.} Such a
mechanism maps the agent's value $v$ to a deterministic allocation $x\in
\{0,1,\ldots,k\}$. The agent gets value for allocation $v\cdot x(v)$ (i.e.,
its value is additive across identical items), and is charged a deterministic
payment $p(v)$.

We make two main observations. First, we note that the revenue-optimal mechanism for a value maximizer generally offers the agent the option to buy any number of items from $0$ to $k$, and a positive measure of values will take each of the $k+1$ different offers. In other words, the optimal mechanism involves \emph{second-degree price discrimination}. This stands in contrast to the optimal mechanism for a quasilinear agent, in which the menu consists of $0$ items and $k$ items, with nothing in between. Second, we observe that the optimal single-agent mechanism can be computed in polynomial time via dynamic programming.

\subsection{Example: Two Items, Uniform Agent}
\label{sec:discexample}

Consider selling a supply of two items to an agent with value $v$ drawn uniformly from $[0,1]$. If the agent was quasilinear, the results of \cite{myerson81} imply that the optimal mechanism would be to sell the bundle of both items at price $1$ if $v\geq 1/2$, and to sell nothing otherwise. We will show that if the agent is a simple value maximizer, the optimal mechanism will sell a single item to a positive measure of values, in addition to selling both items and no items at all with positive probability.

To derive the optimal mechanism, we use the characterization in Section~\ref{SEC:SINGLEPARAM}. Namely, we optimize over all deterministic, monotone allocation rules, which are given by two values: the value $t_1$ where the allocation steps up from $0$ to $1$, and the value $t_2$ where the allocation steps up from $1$ to $2$. Individual rationality implies that the truthful payments for an agent with value $v<t_1$ is 0. Corollary~\ref{COR:CRITICALPAY} implies that the truthful payment for an agent with value $v\in [t_1,t_2)$ is $t_1$, and for an agent with value $v\geq t_2$ is $2\cdot t_2$. The revenue of our mechanism is therefore $t_1(t_2-t_1)+2 t_2(1-t_2)$, where the first term is revenue from the event that the agent receives a single item, and the second term from the event where the agent receives two items. All that remains is to optimize this function over $0\leq t_1\leq t_2\leq 1$, which yields an optimal solution of $t_1= 2/7$, and $t_2 = 4/7$. Hence, the optimal mechanism allocates exactly one item with probability $2/7$. This is second-degree price discrimination.

%It is illuminating to compare this mechanism to the optimal mechanism if the agent had quasilinear preferences instead. Myerson's characterization implies that for any distribution over the agent's value, the optimal mechanism would be given by a single threshold $t$, below which the agent would receive no allocation and be charged nothing, and above which the agent would receive both items and be charged $2t$. In other words, the optimal mechanism for quasilinear preferences does not discriminate by varying the quantity of service, while the optimal mechanism for value maximizers does.

\subsection{Optimal Single-Agent Mechanisms}

We now give a polynomial-time algorithm to compute the optimal mechanism for selling $k$ items to a simple value maximizing agent. Note that for a deterministic mechanism, Theorem~\ref{THM:SPDSIC} implies that we need only choose the thresholds $t_j$ at which the allocation level increases from $j-1$ to $j$ for all $j$ from $1$ to $k$. For simplicity of exposition, we assume the value distribution $F$ is finitely supported on a set $v_1,\ldots,v_n$, with probability mass function given by $f(\cdot)$. Label this set such that $v_1 < v_2 < \ldots < v_n$. Extending our algorithm to continuous distributions is straightforward for most standard models for distributional access.

Corollary~\ref{COR:CRITICALPAY} implies that the expected revenue of a mechanism with thresholds $t_1\leq t_2\leq\ldots\leq t_k$ is given by:
\begin{equation}
\label{eq:optobjective}
\sum_{\ell=1}^k \ell\cdot t_\ell(F(t_{\ell+1})-F(t_\ell)),
\end{equation}
where $F(v_i)$ is given by $\sum_{j=1}^{i-1} f(v_i)=\text{Pr}[v<v_i]$, and where $F(v_{n+1})$ is defined to be $1$.

Define $\text{OPT}(i, j)$ to be the maximum attainable revenue from only selling to values at least $v_j$, and only selling $i$ or more items in the event of a sale. Then the value of (\ref{eq:optobjective}) with the optimal thresholds is equal to $\text{OPT}(1,1)$. Moreover, we have the following recurrence relation:
\begin{equation}
\label{eq:recurrence}
\text{OPT}(i,j)=\max_{\ell\geq j}\left[iv_j(F(v_\ell)-F(v_j))+OPT(i+1,\ell)\right]
\end{equation}

This yields a straightforward two-dimensional dynamic program. For $i=k$, we have $\text{OPT}(i,j)=kv_j(1-F(v_j))$ for all $j\leq n$. For $j=n+1$, we have $OPT(i,j)=0$ for all $i$. The remaining values of $OPT(i,j)$ can be computed by filling a memoization table starting with high values of $i$ and $j$ and moving to low values.

\subsection{The Ubiquity of Price Discrimination}
Finally, we show that in a sense, the second-degree price discrimination observed in Section~\ref{sec:discexample} is unavoidable. In particular, it will occur for \emph{every} continuous, fully-supported value distribution. Formally:

\begin{theorem}
For every continuous, fully-supported value distribution $F$, and for every number of items $i$ between $0$ and $k$, there is a positive measure of values who will purchase exactly $i$ items under the revenue-optimal mechanism to sell to a simple value maximizer with value distribution $F$.
\end{theorem}

\begin{proof}
Theorem~\ref{THM:SPDSIC} implies that every deterministic truthful mechanism is characterized completely by its choice of thresholds $t_j$ at which the allocation level increases from $j-1$ to $j$ for all $j$ from $1$ to $k$. Moreover, we have that the revenue of such a mechanism is given by 
\begin{equation}
\label{eq:optobjectiveagain}
\sum_{\ell=1}^k \ell\cdot t_\ell(F(t_{\ell+1})-F(t_\ell)).
\end{equation}

We consider a mechanism which does not sell $i$ items with positive probability, and show how to improve the mechanism's revenue --- hence, such a mechanism cannot be optimal. A similar argument implies that no mechanism which sells with probability $1$ is optimal.

A mechanism which for some $i\in\{1,\ldots,k\}$ does not sell exactly $i$ items with positive probability must have $t_i=t_{i+1}$. Choose the lowest $i$ for which this is the case. Then $t_i-t_{i-1}>0$. We will show that such a mechanism's revenue can be improved by slightly decreasing $t_i$ to $t_i'=t_i-\epsilon$ for some sufficiently small $\epsilon>0$. This decreases the measure of values purchasing exactly $i-1$ items by $F(t_i)-F(t_i-\epsilon)$, which decreases the revenue contribution from this event by $(i-1)t_{i-1}(F(t_i)-F(t_i-\epsilon))$. Meanwhile, decreasing $t_i$ causes a $F_i(t_i)-F(t_i-\epsilon)$ measure of values to purchase exactly $i$ items instead, yielding a revenue increase of $i(t_i-\epsilon)(F_i(t_i)-F(t_i-\epsilon))$. The gain from decreasing $t_i$ outweighs the loss as long as $(i-1)t_{i-1}<i(t_i-\epsilon)$, which holds as long as $\epsilon$ is sufficiently close to zero.
\end{proof}


==> ssa.tex <==


\section{GSP and Slot Auctions}  \label{sec:value-max}

The model we choose to represent bidder preferences fundamentally affects the prescriptions that theory makes. Modeling bidders as value maximizers turns some standard theory on its head and gives new ideas for solving some current industry auction problems. In this section we explore three applications to sponsored search:
\begin{itemize}
\item We show that, contrary to standard theory, the generalized second price (GSP) auction is truthful. This is an application of~\cite{aggarwal09}.
\item We use truthful auctions for value maximizers to generalize GSP to domains where it currently cannot be used.
%\item We use preferences that are a hybrid between quasilinear and value maximizing preferences that allow a search engine to tune its pricing based on the expectations of advertisers.
\end{itemize}

\subsection{GSP is Truthful}

The generalized second price auction (GSP) is a textbook example of the importance of modeling bidders' preferences carefully.

GSP was developed by an engineering group at Google~\cite{varian14}, thinking at the time that it was the appropriate way to generalize the standard second price auction to a multi-slot setting. It was quickly decided, however, that the Vickrey-Clarke-Groves mechanism (VCG) was actually the right way to generalize a second price auction, and much effort has been spent to rationalize and justify the continued use of GSP. However, this reaction assumes bidders have quasilinear preferences; in fact, to the degree that value maximizers are a better model of real advertisers, we show that GSP is the natural generalization of a second price auction.

The generalized second price auction is as follows:

\begin{definition}
The {\em generalized second price} auction (GSP) proceeds as follows:
\begin{enumerate}
\item Bidders are sorted by $\beta_ib_i$; the bidder ranked $j$ gets slot $j$.
\item A bidder is charged a price-per-click equal to the minimum bid required to keep the same slot.
\end{enumerate}
\end{definition}

Aggarwal et al.~\cite{aggarwal09} study a different generalization of quasilinear preferences and remark that GSP is truthful for bidders who buy as much as they can subject to a maximum price. In our setting, this is equivalent to a simple value maximizer. Alternatively, this can also be seen as a simple special case of our Theorem~\ref{thm:vm-sp-char}.

Since value maximizers with ROI constraints are equivalent to simple value maximizers with a reduced value (see Remark~\ref{def:rvmp}), we also find that GSP is truthful for value maximizers with ROI constraints.

\begin{theorem}[Aggarwal et Al.~\cite{aggarwal09}, interpreted]
GSP is truthful\footnote{Effectively DSIC-AE (see Definition~\ref{def:dsic-ae}).} for simple value maximizers and value maximizers with ROI constraints.
\end{theorem}

\subsection{Generalizing GSP Beyond Slot Auctions}

As noted earlier, the algorithms for optimizing ad placement in sponsored search and other online ad platforms are getting progressively more complex. As a result, GSP does not immediately apply, and a different solution is required.

The industry reaction has often been to use a VCG auction in these more complicated settings (e.g. Facebook or Google's Contextual Ads~\cite{varian14}); however, in established marketplaces like sponsored search, quickly transitioning from a GSP-based system to a VCG-based system is tricky and potentially perilous. Advertisers are accustomed to GSP prices, so any switch will force advertisers to revise their expectations. Moreover, GSP prices are higher than their VCG counterparts, so to the degree that advertisers do not react, there may be a significant revenue loss for the advertising platform. As a result, a line of research has focused on both ways to generalize GSP (e.g.~\cite{cavallo14,bachrach14}) and to transition smoothly from GSP to VCG (e.g.~\cite{bachrach15}).

Our work suggests a new way to approach this problem: define GSP as the welfare maximizing auction for value maximizers and run an analogous truthful auction for the new setting:
\begin{proposition}%[Generalized GSP]
The generalized second price auction (GSP) is the welfare-maximizing auction for simple value maximizers.
\end{proposition}

%One problem with this definition is that it changes the objective from maximizing (quasilinear) welfare to maximizing the $L^\infty$-norm of bidders' values, which may be undesirable for the search engine. While this is required for truthfulness in general settings, it is not required when (as is standard in practice) the auction is a single parameter domain. Thus, we propose the following alternative definition for practically implementing a generalized GSP auction:
%
%\begin{definition}[Generalized GSP, V2]
%The generalized second price auction (GSP) is the auction that maximizes welfare in the standard quasilinear sense, then charges prices that are truthful for a simple value maximizer.
%\end{definition}
%
%Both of these definitions coincide with traditional GSP in the special case of the standard model of a sponsored search auction.


%%%%%%%%%%%%

%\subsection{Hybrid Generalized GSP}
%
%While we contend that value maximization is a better model of bidder preferences than quasilinear, it also has its own problems. For example, a value maximizer will prefer 1000 clicks at \$1 each to 999 clicks for free. We hypothesize that bidders' true preferences lie somewhere between quasilinear and value-maximizing, and propose that a practical way to generalize GSP is based on a model of hybrid preferences:
%
%\begin{definition}[Hybrid Generalized GSP]
%The hybrid generalized second price auction (GSP) is the auction that maximizes welfare in the standard quasilinear sense, then charges prices that are truthful for a bidder with (a) $\alpha$-hybrid preferences, or (b) profit-maximizing preferences with a ROI constraint of $\gamma$.
%
%The parameter $\alpha$ or $\gamma$ can be tuned to match (a) bidders' measured preferences or (b) current marketplace operating characteristics (e.g. to match current price/quantity trade-offs).
%\end{definition}
%
%Note that for $\alpha=1$ or $\gamma=1$, this corresponds to truthful pricing for a quasilinear bidder, while as $\alpha\rightarrow\infty$ or as $\gamma\rightarrow\infty$, it corresponds to truthful pricing for a value maximizer. (See Section~\ref{sec:real}.)
%
%
%
%




==> value-max-a.tex <==
%\section{More Details of The Transformed Greedy Mechanism for General Domains}
\label{sec:value-max-a}
%Here, we introduce a family of mechanisms that generalizes the greedy mechanism, defined in Algorithm~\ref{alg:greedy-tmech}. This formulation allow negative values, discretized bid spaces, arbitrary monotone transformations of bidders' values, and outcome-specific ``offsets.'' Informally, the {\em transformed greedy auction for value maximizers} transforms agent $i$'s value according to a monotone function $\theta_i:\Re\rightarrow\Re$ and greedily chooses an outcome according to $\theta$. Again, any mechanism in this family is truthful for any transformation of value:
%\begin{algorithm}[h]
%	\SetAlgoNoLine
%	\SetKwFunction{tfgreedy}{TransformedGreedy}\SetKwFunction{ftgreedymech}{TransformedGreedyMech}
%	\SetKwProg{opt}{Algorithm}{}{}
%	\SetKwProg{mech}{Mechanism}{}{}
%	\opt{\tfgreedy{$\{b_i\}$}}{
%	\KwIn{Bids , one vector $b_i\in\Re^m$ per bidder.}
%	\KwOut{An outcome $o^*$.}
%	
%	\For{$o\in\mathcal O$}{
%		$z(o)\leftarrow \mbox{\texttt{Sort} }\{\theta_1(v_1(o)),\dots,\theta_n(v_n(o)),\theta_0(o)\}\mbox{ by }|\theta_i(v_i(o))|\mbox{ in descending order.}$\;
%	}
%	$o^*\leftarrow $outcome $o$ with greatest $z(o)$ according to a lexicographic order\tcp*{Break ties by order on $\O$}
%	\Return{$o^*$}\;
%	}
%	
%	\mech{\ftgreedymech{$\{b_I\}$}}{
%		\KwIn{Bids $\{b_i\}$, one vector $b_i\in\Re^m$ per bidder.}
%	\KwOut{An outcome $o^*$ and payments $\{p_i\}$.}
%	
%	$o^*\leftarrow\greedy{b}$\;
%	\For{$i=1$ to $n$}{
%		$p_i\leftarrow\inf \left\{b_i'(o^+)\left|o^+=\mbox{\tfgreedy{$b_{-i},b_i'$} and }b_j(o^+)=b_j(o^*)\right.\right\}$\;
%	}
%	\Return{$o^*$, $\{p_i\}$}\;
%	
%	}
%	
%	\caption{The Transformed Greedy Family of Mechanisms.}
%\label{alg:greedy-tmech}
%\end{algorithm}
%
%
%\begin{theorem}\label{thm:twm}
%The transformed greedy auction is truthful for any nondecreasing transformations $\theta_i$ and offsets $\theta_0(o)$ as long as ties under truthful bidding happen with measure zero or the bid space is discretized with a minimum increment..
%\end{theorem}

\begin{proof}[of Theorem~\ref{thm:twm}] We prove the theorem when values are nonnegative. The reasoning for negative values is analogous.

Say that a value vector $v$ results in a tie if there are distinct $i,j\in\{0,1,\dots,n\}$ and outcomes $o_i$ and $o_j$ such that $\theta_i(o_i)=\theta_j(o_j)>0$. For now, assume that ties do not happen.

Note the following:
\begin{itemize}
\item[(a)] The mechanism is IR by construction, so a bidder will never wish to lie to achieve a smaller value.
\item[(b)] By definition the mechanism charges the same price to all types that get the same value, so there is no incentive to misreport to get the same outcome at a lower price.
\item[(c)] Let $o^*$ be the outcome chosen by the mechanism and $z^*=z(o)$. Let $\mathcal O_r$ denote the set of outcomes that have the same value as $z^*$ in positions $1,\dots r-1$, and suppose that bidder $i$ ranks $r$-th in the vector $z^*$. Then for all $k<r$, $z_k^*>\max_{o\in\mathcal O_k}\theta_i(v_i(o))$ (strictly since we assumed no ties).
\end{itemize}
(a) and (b) imply that if there is a reason to lie about one's type, it is to achieve a strictly higher value. In order to do this, a bidder $i$ must move up in the ranking; however, this requires placing a bid $b_i(o)$ for some outcome such that $\theta_i(b_i(o))\geq z_{r-1}^*$ and will cause bidder $i$ to pay $p_i\geq \theta_i^{-1}(z_{r-1}^*)$. By (c) this implies $p_i>\max_ov_i(o)$, i.e. bidder $i$ would necessarily pay more than its value.

As in~\ref{thm:greedy-mech}, ties happen with measure zero when the bid space is continuous and we find that the mechanism is DSIC-AE.

Moreover, when values are discretized additional analysis reveals that the mechanism is DSIC. Note that our argument above only gets into trouble when the inequality in (c) is in fact equality, i.e. $z_{r-1}^*=\max_{o\in\mathcal O_k}\theta_i(v_i(o))$. In particular, this implies that there is an outcome $o'\neq o^*$ such that $z_{r-1}^*=\theta_i(v_i(o'))$. Suppose that $i$ lies and reports $v_i'$ instead, inducing the outcome $o'$. The payment $p_i'$ will be (replacing $\inf$ with $\min$ because we are in a discretized space with a minimum bid increment):
\[p_i'=\min \left\{b_i''(o^+)\left|o^+=\mbox{\tfgreedy{$b_{-i},b_i''$} and }b_j'(o^+)=b_j'(o')\right.\right\}\geq v_i(o')+\delta\]
where $\delta$ represents the minimum bid increment and the inequality follows because $i$ needed to increase its bid to get $o'$. This implies $p_i'\geq v_i(o')+\delta>v_i(o')$ and therefore $i$ does not benefit by lying in this scenario either. Thus, the mechanism is DSIC when values are discrete.
\end{proof}

%\subsection{Bounding Welfare}
%\label{appendix:BW}
%While the existence of truthful mechanisms is a positive result, a greedy optimization cannot generally guarantee a welfare approximation better than $\Theta(n)$:
%\begin{lemma}
%No transformed greedy mechanism can guarantee more than than a $\frac1{n}$ fraction of the optimal welfare in the worst case.
%\end{lemma}
%\begin{proof}
%Suppose there are at least two outcomes and $n$ bidders. Pick any non-trivial transformed greedy mechanism (i.e. a mechanism that realizes at least two outcomes for some inputs) with transformations $\theta_i$ and offsets $\theta_0$.
%
%We label bidders and select $v$ such that $\theta_1(v)>\theta_i(v-\epsilon)$ for all $i>1$. Let bidder 1 have value $v_1=(1, 1-\epsilon, 0,\dots)$ and let other bidders have values $v_{i}=(0,1-\epsilon,0,\dots)$. The welfare-optimal outcome is outcome 2, with a total welfare of $(n-1)(1-\epsilon)$; however, a greedy mechanism must choose outcome 1 because $\theta_1(v)>\theta_i(v-\epsilon)$ for all $i$, leading to a welfare of $1$. This implies a worst-case welfare approximation of $\frac{1}{n(1-\epsilon)}$.
%
%The non-transformed greedy mechanism will achieve a welfare of at least $\max_{i,o}v_i(o)\geq\frac1n\max_o\sum_iv_i(o)$ and therefore guarantee at least a $\frac1n$ fraction of the optimal welfare.
%\end{proof}




==> xstring.tex <==
%  __________________________________________________
% |                                                  |
% |                                                  |
% |                   xstring v1.7c                  |
% |                                                  |
% |                  13 octobre 2013                 |
% |                                                  |
% |__________________________________________________|
%
% This is xtring.tex
%
% "xstring" package consists of the 7 following files:
%   xstring.tex (this file)
%   xstring.sty
%   README
%   xstring_doc_fr.tex, xstring_doc_fr.pdf (manual in french)
%   xstring_doc_en.tex, xstring_doc_en.pdf (manual in english)
%
% Christian Tellechea 2008-2013
% email : unbonpetit@gmail.com
% -------------------------------------------------------------------
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%
%     http://www.latex-project.org/lppl.txt
%
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% -------------------------------------------------------------------
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Christian Tellechea
% -------------------------------------------------------------------
\def\xstringversion     {1.7c}
\def\xstringdate        {2013/10/13}
\def\xstringfrenchdate  {13 octobre 2013}
\def\xstringenglishdate {13 october 2013}
\edef\CurrentAtCatcode  {\the\catcode`\@}
\catcode`\@=11
\newwrite\@xs@message% canal pour les messages
\newcount\integerpart
\newcount\decimalpart% compteurs utilis\'es par xstring

\expandafter\ifx\csname @latexerr\endcsname\relax% on n'utilise pas LaTeX ?
	\immediate\write\m@ne{Package: xstring \xstringdate\space\space v\xstringversion\space\space String manipulations}%
	\long\def\@firstoftwo#1#2{#1}
	\long\def\@secondoftwo#1#2{#2}
	\long\def\@gobble#1{}
	\long\def\@ifnextchar#1#2#3{%
		\let\reserved@d=#1%
		\def\reserved@a{#2}%
		\def\reserved@b{#3}%
		\futurelet\@let@arg\@ifnch}
	\def\@ifnch{%
		\ifx\@let@arg\@sptoken
			\let\reserved@c\@xifnch
		\else
			\ifx\@let@arg\reserved@d
				\let\reserved@c\reserved@a
			\else
				\let\reserved@c\reserved@b
			\fi
		\fi
		\reserved@c}
	\def\:{\let\@sptoken= } \:
	\def\:{\@xifnch} \expandafter\def\: {\futurelet\@let@arg\@ifnch}
	\def\@ifstar#1{\@ifnextchar *{\@firstoftwo{#1}}}
	\long\def\@testopt#1#2{\@ifnextchar[{#1}{#1[{#2}]}}
	\def\@empty{}
\fi% fin des d\'efinitions LaTeX

\long\def\@xs@ifempty#1{%
	\expandafter\ifx\expandafter\relax\detokenize{#1}\relax
		\expandafter\@firstoftwo
	\else
		\expandafter\@secondoftwo
	\fi
}
% Ouvre un groupe o\`u les catcodes sont \`a 12 et \`a 10 pour les espaces
% ensuite, appelle \@xs@ReadVerb qui lit un argument entre d\'elimiteurs verb
\def\@xs@MakeVerb{% lit 1 argument et le transforme en verb
	\begingroup% groupe o\`u les catcodes sont \`a 12 pour la lecture suivante
		\def\do##1{\catcode`##112\relax}%
		\dospecials% on entre dans le mode verb
		\obeyspaces% et on tient compte des espaces
		\@xs@ReadVerb% et on va lire l'argument
}

% D\'efinit \@xs@ReadVerb qui lit un argument entre d\'elimiteurs verb
\def\setverbdelim#1{% d\'efinit quel est le d\'elimiteur de verb
	\expandafter\@xs@ifempty\expandafter{\@gobble#1}%
		\relax
		{\begingroup
			\newlinechar`\^^J%
			\immediate\write\@xs@message
			{Package xstring Warning: verb delimiter is not a single token on input line \the\inputlineno^^J}%
		\endgroup
		}%
	\def\@xs@ReadVerb##1#1##2#1{% lit ##2 qui est entre les d\'elimiteurs de verb
		\endgroup% on ferme le groupe
		\@xs@afterreadverb{##2}}% on appelle l'ex\'ecution de fin
}

% Assigne l'argument entre d\'elimiteur verb dans la sc #1' +
\def\verbtocs#1{%
	\def\@xs@afterreadverb##1{\def#1{##1}}%
	\@xs@MakeVerb
}

\begingroup
	\catcode\z@3 \def\@xs@twochars{^^00}%
	\catcode\z@7 \xdef\@xs@twochars{\@xs@twochars^^00}%
\endgroup

\edef\@xs@reserved@A{\long\def\noexpand\@xs@AssignResult##1\@xs@twochars}

\@xs@reserved@A#2{\endgroup\expandafter\def\expandafter#2\expandafter{\@gobble#1}}

\def\tokenize#1#2{%
	\begingroup
		\@xs@def\@xs@reserved@A{#2}% on d\'eveloppe en accord avec \fullexpandarg ou \noexpandarg
		\everyeof\expandafter{\@xs@twochars#1}% met "^^@^^@#1" \`a la fin du fichier virtuel
		\endlinechar\m@ne
		\expandafter\@xs@AssignResult\scantokens\expandafter{\expandafter\relax\@xs@reserved@A}% on fait l'assignation
}%

% Macro tr\`es simple qui assigne ou affiche le r\'esultat, selon la pr\'esence
% ou non de #2 qui est l'argument optionnel venant en derni\`ere position des macros
\long\def\@xs@ReturnResult#1#2{%
	\def\@xs@argument@A{#1}%
	\@xs@ifempty{#2}%
		\@xs@argument@A
		{\let#2\@xs@argument@A}%
}

\def\@xs@ldef{\long\def}

\def\@xs@ledef{\long\edef}

% Pas d'expansion des arguments
\def\normalexpandarg{%
	\let\@xs@def\@xs@ldef% on d\'efinit \@xs@call avec \def
	\def\@xs@expand##1{\unexpanded\expandafter{##1}}}
\let\noexpandarg\normalexpandarg% synonyme

% 1-d\'eveloppement du premier token des arguments
\def\expandarg{%
	\let\@xs@def\@xs@ldef% on d\'efinit \@xs@call avec \def
	\def\@xs@expand##1{\unexpanded\expandafter\expandafter\expandafter{##1}}%
}

% D\'eveloppement maximum des arguments
\def\fullexpandarg{%
	\let\@xs@def\@xs@ledef% on d\'efinit\@xs@call avec \edef
	\def\@xs@expand##1{##1}% et on neutralise \@xs@expand
}

\def\saveexpandmode{\let\@xs@saved@def\@xs@defarg\let\@xs@saved@expand\@xs@expand}

\def\restoreexpandmode{\let\@xs@defarg\@xs@saved@def\let\@xs@expand\@xs@saved@expand}

% Macro interne renvoyant #2 si son argument commence par une accolade ouvrante "{"
% et #3 sinon (Ulrich Diez sur comp.text.tex)
\long\def\@xs@ifbeginwithbrace#1{%
	\csname @%
		\expandafter\@gobble\string{%
		\expandafter\@gobble\expandafter{\expandafter{\string#1}%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\@firstoftwo
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\@gobble
		\expandafter\expandafter\expandafter\@gobble
		\expandafter\expandafter\expandafter{\expandafter\string\expandafter}\string}%
		\expandafter\@gobble\string}%
		\@secondoftwo{first}{second}oftwo%
	\endcsname
}

% Cette macro interne prend la 1ere unit\'e syntaxique de #1 et assigne le r\'esultat \`a #2
\long\def\@xs@returnfirstsyntaxunit#1#2{%
	\def\@xs@groupfound{\expandafter\def\expandafter#2\expandafter{\expandafter{#2}}\@xs@gobbleall}% on met #2 dans des accolades et on finit
	\long\def\@xs@assignfirsttok##1##2\@xs@nil{\let\@xs@toks0\def#2{##1}}%
	\def\@xs@testfirsttok{%
		\let\@xs@next\@xs@assignfirsttok
		\ifx\@xs@toks\bgroup
			\expandafter\@xs@ifbeginwithbrace\expandafter{\@xs@argument}{\def\@xs@next{\afterassignment\@xs@groupfound\def#2}}{}%
		\fi
		\@xs@next}%
	\def\@xs@argument{#1}%
	\edef\@xs@next{\expandafter\@xs@beforespace\detokenize{#1} \@xs@nil}% #1 commence par un espace ?
	\ifx\@xs@next\@empty
		\def\@xs@next{\expandafter\ifx\expandafter\@empty\detokenize\expandafter{\@xs@argument}\@empty\let#2\@empty\else\def#2{ }\let\@xs@toks0\fi}%
	\else
		\def\@xs@next{\expandafter\futurelet\expandafter\@xs@toks\expandafter\@xs@testfirsttok\@xs@argument\@xs@nil}%
	\fi
	\@xs@next
}

% Cette macro interne enl\`eve la 1ere unit\'e syntaxique de #1 et assigne le r\'esultat \`a #2
\long\def\@xs@testsecondtoken#1\@xs@nil{\@xs@ifbeginwithbrace{#1}}

\long\def\@xs@gobblespacebeforebrace#1#{}% supprime tout ce qui est avant la 1ere accolade ouvrante

\long\def\@xs@removefirstsyntaxunit#1#2{%
	\def\@xs@argument{#1}%
	\expandafter\expandafter\expandafter\ifx\expandafter\expandafter\expandafter\@empty\expandafter\@xs@beforespace\detokenize\expandafter{\@xs@argument} \@xs@nil\@empty% #1 commence par un espace ?
		\expandafter\@xs@ifempty\expandafter{\@xs@argument}%
			{\let#2\@empty}
			{\afterassignment\@xs@testsecondtoken% après avoir mangé le 1er token, on va tester si la suite commence par «{»
			\expandafter\let\expandafter\@xs@secontoken\expandafter=\expandafter\@sptoken\@xs@argument\@xs@@nil\@xs@nil% on mange le 1er token et on rajoute \@xs@@nil à la fin pour éviter de perdre les accolades du groupe
				{\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#2%
				 \expandafter\expandafter\expandafter{\expandafter\@xs@gobblespacebeforebrace\@xs@argument}}%
				{\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#2%
				 \expandafter\expandafter\expandafter{\expandafter\@xs@behindspace\@xs@argument\@xs@nil}}%
			}%
	\else
		\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#2%
		\expandafter\expandafter\expandafter{\expandafter\@gobble\@xs@argument}%
	\fi
}

% Macros \`a arguments d\'elimit\'es pour les macros ci dessus
\long\def\@xs@beforespace#1 #2\@xs@nil{#1}

\long\def\@xs@behindspace#1 #2\@xs@nil{#2}

\long\def\@xs@returnfirstsyntaxunit@ii#1#2\@xs@nil{#1}

\long\def\@xs@gobbleall#1\@xs@nil{}

% Cette macro interne est utilis\'ee dans les macros \'etoil\'ees pour :
% 1) d\'evelopper l'argument selon qu'on a choisit \fullexpandarg
%    ou \normalexpandarg, et ceci \`a l'aide de la macro \@xs@def
% 2) Ensuite, on d\'etokenize ce d\'eveloppement de façon n'avoir plus que
%    des catcodes de 10 pour les espaces et 12 pour le reste.
\long\def\@xs@expand@and@detokenize#1#2{%
	\long\def#1{#2}%
	\expandafter\edef\expandafter#1\expandafter{\@xs@expand#1}% on d\'eveloppe #2 selon le mode de d\'eveloppement
	\long\edef#1{\detokenize\expandafter{#1}}% puis on d\'etokenize et on assigne \`a #1
}

\long\def\@xs@expand@and@assign#1#2{\@xs@def#1{#2}}% on d\'eveloppe #2 selon \fullexpandarg ou \normalexpandarg

\long\def\@xs@edefaddtomacro#1#2{\edef#1{\unexpanded\expandafter{#1}#2}}

\long\def\@xs@addtomacro#1#2{\expandafter\def\expandafter#1\expandafter{#1#2}}

\def\@xs@argstring{0########1########2########3########4########5########6########7########8########9}

% \@xs@DefArg{3} met dans la sc \@xs@myarg les tokens "####1####2####3"
\def\@xs@DefArg#1{\def\@xs@defarg0##1#1##2\@xs@nil{\def\@xs@myarg{##1#1}}\expandafter\@xs@defarg\@xs@argstring\@xs@nil}

% \@xs@DefArg@{3} met dans la sc \@xs@myarg les tokens "[####1]####2####3####4"
\def\@xs@DefArg@#1{\expandafter\@xs@defarg@\expandafter{\number\numexpr#1+1}}

\def\@xs@defarg@#1{\def\@xs@defarg0##11##2#1##3\@xs@nil{\def\@xs@myarg{[##11]##2#1}}\expandafter\@xs@defarg\@xs@argstring\@xs@nil}

% \@xs@OneArg{3} met dans la sc \@xs@myarg les tokens "####3"
\def\@xs@OneArg#1{\expandafter\@xs@onearg\expandafter{\number\numexpr#1-1}{#1}}

\def\@xs@onearg#1#2{\def\@xs@defarg##1#1##2#2##3\@xs@nil{\def\@xs@myarg{##2#2}}\expandafter\@xs@defarg\@xs@argstring\@xs@nil}

% #1 : num\'ero du 1er argument; #2 : nombre de lignes; #3 argument optionnel; #4 : dernier num\'ero de l'argument devant être d\'etokenis\'e si \'etoile
\def\@xs@BuildLines#1#2#3#4{%
	\let\@xs@newlines\@empty
	\let\@xs@newargs\@empty
	\def\@xs@buildlines##1{%
		\expandafter\@xs@OneArg\expandafter{\number\numexpr##1+#1-1}%
		\edef\@xs@reserved@B{\noexpand\@xs@expand\csname @xs@arg@\romannumeral\numexpr##1\endcsname}%
		\ifnum##1=\@ne% si c'est le premier argument
			\@xs@ifempty{#3}%
				{\expandafter\@xs@addtomacro\expandafter\@xs@newargs\expandafter{\expandafter{\@xs@reserved@B}}%
				\edef\@xs@reserved@B{\ifnum##1>#4 @xs@def\else @xs@assign\fi}%
				}% et s'il y a un argument optionnel alors, on met des crochets
				{\expandafter\@xs@addtomacro\expandafter\@xs@newargs\expandafter{\expandafter[\@xs@reserved@B]}%
				\def\@xs@reserved@B{@xs@def}% ne pas d\'etok\'eniser l'argument optionnel grace au \@xs@def
				}
		\else
			\expandafter\@xs@addtomacro\expandafter\@xs@newargs\expandafter{\expandafter{\@xs@reserved@B}}%
			\edef\@xs@reserved@B{\ifnum##1>#4 @xs@def\else @xs@assign\fi}%
		\fi
		\edef\@xs@newlines{\unexpanded\expandafter{\@xs@newlines}\expandafter\noexpand\csname\@xs@reserved@B\endcsname\expandafter\noexpand\csname @xs@arg@\romannumeral\numexpr##1\endcsname{\@xs@myarg}}%
		\ifnum##1<#2\relax
			\def\@xs@next{\expandafter\@xs@buildlines\expandafter{\number\numexpr##1+1}}%
			\expandafter\@xs@next
		\fi}%
	\@xs@buildlines\@ne
}

\def\@xs@newmacro{%
	\@ifstar
		{\let\@xs@reserved@D\@empty\@xs@newmacro@}
		{\let\@xs@reserved@D\relax\@xs@newmacro@0}%
}

% #1 : dernier num\'ero de l'argument devant être d\'etokenis\'e
% #2 : nom de la macro publique
% #3 : argument optionnel (vide si pas d'arg optionnel)
% #4 : nombre d'arguments obligatoires
% #5 : utilisation de testopt (1 si oui, 0 si non)
% #6 : code de la macro
\def\@xs@newmacro@#1#2#3#4#5{%
	\edef\@xs@reserved@A{@xs@\expandafter\@gobble\string#2}%
	\edef\@xs@reserved@C{\expandafter\noexpand\csname\@xs@reserved@A @\ifx\@empty#3\@empty @\fi\endcsname}%
	\edef\@xs@reserved@B{%
		\ifx\@empty\@xs@reserved@D
			\def\noexpand#2{\noexpand\@ifstar
				{\let\noexpand\@xs@assign\noexpand\@xs@expand@and@detokenize\expandafter\noexpand\@xs@reserved@C}%
				{\let\noexpand\@xs@assign\noexpand\@xs@expand@and@assign\expandafter\noexpand\@xs@reserved@C}%
			}%
		\else
			\def\noexpand#2{\let\noexpand\@xs@assign\noexpand\@xs@expand@and@assign\expandafter\noexpand\@xs@reserved@C}%
		\fi
		\ifx\@empty#3\@empty
		\else
			\def\expandafter\noexpand\@xs@reserved@C{%
				\noexpand\@testopt{\expandafter\noexpand\csname\@xs@reserved@A @@\endcsname}{\ifx\@xs@def\@xs@ledef#3\else\unexpanded{#3}\fi}}%
		\fi
	}%
	% Que fait \@xs@reserved@B ? Il d\'efinit :
	% si #3 est vide : \NOM{\@ifstar{\let\@xs@assign\@xs@expand@and@detokenize\@xs@NOM@@}{\let\@xs@assign\@xs@expand@and@assign\@xs@NOM@@}}
	% si #3 existe   : \NOM{\@ifstar{\let\@xs@assign\@xs@expand@and@detokenize\@xs@NOM@}{\let\@xs@assign\@xs@expand@and@assign\@xs@NOM@}}
	%                  \@xs@NOM@{\@testopt{\@xs@NOM@@}{#3}}}
	\long\@xs@reserved@B
	\ifx\@empty#3\@empty
		\@xs@BuildLines1{#4}{#3}{#1}%
		\@xs@DefArg{#4}%
	\else
		\expandafter\@xs@BuildLines\expandafter1\expandafter{\number\numexpr#4+1}{#3}{#1}%
		\@xs@DefArg@{#4}%
	\fi
	\edef\@xs@reserved@B{\def\expandafter\noexpand\csname\@xs@reserved@A @@\endcsname\@xs@myarg}%
	\edef\@xs@reserved@C{\unexpanded\expandafter{\@xs@newlines}\edef\noexpand\@xs@call}%
	\edef\@xs@reserved@D{%
		\noexpand\noexpand\expandafter\noexpand\csname\@xs@reserved@A\endcsname\unexpanded\expandafter{\@xs@newargs}%
	}%
	\ifnum#5=\@ne\edef\@xs@reserved@D{\noexpand\noexpand\noexpand\@testopt{\unexpanded\expandafter{\@xs@reserved@D}}{}}\fi
	\@xs@edefaddtomacro\@xs@reserved@C{{\unexpanded\expandafter{\@xs@reserved@D}}\noexpand\@xs@call}%
	\@xs@edefaddtomacro\@xs@reserved@B{{\unexpanded\expandafter{\@xs@reserved@C}}}%
	% Que fait \@xs@reserved@B ? Il d\'efinit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def\@xs@NOM@@[##2]##3##4##5{%
	%          \@xs@def\@xs@arg@i{##2}\@xs@assign\@xs@arg@ii{##3}\@xs@assign\@xs@arg@iii{##4}\@xs@asign\@xs@arg@iv{##5}%
	% si #5=0: \edef\@xs@call{\noexpand\@xs@NOM[\@xs@expand\@xs@arg@i]{\@xs@expand\@xs@arg@ii}{\@xs@expand\@xs@arg@iii}{\@xs@expand\@xs@arg@iv}}%
	% si #5=1: \edef\@xs@call{\noexpand\@testopt{\noexpand\@xs@NOM[\@xs@expand\@xs@arg@i]{\@xs@expand\@xs@arg@i}{\@xs@expand\@xs@arg@ii}{\@xs@expand\@xs@arg@iii}{\@xs@expand\@xs@arg@iv}}{}}%
	%          \@xs@call}
	\long\@xs@reserved@B
	\edef\@xs@reserved@B{%
		\def\expandafter\noexpand\csname\@xs@reserved@A\endcsname
			\@xs@myarg\ifnum#5=\@ne[\unexpanded{##}\number\numexpr\ifx\@empty#3\@empty#4+1\else#4+2\fi]\fi
	}%
	% Que fait \@xs@reserved@B ? Il d\'efinit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def \@xs@NOM[##2]##3##4##5[##6]{#6}
	\long\@xs@reserved@B
}

% macro g\'en\'erique qui lit \@xs@reserved@C us par us
% 3 sous-routines sont appel\'ees \`a des moments cl\'e :
% \@xs@atendofgroup      (un groupe se finit, appel r\'ecursif)
% \@xs@atbegingroup      (un groupe vient d'être ouvert)
% \@xs@atnextsyntaxunit  (la future US n'est pas un groupe)
\def\@xs@read@reserved@C{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		{\ifnum\@xs@nestlevel=\z@
			\let\@xs@next\relax
		\else
			\let\@xs@next\@xs@atendofgroup
		\fi
		}
		{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@A
		\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
		\let\@xs@next\@xs@read@reserved@C
		\@xs@exploregroups
		\ifx\bgroup\@xs@toks
			\advance\integerpart\@ne
			\begingroup
				\expandafter\def\expandafter\@xs@reserved@C\@xs@reserved@A
				\@xs@manage@groupID
				\let\@xs@nestlevel\@ne
				\integerpart\z@
				\@xs@atbegingroup
		\else
			\global\advance\decimalpart\@ne
			\@xs@atnextsyntaxunit
		\fi
		}%
	\@xs@next
}

% macro g\'en\'erique qui lit \@xs@reserved@D en proc\'edant \`a des tests avec \IfBeginWith
% 2 sous-routines sont appel\'ees \`a des moments cl\'e :
% \@xs@atendofgroup      (un groupe se finit, appel r\'ecursif)
% \@xs@atoccurfound      (une occurrence a \'et\'e trouv\'ee)
\def\@xs@read@reserved@D{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@D}%
		{\ifnum\@xs@nestlevel=\z@
			\let\@xs@next\relax
		\else
			\let\@xs@next\@xs@atendofgroup
		\fi
		}%
		{\expandafter\expandafter\expandafter\@xs@IfBeginWith@i\expandafter\expandafter\expandafter
			{\expandafter\@xs@reserved@D\expandafter}\expandafter{\@xs@reserved@E}%
			{\global\advance\decimalpart\@ne
			\let\@xs@reserved@D\@xs@reserved@A
			\@xs@atoccurfound
			}%
			{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@A
			\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@D
			\let\@xs@next\@xs@read@reserved@D
			\@xs@exploregroups
			\ifx\bgroup\@xs@toks
				\advance\integerpart\@ne
				\begingroup
					\expandafter\def\expandafter\@xs@reserved@D\@xs@reserved@A
					\@xs@manage@groupID
					\let\@xs@reserved@C\@empty
					\let\@xs@nestlevel\@ne
					\integerpart\z@
			\else
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@A}%
			\fi
			}%
		}%
	\@xs@next
}

\@xs@newmacro\StrRemoveBraces{}{1}{1}{%
	\def\@xs@reserved@C{#1}%
	\let\@xs@reserved@B\@empty
	\let\@xs@nestlevel\z@
	\@xs@StrRemoveBraces@i
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#2}%
}

\def\@xs@StrRemoveBraces@i{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		{\ifnum\@xs@nestlevel=\z@
			\let\@xs@next\relax
		\else
			\expandafter\endgroup
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\@xs@reserved@B}%
			\let\@xs@next\@xs@StrRemoveBraces@i
		\fi
		}
		{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@A
		\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
		\let\@xs@next\@xs@StrRemoveBraces@i
		\ifx\bgroup\@xs@toks
			\ifx\@xs@exploregroups\relax% on explore les groupes ?
				\begingroup
					\expandafter\def\expandafter\@xs@reserved@C\@xs@reserved@A
					\let\@xs@nestlevel\@ne
					\integerpart\z@
					\let\@xs@reserved@B\@empty
			\else
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\@xs@reserved@A
			\fi
		\else
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\@xs@reserved@A}%
		\fi
		}%
	\@xs@next
}

% \@xs@cutafteroccur coupe l'argument #1 apr\`es la #3\`eme occurrence de #2
% \@xs@reserved@C : contient ce qui se trouve avant cette occurrence
% \@xs@reserved@D : contient ce qui se trouve avant cette occurrence y compris cette occurrence
% \@xs@reserved@E : contient ce qui se trouve apr\`es l'occurrence
% si l'occurrence n'existe pas ou qu'un des arguments est vide, toutes les chaines renvoy\'ees sont vides
\long\def\@xs@cutafteroccur#1#2#3{%
	\ifnum#3<\@ne\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
		{\let\@xs@reserved@C\@empty
		\let\@xs@reserved@E\@empty
		\global\let\groupID\@empty
		}
		{\@xs@cutafteroccur@i{#1}{#2}{#3}}%
}
	
\long\def\@xs@cutafteroccur@i#1#2#3{%
	\def\@xs@reserved@D{#1}\let\@xs@reserved@C\@empty\def\@xs@reserved@E{#2}%
	\decimalpart\z@
	\integerpart\z@
	\gdef\groupID{0}%
	\let\@xs@nestlevel\z@
	\def\@xs@atendofgroup{%
		\expandafter\endgroup
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
		\@xs@read@reserved@D}%
	\def\@xs@atoccurfound{%
		\ifnum\decimalpart=\numexpr(#3)\relax
			\global\let\@xs@reserved@D\@xs@reserved@D
			\global\let\@xs@reserved@C\@xs@reserved@C
			\@xs@exitallgroups
			\let\@xs@next\relax
		\else
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@E}%
			\let\@xs@next\@xs@read@reserved@D
		\fi}%
	\@xs@read@reserved@D
	\def\@xs@argument@A{#2}%
	\ifnum\decimalpart=\numexpr(#3)\relax % occurrence trouv\'ee ?
		\let\@xs@reserved@E\@xs@reserved@D
		\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter\@xs@reserved@D\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\@xs@argument@A}%
	\else
		\let\@xs@reserved@C\@empty
		\let\@xs@reserved@E\@empty
		\global\let\groupID\@empty
	\fi
}

\@xs@newmacro*3\IfSubStr{1}{2}{0}{%
	\def\@xs@argument@A{#2}\def\@xs@argument@B{#3}%
	\expandafter\expandafter\expandafter\@xs@cutafteroccur
	\expandafter\expandafter\expandafter{\expandafter\@xs@argument@A\expandafter}\expandafter{\@xs@argument@B}{#1}%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@D}%
		\@secondoftwo
		\@firstoftwo
}

\@xs@newmacro*2\IfBeginWith{}{2}{0}{%
	\def\@xs@argument@A{#1}\def\@xs@argument@B{#2}%
	\expandafter\@xs@ifempty\expandafter{\@xs@argument@B}%
		{\let\@xs@next\@secondoftwo
		}
		{\def\@xs@next{%
			\expandafter\expandafter\expandafter\@xs@IfBeginWith@i\expandafter\expandafter\expandafter
				{\expandafter\@xs@argument@A\expandafter}\expandafter
				{\@xs@argument@B}}%
		}%
	\@xs@next
}

\long\def\@xs@IfBeginWith@i#1#2{%
	\def\@xs@argument@A{#1}\def\@xs@argument@B{#2}%
	\expandafter\@xs@ifempty\expandafter{\@xs@argument@B}%
		{\let\@xs@next\@firstoftwo% #2 est vide, tous les tests sont pass\'es avec succ\`es : on renvoie #3
		}
		{\expandafter\@xs@ifempty\expandafter{\@xs@argument@A}%
			{\let\@xs@next\@secondoftwo% #1 est vide, c'est que #2 est + long que #1 : on renvoie #4
			}
			{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@argument@B}\@xs@reserved@B
			\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@A
			\ifx\@xs@reserved@A\@xs@reserved@B% il y a \'egalit\'e...
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@B}\@xs@reserved@B
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@A% on enl\`eve les 1ere unit\'es syntaxiques
				\def\@xs@next{% et on recommence avec ces arguments racourcis d'1 unit\'e syntaxique
					\expandafter\expandafter\expandafter\@xs@IfBeginWith@i
					\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@A\expandafter}\expandafter{\@xs@reserved@B}}%
			\else
				\let\@xs@next\@secondoftwo
			\fi
			}%
		}%
	\@xs@next
}

\@xs@newmacro*2\IfEndWith{}{2}{0}{%
	\def\@xs@argument@A{#1}\def\@xs@argument@B{#2}%
	\@xs@ifempty{#2}%
		{\let\@xs@reserved@A\@secondoftwo
		}
		{\expandafter\expandafter\expandafter\@xs@StrCount
			\expandafter\expandafter\expandafter{\expandafter\@xs@argument@A\expandafter}\expandafter
			{\@xs@argument@B}[\@xs@reserved@A]%
		\ifnum\@xs@reserved@A=\z@
			\let\@xs@reserved@A\@secondoftwo
		\else
			\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
				{\let\@xs@reserved@A\@firstoftwo}
				{\let\@xs@reserved@A\@secondoftwo}%
		\fi
		}%
	\@xs@reserved@A
}

\@xs@newmacro*4\IfSubStrBefore{1,1}{3}{0}{\@xs@IfSubStrBefore@i[#1]{#2}{#3}{#4}}

\def\@xs@IfSubStrBefore@i[#1,#2]#3#4#5{%
	\def\@xs@reserved@C{#3}%
	\ifx\@xs@exploregroups\relax% si on explore les groupes
		\let\@xs@reserved@B\@empty
		\let\@xs@nestlevel\z@
		\@xs@StrRemoveBraces@i% on retire les accolades
		\let\@xs@reserved@C\@xs@reserved@B
	\fi
	\def\@xs@reserved@A{#5}%
	\expandafter\expandafter\expandafter\@xs@cutafteroccur\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\expandafter}\expandafter{\@xs@reserved@A}{#2}%
	\def\@xs@reserved@A{#4}%
	\expandafter\expandafter\expandafter\@xs@cutafteroccur\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\expandafter}\expandafter{\@xs@reserved@A}{#1}%
	\global\let\groupID\@empty
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		\@secondoftwo
		\@firstoftwo
}

\@xs@newmacro*4\IfSubStrBehind{1,1}{3}{0}{\@xs@IfSubStrBehind@i[#1]{#2}{#3}{#4}}

\long\def\@xs@IfSubStrBehind@i[#1,#2]#3#4#5{\@xs@IfSubStrBefore@i[#2,#1]{#3}{#5}{#4}}

\long\def\@xs@formatnumber#1#2{%
	\def\@xs@argument@A{#1}%
	\@xs@ifempty{#1}%
		{\def#2{0X}% si vide, renvoie 0X
		}
		{\@xs@returnfirstsyntaxunit{#1}\@xs@reserved@A
		\def\@xs@reserved@B{+}%
		\ifx\@xs@reserved@A\@xs@reserved@B
			\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@C
			\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
			 	{\def#2{+0X}}
			 	{\expandafter\def\expandafter#2\expandafter{\expandafter+\expandafter0\@xs@reserved@C}}%
		\else
			\def\@xs@reserved@B{-}%
			\ifx\@xs@reserved@A\@xs@reserved@B
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@A
				\expandafter\@xs@ifempty\expandafter{\@xs@reserved@A}%
					{\def#2{-0X}}%
					{\expandafter\def\expandafter#2\expandafter{\expandafter-\expandafter0\@xs@reserved@A}}%
			\else
				\expandafter\def\expandafter#2\expandafter{\expandafter0\@xs@argument@A}%
			\fi
		\fi
		}%
}

\@xs@newmacro\IfInteger{}{1}{0}{%
	\@xs@formatnumber{#1}\@xs@reserved@A
	\decimalpart\z@
	\afterassignment\@xs@defafterinteger\integerpart\@xs@reserved@A\relax\@xs@nil
	\let\@xs@after@intpart\@xs@afterinteger
	\expandafter\@xs@testdot\@xs@afterinteger\@xs@nil
	\ifx\@empty\@xs@afterdecimal
		\ifnum\decimalpart=\z@
			\let\@xs@next\@firstoftwo% partie décimale constituée de 0 --> seul cas où on renvoie vrai
		\else
			\let\@xs@afterinteger\@xs@after@intpart
			\let\@xs@next\@secondoftwo
		\fi
	\else
		\let\@xs@afterinteger\@xs@after@intpart
		\let\@xs@next\@secondoftwo
	\fi
	\@xs@next
}

\@xs@newmacro\IfDecimal{}{1}{0}{%
	\@xs@formatnumber{#1}\@xs@reserved@A
	\decimalpart\z@
	\afterassignment\@xs@defafterinteger\integerpart\@xs@reserved@A\relax\@xs@nil
	\expandafter\@xs@testdot\@xs@afterinteger\@xs@nil
	\ifx\@empty\@xs@afterdecimal
		\expandafter\@firstoftwo
	\else
		\expandafter\@secondoftwo
	\fi
}

\long\def\@xs@defafterinteger#1\relax\@xs@nil{\def\@xs@afterinteger{#1}}

\def\@xs@testdot{%
	\let\xs@decsep\@empty
	\@ifnextchar.%
		{\def\xs@decsep{.}\@xs@readdecimalpart}%
		{\@xs@testcomma}%
}

\def\@xs@testcomma{%
	\@ifnextchar,%
		{\def\xs@dessep{,}\@xs@readdecimalpart}%
		{\@xs@endnumber}%
}

\long\def\@xs@readdecimalpart#1#2\@xs@nil{%
	\ifx\@empty#2\@empty
		\def\@xs@reserved@A{0X}%
	\else
		\def\@xs@reserved@A{0#2}%
	\fi
	\afterassignment\@xs@defafterinteger\decimalpart\@xs@reserved@A\relax\@xs@nil
	\expandafter\@xs@endnumber\@xs@afterinteger\@xs@nil
}

\long\def\@xs@endnumber#1\@xs@nil{\def\@xs@afterdecimal{#1}}

% test d'\'egalit\'e sur des chaines (et des chaines contenant des nombres)
\long\def\@xs@IfStrEqFalse@i#1#2{\let\@xs@reserved@A\@secondoftwo}
\long\def\@xs@IfStrEqFalse@ii#1#2{% renvoie vrai si les 2 arg sont d\'ecimaux et s'ils sont \'egaux, faux sinon
	\@xs@IfDecimal{#1}%
		{\@xs@IfDecimal{#2}%
			{\ifdim#1pt=#2pt
				\let\@xs@reserved@A\@firstoftwo
			\else
				\let\@xs@reserved@A\@secondoftwo
			\fi% les 2 sont d\'ecimaux : on fait le test
			}%
			{\let\@xs@reserved@A\@secondoftwo}% un seul est d\'ecimal
		}%
		{\let\@xs@reserved@A\@secondoftwo}% #1 n'est pas d\'ecimal
}

\long\def\@xs@TestEqual#1#2{% teste si les 2 arguments sont \'egaux
	\def\@xs@reserved@A{#1}\def\@xs@reserved@B{#2}%
	\ifx\@xs@reserved@A\@xs@reserved@B
		\let\@xs@reserved@A\@firstoftwo% \'egalit\'e parfaite des 2 chaines
	\else
		\expandafter\expandafter\expandafter\@xs@reserved@D\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@A\expandafter}\expandafter{\@xs@reserved@B}%
	\fi
	\@xs@reserved@A
}

\@xs@newmacro*2\IfStrEq{}{2}{0}{% teste si les deux chaines sont \'egales
	\let\@xs@reserved@D\@xs@IfStrEqFalse@i
	\@xs@TestEqual{#1}{#2}%
}

\@xs@newmacro*2\IfEq{}{2}{0}{% teste si les 2 arguments (chaine ou nombre) sont \'egaux
	\let\@xs@reserved@D\@xs@IfStrEqFalse@ii
	\@xs@TestEqual{#1}{#2}%
}

\def\IfStrEqCase{%
	\@ifstar
		{\def\@xs@reserved@E{\IfStrEq*}\@xs@IfStrCase}%
		{\def\@xs@reserved@E{\IfStrEq}\@xs@IfStrCase}%
}

\long\def\@xs@IfStrCase#1#2{\@testopt{\@xs@IfStringCase{#1}{#2}}{}}

\def\IfEqCase{%
	\@ifstar
		{\def\@xs@reserved@E{\IfEq*}\@xs@IfEqCase}%
		{\def\@xs@reserved@E{\IfEq}\@xs@IfEqCase}%
}

\long\def\@xs@IfEqCase#1#2{\@testopt{\@xs@IfStringCase{#1}{#2}}{}}

\long\def\@xs@IfStringCase#1#2[#3]{%
	\long\def\@xs@testcase##1##2##3\@xs@nil{% lit les 2 premieres unit\'es syntaxiques dans ##1 et ##2. Les autres dans ##3
		\@xs@reserved@E{#1}{##1}%
			{##2}% le test est positif, on ex\'ecute le code correspondant
			{\@xs@ifempty{##3}%
			 	{#3}% s'il n'y a plus de cas, on ex\'ecute le code <autres cas>
				{\@xs@testcase##3\@xs@nil}% sinon, on recommence avec ce qui reste
			 }%
	}%
	\@xs@testcase#2\@xs@nil
}

% Renvoie ce qui est \`a gauche de l'occurence n°#1 de la sous chaine #3 dans la chaine #2
\@xs@newmacro*3\StrBefore{1}{2}{1}{%
	\@xs@cutafteroccur{#2}{#3}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#4}%
}

% Renvoie ce qui est \`a droite de l'occurence n°#1 de la sous chaine #3 dans la chaine #2
\@xs@newmacro*3\StrBehind{1}{2}{1}{%
	\@xs@cutafteroccur{#2}{#3}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@E}{#4}%
}

% Renvoie ce qui est strictement compris entre les occurrences n°#1 et n°#2
% des chaines #4 et #5 dans la chaine #3
\@xs@newmacro*4\StrBetween{1,1}{3}{1}{\@xs@StrBetween@i[#1]{#2}{#3}{#4}[#5]}

\long\def\@xs@StrBetween@i[#1,#2]#3#4#5[#6]{%
	\begingroup
		\noexploregroups
		\@xs@cutafteroccur{#3}{#5}{#2}%
		\expandafter\@xs@cutafteroccur\expandafter{\@xs@reserved@C}{#4}{#1}%
		\expandafter
	\endgroup
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@E}{#6}%
	\global\let\groupID\@empty
}

\def\exploregroups{\let\@xs@exploregroups\relax}

\def\noexploregroups{\def\@xs@exploregroups{\let\@xs@toks0\relax}}

\def\saveexploremode{\let\@xs@saveexploremode\@xs@exploregroups}

\def\restoreexploremode{\let\@xs@exploregroups\@xs@saveexploremode}

% Remplace les #1 premi\`eres occurences de la chaine #3
% par la chaine #4 dans la chaine #2
\@xs@newmacro\StrSubstitute{0}{3}{1}{%
	\def\@xs@reserved@D{#2}\let\@xs@reserved@C\@empty\def\@xs@reserved@E{#3}%
	\def\@xs@argument@C{#3}\def\@xs@argument@D{#4}%
	\decimalpart\z@
	\integerpart\z@
	\gdef\groupID{0}%
	\let\@xs@nestlevel\z@
	\def\@xs@atendofgroup{%
		\expandafter\endgroup
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
		\@xs@read@reserved@D
	}%
	\def\@xs@atoccurfound{%
		\ifnum#1<\@ne
			\let\@xs@reserved@A\@xs@argument@D
		\else
			\ifnum\decimalpart>#1
				\let\@xs@reserved@A\@xs@argument@C
			\else
				\let\@xs@reserved@A\@xs@argument@D
			\fi
		\fi
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@A}%
		\@xs@read@reserved@D
	}%
	\@xs@ifempty{#3}%
		{\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@D}{#5}%
		}
		{\@xs@read@reserved@D
		\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#5}%
		}%
}

% Supprime les #1 premi\`eres occurrences de #3 dans #2
\@xs@newmacro\StrDel{0}{2}{1}{\@xs@StrSubstitute[#1]{#2}{#3}{}[#4]}

\def\@xs@exitallgroups{\ifnum\@xs@nestlevel>\z@\endgroup\expandafter\@xs@exitallgroups\fi}

% Compte combien d'unit\'es syntaxiques contient la chaine #1 ?
\@xs@newmacro\StrLen{}{1}{1}{%
	\def\@xs@reserved@C{#1}%
	\decimalpart\z@
	\let\@xs@nestlevel\z@
	\gdef\groupID{0}%
	\let\@xs@atbegingroup\relax
	\def\@xs@atendofgroup{\endgroup\@xs@read@reserved@C}%
	\let\@xs@atnextsyntaxunit\relax
	\@xs@read@reserved@C
	\expandafter\@xs@ReturnResult\expandafter{\number\decimalpart}{#2}%
}

% Macro interne fermant autant de groupes que n\'ecessaire pour trouver une unit\'e syntaxique derri\`ere
\def\@xs@continuetonext{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		{\ifnum\@xs@nestlevel>\z@
			\expandafter\endgroup\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\expandafter{\@xs@reserved@B}}% on concat\`ene
			\expandafter\expandafter\expandafter\@xs@continuetonext% on recommence
		\fi}
		\relax
}%

\def\@xs@manage@groupID{%
	\begingroup\def\@xs@reserved@A{0}%
	\ifx\@xs@reserved@A\groupID% si on arrive du groupe de niveau 0
		\endgroup
		\xdef\groupID{\number\integerpart}% on met simplement le niveau
	\else
		\endgroup
		\expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter\groupID\expandafter\expandafter\expandafter{\expandafter\groupID\expandafter,\number\integerpart}%
	\fi
}

% Cette macro coupe la chaine #1 apr\`es l'unit\'e syntaxique n°#2
\def\StrSplit{%
	\@ifstar
		{\let\@xs@reserved@E\@xs@continuetonext\StrSpl@t}%
		{\let\@xs@reserved@E\relax\StrSpl@t}%
}

\@xs@newmacro\StrSpl@t{}{2}{0}{\@xs@StrSplit@i{#2}{#1}\@xs@StrSplit@ii}

% Cette macro interne coupe la chaine #2 apr\`es l'unit\'e syntaxique n°#1
% Le d\'ebut est assign\'e dans \@xs@reserved@B et la fin dans \@xs@reserved@C
\long\def\@xs@StrSplit@i#1#2{%
	\def\@xs@reserved@D{#1}%
	\def\@xs@reserved@C{#2}%
	\let\@xs@reserved@B\@empty
	\global\let\groupID\@empty
	\ifnum#1>\z@
		\decimalpart\z@
		\integerpart\z@
		\gdef\groupID{0}%
		\let\@xs@nestlevel\z@
		\def\@xs@atendofgroup{%
			\expandafter\endgroup
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\expandafter{\@xs@reserved@B}}%
			\@xs@read@reserved@C
		}%
		\def\@xs@atbegingroup{\let\@xs@reserved@B\@empty}%
		\def\@xs@atnextsyntaxunit{%
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\@xs@reserved@A}%
			\ifnum\decimalpart=\@xs@reserved@D\relax
				\ifx\@xs@reserved@C\@empty\@xs@reserved@E\fi
				\global\let\@xs@reserved@B\@xs@reserved@B
				\global\let\@xs@reserved@C\@xs@reserved@C
				\@xs@exitallgroups
				\let\@xs@next\relax
			\fi
		}%
		\@xs@read@reserved@C
	\fi
}

\def\@xs@StrSplit@ii#1#2{\let#1\@xs@reserved@B\let#2\@xs@reserved@C}

% StrCut[n]{<texte>}{<motif>}\macroA\macroB
% \macroA reçoit ce qui se trouve avant la n ème occurrence <motif> dans <texte>
% \macroB reçoit ce qui est après cette n ème occurrence
\@xs@newmacro*3\StrCut{1}{2}{0}{%
	\@xs@ifempty{#3}%
		{\global\let\groupID\@empty
		\let\@xs@reserved@C\@empty
		\let\@xs@reserved@E\@empty
		}
		{\ifnum#1<\@ne\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
			{\@xs@StrCut@ii{#2}{#3}1}
			{\@xs@StrCut@ii{#2}{#3}{#1}}%
		}%
	\@xs@StrCut@iii
}

\long\def\@xs@StrCut@ii#1#2#3{%
	\def\@xs@reserved@D{#1}%
	\let\@xs@reserved@C\@empty
	\def\@xs@reserved@E{#2}%
	\decimalpart\z@\integerpart\z@
	\gdef\groupID{0}%
	\let\@xs@nestlevel\z@
	\def\@xs@atendofgroup{%
		\expandafter\endgroup
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
		\@xs@read@reserved@D
	}%
	\def\@xs@atoccurfound{%
		\ifnum\decimalpart=\numexpr(#3)\relax
			\global\let\@xs@reserved@D\@xs@reserved@D
			\global\let\@xs@reserved@C\@xs@reserved@C
			\@xs@exitallgroups
			\let\@xs@next\relax
		\else
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@E}%
			\let\@xs@next\@xs@read@reserved@D
		\fi
	}%
	\@xs@read@reserved@D
	\def\@xs@argument@A{#2}%
	\let\@xs@reserved@E\@xs@reserved@D
		\expandafter\expandafter\expandafter
	\def
		\expandafter\expandafter\expandafter
	\@xs@reserved@D
		\expandafter\expandafter\expandafter
	{\expandafter\@xs@reserved@C\@xs@argument@A}%
}

\long\def\@xs@StrCut@iii#1#2{\let#1\@xs@reserved@C\let#2\@xs@reserved@E}

% De la chaine #1, renvoie ce qui se trouve entre les positions
%  #2 et #3, unit\'es syntaxiques aux positions compris !
\@xs@newmacro\StrMid{}{3}{1}{%
	\begingroup
		\noexploregroups
		\let\@xs@reserved@E\relax
		\@xs@StrSplit@i{#3}{#1}%
		\edef\@xs@reserved@C{\number\numexpr#2-1}%
		\let\@xs@reserved@E\relax
		\expandafter\expandafter\expandafter\@xs@StrSplit@i\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\expandafter}\expandafter{\@xs@reserved@B}%
	\expandafter\endgroup
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#4}%
	\global\let\groupID\@empty
}

% supprime #2 unit\'es syntaxiques \`a gauche dans la chaine #1
\@xs@newmacro\StrGobbleLeft{}{2}{1}{%
	\let\@xs@reserved@E\relax
	\@xs@StrSplit@i{#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#3}%
}

% extrait de #1 la chaine \`a gauche de longueur #2
\@xs@newmacro\StrLeft{}{2}{1}{%
	\let\@xs@reserved@E\relax
	\@xs@StrSplit@i{#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#3}%
}

% supprime #2 unit\'es syntaxiques \`a droite dans la chaine #1
\@xs@newmacro\StrGobbleRight{}{2}{1}{%
	\@xs@StrLen{#1}[\@xs@reserved@D]%
	\let\@xs@reserved@E\relax
	\expandafter\@xs@StrSplit@i\expandafter{\number\numexpr\@xs@reserved@D-#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#3}%
}

% renvoie #2 unit\'es syntaxiques \`a la droite de la chaine #1
\@xs@newmacro\StrRight{}{2}{1}{%
	\@xs@StrLen{#1}[\@xs@reserved@D]%
	\let\@xs@reserved@E\relax
	\expandafter\@xs@StrSplit@i\expandafter{\number\numexpr\@xs@reserved@D-#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#3}%
}

\@xs@newmacro\StrChar{}{2}{1}{%
	\let\@xs@reserved@B\@empty
	\def\@xs@reserved@C{#1}\def\@xs@reserved@D{#2}%
	\ifnum#2>\z@
		\def\groupID{0}\let\@xs@nestlevel\z@\integerpart\z@\decimalpart\z@
		\let\@xs@atbegingroup\relax
		\def\@xs@atendofgroup{\endgroup\@xs@read@reserved@C}%
		\def\@xs@atnextsyntaxunit{%
			\ifnum\decimalpart=\@xs@reserved@D% la n i\`eme US est atteinte ?
				\global\let\@xs@reserved@B\@xs@reserved@A% on capture l'US en cours qui est celle cherch\'ee
				\@xs@exitallgroups
				\let\@xs@next\relax
			\fi
		}%
		\@xs@read@reserved@C
	\fi
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@B}%
		{\global\let\groupID\@empty}
		\relax
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#3}%
}

% Combien de fois compte t-on #2 dans #1 ?
\@xs@newmacro\StrCount{}{2}{1}{%
	\def\@xs@reserved@D{#1}\def\@xs@reserved@E{#2}\let\@xs@reserved@C\@empty
	\@xs@ifempty{#2}%
		{\@xs@ReturnResult{0}{#3}}
		{\decimalpart\z@
		\integerpart\z@
		\gdef\groupID{0}%
		\let\@xs@nestlevel\z@
		\def\@xs@atendofgroup{%
			\expandafter\endgroup
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
			\@xs@read@reserved@D
		}%
		\def\@xs@atoccurfound{\let\@xs@reserved@C\@empty\@xs@read@reserved@D}%
		\@xs@read@reserved@D
		\expandafter\@xs@ReturnResult\expandafter{\number\decimalpart}{#3}%
		}%
}

% renvoie la position de l'occurrence #1 de la sous chaine #3 dans la chaine #2
\@xs@newmacro\StrPosition{1}{2}{1}{%
	\@xs@cutafteroccur{#2}{#3}{#1}%
	\let\@xs@reserved@E\groupID
	\ifx\@xs@reserved@C\@xs@reserved@D
		\@xs@ReturnResult{0}{#4}%
		\let\@xs@reserved@E\@empty
	\else
		\expandafter\@xs@StrLen\expandafter{\@xs@reserved@C}[\@xs@reserved@C]%
		\expandafter\@xs@ReturnResult\expandafter{\number\numexpr\@xs@reserved@C+1}{#4}%
	\fi
	\global\let\groupID\@xs@reserved@E
}

\def\comparestrict{\let\@xs@comparecoeff\@ne}

\def\comparenormal{\let\@xs@comparecoeff\z@}

\def\savecomparemode{\let\@xs@saved@comparecoeff\@xs@comparecoeff}

\def\restorecomparemode{\let\@xs@comparecoeff\@xs@saved@comparecoeff}

% Compare les deux arguments #1 et #2
% Renvoie 0 s'ils sont \'egaux et renvoie la
% position de la premiere unit\'e syntaxiques diff\'erente sinon
\@xs@newmacro*2\StrCompare{}{2}{1}{%
	\def\@xs@reserved@A{#1}%
	\def\@xs@reserved@B{#2}%
	\ifx\@xs@reserved@B\@xs@reserved@A
		\@xs@ReturnResult{0}{#3}%
	\else
		\def\@xs@next{\@xs@StrCompare@i{#1}{#2}{#3}}%
		\expandafter\@xs@next
	\fi
}

\long\def\@xs@StrCompare@i#1#2#3{%
	\def\@xs@StrCompare@iii##1{%
		\let\@xs@reserved@A\@empty
		\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
			{\def\@xs@reserved@A{*\@xs@comparecoeff}}%
			{\expandafter\@xs@ifempty\expandafter{\@xs@reserved@D}%
				{\def\@xs@reserved@A{*\@xs@comparecoeff}}
				\relax
			}%
		\def\@xs@next{%
			\expandafter\@xs@ReturnResult\expandafter
			{\number\numexpr##1\@xs@reserved@A\relax}{#3}%
		}%
	}%
	\def\@xs@StrCompare@ii##1{% ##1 est la position
		\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@A
		\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@B
		\ifx\@xs@reserved@B\@xs@reserved@A
			\expandafter\@xs@ifempty\expandafter{\@xs@reserved@A}%
				{\@xs@StrCompare@iii{##1}% les 2 unit\'es syntaxiques sont \'egales, on renvoie la position
				}
				{\def\@xs@next{\expandafter\@xs@StrCompare@ii\expandafter{\number\numexpr##1+1}}% les 2 unit\'es syntaxiques sont \'egales et non vides, on recommence
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@D
				}%
		\else% les 2 unit\'es syntaxiques sont diff\'erentes : on renvoie la position
			\@xs@StrCompare@iii{##1}%
		\fi
		\@xs@next
	}%
	\def\@xs@reserved@C{#1}\def\@xs@reserved@D{#2}%
	\@xs@StrCompare@ii1%
}

\@xs@newmacro\StrFindGroup{}{2}{1}{%
	\def\@xs@reserved@A{#2}\def\@xs@reserved@B{0}%
	\ifx\@xs@reserved@A\@xs@reserved@B
		\def\@xs@next{\@xs@ReturnResult{{#1}}{#3}}%
	\else
		\def\@xs@next{\@xs@StrFindGroup@i{#1}{#2}[#3]}%
	\fi
	\@xs@next
}

\long\def\@xs@StrFindGroup@i#1#2[#3]{%
	\def\@xs@StrFindGroup@ii{%
		\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
			{\def\@xs@next{\@xs@ReturnResult{}{#3}}% s'il ne reste plus rien, on renvoie vide
			}
			{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@D
			\ifx\bgroup\@xs@toks% si la 1\`ere unit\'e syntaxique est un groupe explicite
				\advance\decimalpart\@ne% on augmente le compteur
				\ifnum\decimalpart=\@xs@reserved@A% on est au groupe cherch\'e lors de la profondeur courante ?
					\ifx\@empty\@xs@reserved@B% on est \`a la profondeur maximale ?
						\def\@xs@next{\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@D}{#3}}% on renvoie ce groupe
					\else% sinon
						\expandafter\def\expandafter\@xs@next\expandafter{\expandafter\@xs@StrFindGroup@i\@xs@reserved@D}% on recommence avec ce groupe
						\expandafter\@xs@addtomacro\expandafter\@xs@next\expandafter{\expandafter{\@xs@reserved@B}[#3]}% et les profondeurs de recherche restantes
					\fi
				\else
					\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
					\let\@xs@next\@xs@StrFindGroup@ii
				\fi
			\else
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
				\let\@xs@next\@xs@StrFindGroup@ii
			\fi
			}%
		\@xs@next
	}%
	\@xs@extractgroupnumber{#2}\@xs@reserved@A\@xs@reserved@B
	\decimalpart\z@
	\ifnum\@xs@reserved@A>\z@\def\@xs@reserved@C{#1}\else\let\@xs@reserved@C\@empty\fi
	\@xs@StrFindGroup@ii
}

\def\@xs@extractgroupnumber#1#2#3{%
	\def\@xs@extractgroupnumber@i##1,##2\@xs@nil{\def#2{##1}\def#3{##2}}%
	\@xs@extractgroupnumber@i#1,\@xs@nil
	\ifx\@empty#3\else\@xs@extractgroupnumber@i#1\@xs@nil\fi
}

\def\expandingroups{\let\@xs@expandingroups\exploregroups}

\def\noexpandingroups{\let\@xs@expandingroups\noexploregroups}

\def\StrExpand{\@testopt{\@xs@StrExpand}{1}}
\long\def\@xs@StrExpand[#1]#2#3{%
	\begingroup
		\@xs@expandingroups
		\ifnum#1>\z@
			\integerpart#1\relax
			\decimalpart\z@
			\gdef\groupID{0}%
			\let\@xs@nestlevel\z@
			\def\@xs@atendofgroup{%
				\expandafter\endgroup
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\expandafter{\@xs@reserved@B}}%
				\@xs@read@reserved@C
			}%
			\def\@xs@atbegingroup{\let\@xs@reserved@B\@empty}%
			\def\@xs@atnextsyntaxunit{%
				\expandafter\expandafter\expandafter\@xs@addtomacro
				\expandafter\expandafter\expandafter\@xs@reserved@B
				\expandafter\expandafter\expandafter{\@xs@reserved@A}%
			}%
			\def\@xs@reserved@C{#2}%
			\@xs@StrExpand@i{#1}% Appel de la macro r\'ecursive
		\else
			\def\@xs@reserved@B{#2}%
		\fi
		\global\let\@xs@reserved@B\@xs@reserved@B
	\endgroup
	\let#3\@xs@reserved@B
	\global\let\groupID\@empty
}

\long\def\@xs@StrExpand@i#1{%
	\ifnum#1>\z@
		\let\@xs@reserved@B\@empty
		\@xs@read@reserved@C
		\let\@xs@reserved@C\@xs@reserved@B
		\def\@xs@reserved@A{\expandafter\@xs@StrExpand@i\expandafter{\number\numexpr#1-1}}%
	\else
		\let\@xs@reserved@A\relax
	\fi
	\@xs@reserved@A
}

\def\scancs{\@testopt{\@xs@scancs}{1}}
\long\def\@xs@scancs[#1]#2#3{%
	\@xs@StrExpand[#1]{#3}{#2}%
	\edef#2{\detokenize\expandafter{#2}}%
}

% Restaure le code de @
\catcode`\@=\CurrentAtCatcode\relax

% D\'efinit le d\'elimiteur verb
% d\'efinit les diff\'erents modes et les m\'emorise
\setverbdelim{|}%
\fullexpandarg\saveexpandmode
\comparenormal\savecomparemode
\noexploregroups\saveexploremode
\expandingroups

\endinput
%
% Historique
%------------------------------------------------------------------------------
%% v1.0    4/7/2008 : - Package achev\'e.
%          7/7/2008 : - Package publi\'e sur CTAN.
%------------------------------------------------------------------------------
% v1.1    15/8/2008
%   - Le package ne n\'ecessite plus LaTeX et est d\'esormais utilisable sous
%     Plain eTeX.
%   - Ajout des macros \IfInteger et \IfDecimal.
%     Pour cette derni\`ere, la partie enti\`ere et la partie d\'ecimale sont
%     r\'ecup\'erables dans les compteurs \integerpart et \decimalpart. Ce
%     qu'il reste apr\`es qu'un caract\`ere non attendu soit rencontr\'e est
%     dispo dans \@xs@remainafterdecimal
%   - Correction d'un bug dans \tokenize :
%        suppression de l'expansion avec \normalexpandarg pour \'eviter le bug
%        avec les lettres accentu\'ees dans l'exemple : \tokenize\aa{\'e\`u}
%   - Am\'elioration du code de la plupart des macros.
%   - \'Ecriture d'une routine \@xs@newmacro d\'efinissant les  macros.
%   - Suppression de tous les compteurs grace \`a \numexpr.
%   - Nouvelles fonctionnalit\'es internes dans :
%      \IfSubStr
%        ajout des chaines se trouvant avant et apr\`es l'occurrence test\'ee
%        dans les sc \@xs@behind@IfSubStr et \@xs@before@IfSubStr
%      \StrCount
%        a) ajout de ce qui se trouve apr\`es la derni\`ere occurrence dans la
%           sc \@xs@StrCount@afterlastocccur
%        b) la macro ne d\'epend plus d'aucune autre
%------------------------------------------------------------------------------
% v1.2    23/8/2008
%   - Am\'elioration du code de \StrMid \StrGobbleLeft, \StrLeft,
%     \StrGobbleRight et \StrRight \`a l'aide de la nouvelle macro
%     \@xs@StrSplit@i
%   - Nouveau test \IfStrEq qui compare 2 chaines
%   - Nouveau test \IfEq qui compare 2 chaines (ou 2 nombres si les 2 chaines
%     contiennent un nombre)
%   - Correction d'un bug dans \@xs@formatnumber. La macro n'envisageait pas le
%     cas o\`u son argument \'etait vide ce qui faiasait planter
%     \IfDecimal{}{V}{F} et \IfInteger{}{V}{F}
%------------------------------------------------------------------------------
% v1.3    21/9/2008
%  - Am\'elioration du code, mise en place de r\'ecursivit\'es terminales dans
%    toutes les macros r\'ecursives, simplification de \@xs@TestEqual en
%    utilisant \ifx
%  - Nouvelles macros \IfStrEqCase et \IfEqCase
%      Teste si une chaîne est \'egale \`a plusieurs cha\^ines donn\'ee et
%      ex\'ecute un code sp\'ecifique
%  - Cr\'eation de la macro publique \StrSplit
%      Coupe la chaine en 2 \`a une position donn\'ee
%  - Nouvelle macro \StrCompare
%      Compare 2 chaînes et renvoie la position du 1er caract\`ere diff\'erent.
%      Renvoie 0 si elles sont \'egales.
%------------------------------------------------------------------------------
% v1.3a   29/9/2008
%  - Correction d'un bug : \expandafter#1
%    dans les macros \IfSubStrBefore et \StrBetween qui buggue si #1 est un
%    nombre > 9 !
%  - R\'e \'ecriture de \@xs@returnfirstsyntaxunit et \@gobble qui
%    deviennent purement d\'eveloppables.
%  - R\'e \'ecriture de \StrLen
%  - Nouvelle macro interne \@xs@cutafteroccur
%      Coupe la chaine apr\`es la ni\`eme occurrence d'une sous chaine.
%  - Code am\'elior\'e de \StrMid, \StrLeft, \StrGobbleLeft, \StrRight,
%    \StrGobbleRight grace \`a \@xs@cutafteroccur
%------------------------------------------------------------------------------
% v1.4   4/11/2008
%  - xstring traite ses arguments par unit\'e syntaxique, et donc toutes les
%    macros internes ont \'et\'e r\'e-\'ecrites \`a cette fin.
%  - Le manuel a \'et\'e r\'e-\'ecrit, rendu plus clair et mieux structur\'e.
%  - Nouvelle fonctionnalit\'e : \expandarg
%      le 1er lex\`eme de chaque argument est 1-d\'evelopp\'e avant que la
%      macro ne soit appel\'ee. Si un argument comporte plus qu'1 lex\`eme,
%      il faut passer par \scancs*[1] pour 1-d\'evelopper toutes les unit\'es
%      syntaxiques.
%  - Correction de 2 erreurs dans le manuel anglais :  0 est la valeur par
%    d\'efaut dans \StrSubstitute et \StrDel
%  - Coh\'erence dans les nom des s\'equences de contr\^oles temporaires qui
%    sont d\'esormais : \@xs@reserved@A \`a \@xs@reserved@E
%------------------------------------------------------------------------------
% v1.4a  12/11/2008
%  - Correction d'un bug dans \@xs@StrSplit dans le cas o\`u l'argument
%     num\'erique est <1 : la 1ere coupure doit être vide et le seconde doit
%     être \'egale \`a l'argument.
%------------------------------------------------------------------------------
% v1.4b  16/11/2008
%  - Correction de 2 bugs dans \@xs@returnfirstsyntaxunit
%------------------------------------------------------------------------------
% v1.5   31/12/2008
%  - Nouvelles fonctionnalit\'es dans la recherche de groupes par un
%    identificateur caract\'erisant leur imbrication. Impl\'ementation de :
%      1) \StrFindGroup
%      2) \groupID
%  - Ajout des nouvelles macros g\'en\'eriques \@xs@read@reserved@C et
%    \@xs@read@reserved@D
%  - Correction d'un bug dans \StrSplit : \StrSplit{{a}bc}{1}[\truc] faisait
%    que \truc contenait «a{a}».
%  - Correction d'un bug dans \@xs@newmacro : l'argument optionnel \'etait
%    d\'etok\'enis\'e \`a tort dans les macros \'etoil\'ees.
%  - Dans \@xs@newmacro, on doit choisir le num\'ero du dernier argument devant
%    être d\'etok\'enis\'e dans le cas d'une macro \'etoil\'ee (sachant que
%     l'argument optionnel ne l'est jamais)
%------------------------------------------------------------------------------
% v1.5a  09/2/2009
%  - Nouvelle macro \StrExpand, sensible au mode d'exploration. La macro est
%    indépendante du mode d'exploration et dispose de ses propres commandes
%    d'exploration : \expandingroups et \noexpandingroups
%  - R\'e-\'ecriture de \scancs, qui devient triviale puisque d\'ependant de
%    \StrExpand. Il n'y a plus de version \'étoil\'ee et d\'esormais, \scancs
%    est sensible au mode d'exploration.
%  - Correction d'un bug dans \IfInteger : \IfInteger{2.0}{V}{F} affichait F
%  - Correction de bugs : mettre \let\@xs@reserved@E\relax avant d'appeler
%    \@xs@StrSplit@i
%  - Suppression des messages d'erreur, de warning et d'info. xstring devient
%    donc silencieux ;)
%  - Passage de 3 \'a 2 compteurs
%  - Le manuel est d\'esormais plus color\'e, en esp\'erant qu'il sera un peu
%    plus agr\'eable \`a lire !
%------------------------------------------------------------------------------
% v1.5b  13/3/2009
%  - Modification d'un grand nombre de macros de telle sorte que vraiment
%    n'importe quel code peut d\'esormais \^etre plac\'e dans les arguments des
%    macros (comme par exemple des \if, \ifx ou autre, m\^eme sans leur \fi, ce
%    qui n'\'etait pas possible jusqu'alors)
%------------------------------------------------------------------------------
% v1.5c  05/6/2009
%  - Correction d'un bug dans \IfBeginWith : il faut appeler
%    \@xs@returnfirstsyntaxunit pour l'argument #2 puis pour l'argument #1 et
%    non pas l'inverse pour que \@xs@toks reflète ce qui se trouve dans #1
%  - Correction d'un bug dans \@xs@returnfirstsyntaxunit au cas où #1 commence
%    par un espace : mettre \@xs@toks à 0
%  - Correction d'un bug dans \@xs@returnfirstsyntaxunit :
%    \@xs@returnfirstsyntaxunit{{}}\truc
%    faisait que \truc se développait en un espace.
%  - Correction d'un bug dans \@xs@removefirstsyntaxunit où le cas
%    \@xs@removefirstsyntaxunit{ {b}}\truc
%    donnait \truc se développant en «b» au lieu de «{b}».
%------------------------------------------------------------------------------
% v1.5d  28/3/2010
%  - Correction d'un bug dans \IfInteger : \@xs@afterinteger ne donnait pas le
%    bon r\'esultat. Par exemple avec 1.23 il renvoyait {} au lieu de {.23}
%  - \xs@formatnumber ne detokenize plus ses arguments (que m'est-il pass\'e
%    par la t\^ete pour que je code un truc comme ca ?), et donc
%    \@xs@afterinteger et \@xs@afterdecimal ont des tokens ayant le bon
%    catcode
%------------------------------------------------------------------------------
% v1.6  24/10/2012
%  - Correction d'un bug dans \@xs@cutafteroccur au cas o\`u #3<1
%  - \IfDecimal ne \detokenize plus l'argument.
%  - Nouvelle version de \tokenize qui enlevait les accolades si son argument
%    \'etait entre accolades
%  - Nouvelle macro \StrCut
%  - \@xs@cutafteroccur@i ne produit plus d'espace indésirable si #3 était
%    évalué par \numexpr
%------------------------------------------------------------------------------
% v1.7  13/1/2013
%  - Correction d'un manque de rigueur dans les assignations concernant
%    \groupID : elles sont toutes globales d\'esormais
%  - Les macros de xstring sont \long
%------------------------------------------------------------------------------
% v1.7a 28/2/2013
%  - Correction d'un espace parasite dans \@xs@removefirstsyntaxunit
%------------------------------------------------------------------------------
% v1.7b 29/7/2013
%  - La date contenue dans \xstringdate est désormais conforme
%------------------------------------------------------------------------------
% v1.7c 13/10/2013 
%  - les macros impliquées dans \IfStrCase et \IfStrEqCase sont désormais \long
